An analysis of linear regression and neural networks approximation for the pricing of swing options

Linear regression, firstly introduced for the pricing of American-style options, has since been expanded to include swing options pricing. Swing options price may be viewed as the solution to a Backward Dynamic Programming Principle, which involves a conditional expectation known as the continuation value. The approximation of the continuation value using linear regression involves two levels of approximation. First, the continuation value is replaced by an orthogonal projection over a subspace spanned by a finite set of $m$ squared-integrable functions yielding a first approximation $V^m$ of the swing value function. In this paper, we prove that, with well-chosen regression functions, $V^m$ converges to the swing actual price $V$ as $m \to + \infty$. A similar result is proved when classic regression functions are replaced by neural networks. For both methods (linear regression and neural networks), we analyze the second level of approximation involving practical computation of the swing price using Monte Carlo simulations and yielding an approximation $V^{m, N}$ (where $N$ denotes the Monte Carlo sample size). Especially, we prove that $V^{m, N} \to V^m$ as $N \to + \infty$ for both methods and using a Hilbert basis assumption in the linear regression. Besides, a convergence rate of order $\mathcal{O}\big(\frac{1}{\sqrt{N}} \big)$ is proved in the linear regression case.

==> biblio/Continuity_of_the_infimum___Bubbles__Bad__Ripples__Good_files/saved_resource <==
/**
 The MIT License

 Copyright (c) 2010 Daniel Park (http://metaweb.com, http://postmessage.freebaseapps.com)

 Permission is hereby granted, free of charge, to any person obtaining a copy
 of this software and associated documentation files (the "Software"), to deal
 in the Software without restriction, including without limitation the rights
 to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
 copies of the Software, and to permit persons to whom the Software is
 furnished to do so, subject to the following conditions:

 The above copyright notice and this permission notice shall be included in
 all copies or substantial portions of the Software.

 THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
 IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
 FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
 AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
 LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
 OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN
 THE SOFTWARE.
 **/
var NO_JQUERY = {};
(function(window, $, undefined) {

     if (!("console" in window)) {
         var c = window.console = {};
         c.log = c.warn = c.error = c.debug = function(){};
     }

     if ($ === NO_JQUERY) {
         // jQuery is optional
         $ = {
             fn: {},
             extend: function() {
                 var a = arguments[0];
                 for (var i=1,len=arguments.length; i<len; i++) {
                     var b = arguments[i];
                     for (var prop in b) {
                         a[prop] = b[prop];
                     }
                 }
                 return a;
             }
         };
     }

     $.fn.pm = function() {
         console.log("usage: \nto send:    $.pm(options)\nto receive: $.pm.bind(type, fn, [origin])");
         return this;
     };

     // send postmessage
     $.pm = window.pm = function(options) {
         pm.send(options);
     };

     // bind postmessage handler
     $.pm.bind = window.pm.bind = function(type, fn, origin, hash, async_reply) {
         pm.bind(type, fn, origin, hash, async_reply === true);
     };

     // unbind postmessage handler
     $.pm.unbind = window.pm.unbind = function(type, fn) {
         pm.unbind(type, fn);
     };

     // default postmessage origin on bind
     $.pm.origin = window.pm.origin = null;

     // default postmessage polling if using location hash to pass postmessages
     $.pm.poll = window.pm.poll = 200;

     var pm = {

         send: function(options) {
             var o = $.extend({}, pm.defaults, options),
             target = o.target;
             if (!o.target) {
                 console.warn("postmessage target window required");
                 return;
             }
             if (!o.type) {
                 console.warn("postmessage type required");
                 return;
             }
             var msg = {data:o.data, type:o.type};
             if (o.success) {
                 msg.callback = pm._callback(o.success);
             }
             if (o.error) {
                 msg.errback = pm._callback(o.error);
             }
             if (("postMessage" in target) && !o.hash) {
                 pm._bind();
                 target.postMessage(JSON.stringify(msg), o.origin || '*');
             }
             else {
                 pm.hash._bind();
                 pm.hash.send(o, msg);
             }
         },

         bind: function(type, fn, origin, hash, async_reply) {
           pm._replyBind ( type, fn, origin, hash, async_reply );
         },

         _replyBind: function(type, fn, origin, hash, isCallback) {
           if (("postMessage" in window) && !hash) {
               pm._bind();
           }
           else {
               pm.hash._bind();
           }
           var l = pm.data("listeners.postmessage");
           if (!l) {
               l = {};
               pm.data("listeners.postmessage", l);
           }
           var fns = l[type];
           if (!fns) {
               fns = [];
               l[type] = fns;
           }
           fns.push({fn:fn, callback: isCallback, origin:origin || $.pm.origin});
         },

         unbind: function(type, fn) {
             var l = pm.data("listeners.postmessage");
             if (l) {
                 if (type) {
                     if (fn) {
                         // remove specific listener
                         var fns = l[type];
                         if (fns) {
                             var m = [];
                             for (var i=0,len=fns.length; i<len; i++) {
                                 var o = fns[i];
                                 if (o.fn !== fn) {
                                     m.push(o);
                                 }
                             }
                             l[type] = m;
                         }
                     }
                     else {
                         // remove all listeners by type
                         delete l[type];
                     }
                 }
                 else {
                     // unbind all listeners of all type
                     for (var i in l) {
                       delete l[i];
                     }
                 }
             }
         },

         data: function(k, v) {
             if (v === undefined) {
                 return pm._data[k];
             }
             pm._data[k] = v;
             return v;
         },

         _data: {},

         _CHARS: '0123456789ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz'.split(''),

         _random: function() {
             var r = [];
             for (var i=0; i<32; i++) {
                 r[i] = pm._CHARS[0 | Math.random() * 32];
             };
             return r.join("");
         },

         _callback: function(fn) {
             var cbs = pm.data("callbacks.postmessage");
             if (!cbs) {
                 cbs = {};
                 pm.data("callbacks.postmessage", cbs);
             }
             var r = pm._random();
             cbs[r] = fn;
             return r;
         },

         _bind: function() {
             // are we already listening to message events on this w?
             if (!pm.data("listening.postmessage")) {
                 if (window.addEventListener) {
                     window.addEventListener("message", pm._dispatch, false);
                 }
                 else if (window.attachEvent) {
                     window.attachEvent("onmessage", pm._dispatch);
                 }
                 pm.data("listening.postmessage", 1);
             }
         },

         _dispatch: function(e) {
             //console.log("$.pm.dispatch", e, this);
             try {
                 var msg = JSON.parse(e.data);
             }
             catch (ex) {
                 //console.warn("postmessage data invalid json: ", ex); //message wasn't meant for pm
                 return;
             }
             if (!msg.type) {
                 //console.warn("postmessage message type required"); //message wasn't meant for pm
                 return;
             }
             var cbs = pm.data("callbacks.postmessage") || {},
             cb = cbs[msg.type];
             if (cb) {
                 cb(msg.data);
             }
             else {
                 var l = pm.data("listeners.postmessage") || {};
                 var fns = l[msg.type] || [];
                 for (var i=0,len=fns.length; i<len; i++) {
                     var o = fns[i];
                     if (o.origin && o.origin !== '*' && e.origin !== o.origin) {
                         console.warn("postmessage message origin mismatch", e.origin, o.origin);
                         if (msg.errback) {
                             // notify post message errback
                             var error = {
                                 message: "postmessage origin mismatch",
                                 origin: [e.origin, o.origin]
                             };
                             pm.send({target:e.source, data:error, type:msg.errback});
                         }
                         continue;
                     }

                     function sendReply ( data ) {
                       if (msg.callback) {
                           pm.send({target:e.source, data:data, type:msg.callback});
                       }
                     }

                     try {
                         if ( o.callback ) {
                           o.fn(msg.data, sendReply, e);
                         } else {
                           sendReply ( o.fn(msg.data, e) );
                         }
                     }
                     catch (ex) {
                         if (msg.errback) {
                             // notify post message errback
                             pm.send({target:e.source, data:ex, type:msg.errback});
                         } else {
                             throw ex;
                         }
                     }
                 };
             }
         }
     };

     // location hash polling
     pm.hash = {

         send: function(options, msg) {
             //console.log("hash.send", target_window, options, msg);
             var target_window = options.target,
             target_url = options.url;
             if (!target_url) {
                 console.warn("postmessage target window url is required");
                 return;
             }
             target_url = pm.hash._url(target_url);
             var source_window,
             source_url = pm.hash._url(window.location.href);
             if (window == target_window.parent) {
                 source_window = "parent";
             }
             else {
                 try {
                     for (var i=0,len=parent.frames.length; i<len; i++) {
                         var f = parent.frames[i];
                         if (f == window) {
                             source_window = i;
                             break;
                         }
                     };
                 }
                 catch(ex) {
                     // Opera: security error trying to access parent.frames x-origin
                     // juse use window.name
                     source_window = window.name;
                 }
             }
             if (source_window == null) {
                 console.warn("postmessage windows must be direct parent/child windows and the child must be available through the parent window.frames list");
                 return;
             }
             var hashmessage = {
                 "x-requested-with": "postmessage",
                 source: {
                     name: source_window,
                     url: source_url
                 },
                 postmessage: msg
             };
             var hash_id = "#x-postmessage-id=" + pm._random();
             target_window.location = target_url + hash_id + encodeURIComponent(JSON.stringify(hashmessage));
         },

         _regex: /^\#x\-postmessage\-id\=(\w{32})/,

         _regex_len: "#x-postmessage-id=".length + 32,

         _bind: function() {
             // are we already listening to message events on this w?
             if (!pm.data("polling.postmessage")) {
                 setInterval(function() {
                                 var hash = "" + window.location.hash,
                                 m = pm.hash._regex.exec(hash);
                                 if (m) {
                                     var id = m[1];
                                     if (pm.hash._last !== id) {
                                         pm.hash._last = id;
                                         pm.hash._dispatch(hash.substring(pm.hash._regex_len));
                                     }
                                 }
                             }, $.pm.poll || 200);
                 pm.data("polling.postmessage", 1);
             }
         },

         _dispatch: function(hash) {
             if (!hash) {
                 return;
             }
             try {
                 hash = JSON.parse(decodeURIComponent(hash));
                 if (!(hash['x-requested-with'] === 'postmessage' &&
                       hash.source && hash.source.name != null && hash.source.url && hash.postmessage)) {
                     // ignore since hash could've come from somewhere else
                     return;
                 }
             }
             catch (ex) {
                 // ignore since hash could've come from somewhere else
                 return;
             }
             var msg = hash.postmessage,
             cbs = pm.data("callbacks.postmessage") || {},
             cb = cbs[msg.type];
             if (cb) {
                 cb(msg.data);
             }
             else {
                 var source_window;
                 if (hash.source.name === "parent") {
                     source_window = window.parent;
                 }
                 else {
                     source_window = window.frames[hash.source.name];
                 }
                 var l = pm.data("listeners.postmessage") || {};
                 var fns = l[msg.type] || [];
                 for (var i=0,len=fns.length; i<len; i++) {
                     var o = fns[i];
                     if (o.origin) {
                         var origin = /https?\:\/\/[^\/]*/.exec(hash.source.url)[0];
                         if (o.origin !== '*' && origin !== o.origin) {
                             console.warn("postmessage message origin mismatch", origin, o.origin);
                             if (msg.errback) {
                                 // notify post message errback
                                 var error = {
                                     message: "postmessage origin mismatch",
                                     origin: [origin, o.origin]
                                 };
                                 pm.send({target:source_window, data:error, type:msg.errback, hash:true, url:hash.source.url});
                             }
                             continue;
                         }
                     }

                     function sendReply ( data ) {
                       if (msg.callback) {
                         pm.send({target:source_window, data:data, type:msg.callback, hash:true, url:hash.source.url});
                       }
                     }

                     try {
                         if ( o.callback ) {
                           o.fn(msg.data, sendReply);
                         } else {
                           sendReply ( o.fn(msg.data) );
                         }
                     }
                     catch (ex) {
                         if (msg.errback) {
                             // notify post message errback
                             pm.send({target:source_window, data:ex, type:msg.errback, hash:true, url:hash.source.url});
                         } else {
                             throw ex;
                         }
                     }
                 };
             }
         },

         _url: function(url) {
             // url minus hash part
             return (""+url).replace(/#.*$/, "");
         }

     };

     $.extend(pm, {
                  defaults: {
                      target: null,  /* target window (required) */
                      url: null,     /* target window url (required if no window.postMessage or hash == true) */
                      type: null,    /* message type (required) */
                      data: null,    /* message data (required) */
                      success: null, /* success callback (optional) */
                      error: null,   /* error callback (optional) */
                      origin: "*",   /* postmessage origin (optional) */
                      hash: false    /* use location hash for message passing (optional) */
                  }
              });

 })(this, typeof jQuery === "undefined" ? NO_JQUERY : jQuery);
;
var Jed=function(){"use strict";var a,u,c,l;a={"(":9,"!":8,"*":7,"/":7,"%":7,"+":6,"-":6,"<":5,"<=":5,">":5,">=":5,"==":4,"!=":4,"&&":3,"||":2,"?":1,"?:":1},u=["(","?"],c={")":["("],":":["?","?:"]},l=/<=|>=|==|!=|&&|\|\||\?:|\(|!|\*|\/|%|\+|-|<|>|\?|\)|:/;var p={"!":function(t){return!t},"*":function(t,n){return t*n},"/":function(t,n){return t/n},"%":function(t,n){return t%n},"+":function(t,n){return t+n},"-":function(t,n){return t-n},"<":function(t,n){return t<n},"<=":function(t,n){return t<=n},">":function(t,n){return n<t},">=":function(t,n){return n<=t},"==":function(t,n){return t===n},"!=":function(t,n){return t!==n},"&&":function(t,n){return t&&n},"||":function(t,n){return t||n},"?:":function(t,n,e){if(t)throw n;return e}};function o(t){var n=function(t){for(var n,e,r,i,o=[],s=[];n=t.match(l);){for(e=n[0],(r=t.substr(0,n.index).trim())&&o.push(r);i=s.pop();){if(c[e]){if(c[e][0]===i){e=c[e][1]||e;break}}else if(0<=u.indexOf(i)||a[i]<a[e]){s.push(i);break}o.push(i)}c[e]||s.push(e),t=t.substr(n.index+e.length)}return(t=t.trim())&&o.push(t),o.concat(s.reverse())}(t);return function(t){return function(t,n){var e,r,i,o,s,a,u=[];for(e=0;e<t.length;e++){if(s=t[e],o=p[s]){for(r=o.length,i=Array(r);r--;)i[r]=u.pop();try{a=o.apply(null,i)}catch(t){return t}}else a=n.hasOwnProperty(s)?n[s]:+s;u.push(a)}return u[0]}(n,t)}}var r={contextDelimiter:"",onMissingKey:null};function i(t,n){var e;for(e in this.data=t,this.pluralForms={},this.options={},r)this.options[e]=void 0!==n&&e in n?n[e]:r[e]}i.prototype.getPluralForm=function(t,n){var e,r,i=this.pluralForms[t];return i||("function"!=typeof(r=(e=this.data[t][""])["Plural-Forms"]||e["plural-forms"]||e.plural_forms)&&(r=function(t){var n=o(t);return function(t){return+n({n:t})}}(function(t){var n,e,r;for(n=t.split(";"),e=0;e<n.length;e++)if(0===(r=n[e].trim()).indexOf("plural="))return r.substr(7)}(e["Plural-Forms"]||e["plural-forms"]||e.plural_forms))),i=this.pluralForms[t]=r),i(n)},i.prototype.dcnpgettext=function(t,n,e,r,i){var o,s,a;return o=void 0===i?0:this.getPluralForm(t,i),s=e,n&&(s=n+this.options.contextDelimiter+e),(a=this.data[t][s])&&a[o]?a[o]:(this.options.onMissingKey&&this.options.onMissingKey(e,t),0===o?e:r)};var n=/%(((\d+)\$)|(\(([$_a-zA-Z][$_a-zA-Z0-9]*)\)))?[ +0#-]*\d*(\.(\d+|\*))?(ll|[lhqL])?([cduxXefgsp%])/g;function s(t,o){var s;if(!Array.isArray(o))for(o=new Array(arguments.length-1),s=1;s<arguments.length;s++)o[s-1]=arguments[s];return s=1,t.replace(n,function(){var t,n,e,r,i;return t=arguments[3],n=arguments[5],e=arguments[7],"%"===(r=arguments[9])?"%":("*"===e&&(e=o[s-1],s++),void 0!==n?o[0]&&"object"==typeof o[0]&&o[0].hasOwnProperty(n)&&(i=o[0][n]):(void 0===t&&(t=s),s++,i=o[t-1]),"f"===r?i=parseFloat(i)||0:"d"===r&&(i=parseInt(i)||0),void 0!==e&&("f"===r?i=i.toFixed(e):"s"===r&&(i=i.substr(0,e))),null!=i?i:"")})}var f={locale_data:{messages:{"":{domain:"messages",lang:"en",plural_forms:"nplurals=2; plural=(n != 1);"}}},domain:"messages"};function e(t,n){this._key=t,this._instance=n}function h(t){var n,e,r;for(n in t=t||{},this.options={},f)this.options[n]=t[n]||f[n];for(n in this.options.locale_data)(e=this.options.locale_data[n][""]).plural_forms||e["Plural-Forms"]||e["plural-forms"]||(e.plural_forms=f.locale_data.messages.plural_forms);if(t.domain&&!this.options.locale_data[this.options.domain])throw new Error("Text domain set to non-existent domain: `"+t.domain+"`");this.textdomain(this.options.domain),this.sprintf=s,r=this.tannin=new i(this.options.locale_data,{contextDelimiter:h.context_delimiter,onMissingKey:t.missing_key_callback}),Object.defineProperty(this.options,"locale_data",{get:function(){return r.data},set:function(t){r.data=t}}),h.instances.push(this)}return e.prototype.onDomain=function(t){return this._domain=t,this},e.prototype.withContext=function(t){return this._context=t,this},e.prototype.ifPlural=function(t,n){return this._val=t,this._pkey=n,this},e.prototype.fetch=function(t){var n;return Array.isArray(t)||(t=Array.prototype.slice.call(arguments,0)),n=this._instance.dcnpgettext(this._domain,this._context,this._key,this._pkey,this._val),t.length?h.sprintf(n,t):n},h.instances=[],Object.defineProperty(h,"context_delimiter",{get:function(){return h.instances.length?h.instances[0].tannin.options.contextDelimiter:String.fromCharCode(4)},set:function(n){h.instances.forEach(function(t){t.tannin.options.contextDelimiter=n})}}),h.sprintf=s,(h.PF={}).compile=function(t){var n=new i({default:{"":{plural_forms:t}}});return function(t){return n.getPluralForm("default",t)}},h.prototype.textdomain=function(t){if(!t)return this._textdomain;this._textdomain=t},h.prototype.dcnpgettext=function(t,n,e,r,i){return r=r||e,t=t||this._textdomain,this.tannin.dcnpgettext(t,n,e,r,i)},h.prototype.translate=function(t){return new e(t,this)},h.prototype.gettext=function(t){return this.dcnpgettext.call(this,void 0,void 0,t)},h.prototype.dgettext=function(t,n){return this.dcnpgettext.call(this,t,void 0,n)},h.prototype.dcgettext=function(t,n){return this.dcnpgettext.call(this,t,void 0,n)},h.prototype.ngettext=function(t,n,e){return this.dcnpgettext.call(this,void 0,void 0,t,n,e)},h.prototype.dngettext=function(t,n,e,r){return this.dcnpgettext.call(this,t,void 0,n,e,r)},h.prototype.dcngettext=function(t,n,e,r){return this.dcnpgettext.call(this,t,void 0,n,e,r)},h.prototype.pgettext=function(t,n){return this.dcnpgettext.call(this,void 0,t,n)},h.prototype.dpgettext=function(t,n,e){return this.dcnpgettext.call(this,t,n,e)},h.prototype.dcpgettext=function(t,n,e){return this.dcnpgettext.call(this,t,n,e)},h.prototype.npgettext=function(t,n,e,r){return this.dcnpgettext.call(this,void 0,t,n,e,r)},h.prototype.dnpgettext=function(t,n,e,r,i){return this.dcnpgettext.call(this,t,n,e,r,i)},h}();;
/*
 * WordPress REST Proxy Request
 * Name:   WPCOM_Proxy_Request
 * Author: Dan Walmsley <dan.walmsley@automattic.com>, Beau Collins <beaucollins@gmail.com>
 *
 * A function that makes proxy requests (using window.postMessage) to the
 * WordPress.com REST api (https://public-api.wordpress.com/rest/v1/help)
 *
 * Usage:
 * 	window.WPCOM_Proxy_Request( path );
 * 	window.WPCOM_Proxy_Request( path, request );
 * 	window.WPCOM_Proxy_Request( request );
 *
 * Arguments:
 * 	path     : the REST URL path to request (will be appended to the rest base URL)
 * 	request  : request parameters: method (string), path (string), query (object), body (object)
 *
 * Returns
 * 	A promise()-like object whose callbacks accept the following arguments:
 * 		response : the JSON response for your request
 * 		statusCode : the HTTP statusCode for your request
 *
 * Example:
 * 	// For simple GET requests
 * 	window.WPCOM_Proxy_Request( '/me' ).done( function( response, statusCode ){
 * 		/// ...
 * 	} );
 *
 * 	// More Advanced GET request
 * 	window.WPCOM_Proxy_Request( {
 * 		path: '/sites/en.blog.wordpress.com/posts',
 * 		query: { number: 100 }
 * 	} );
 *
 * 	// POST request
 * 	window.WPCOM_Proxy_Request( {
 * 		method: 'POST',
 * 		path: '/sites/en.blog.wordpress.com/posts/9776/replies/new',
 * 		body: { content: 'This is a comment' }
 * 	} );
 */
(function(){
	// don't run this more than once per context
	if ( window.WPCOM_Proxy_Request) {
		return;
	}

	// polyfill for jQuery Deferred
	var Deferred = function() {
		this._done = [];
		this._fail = [];
	};

	Deferred.prototype = {
		execute: function(list, args){
			var i = list.length;

			// convert arguments to an array
			// so they can be sent to the
			// callbacks via the apply method
			args = Array.prototype.slice.call(args);

			while(i--) list[i].apply(null, args);
		},
		resolve: function(){
			this.execute(this._done, arguments);
		},
		reject: function(){
			this.execute(this._fail, arguments);
		},
		done: function(callback){
			this._done.push(callback);
			return this;
		},
		fail: function(callback){
			this._fail.push(callback);
			return this;
		},
		promise: function() {
			var x = {};
			x.done = this.done.bind( this );
			x.fail = this.fail.bind( this );
			return x;
		}
	};

	// polyfill for jQuery.extend
	var extend = function( out ) {
		out = out || {};

		for (var i = 1; i < arguments.length; i++) {
			if (!arguments[i])
				continue;

			for (var key in arguments[i]) {
				if (arguments[i].hasOwnProperty(key))
					out[key] = arguments[i][key];
			}
		}

		return out;
	}

	var proxy,
	origin         = window.location.protocol + '//' + window.location.hostname,
	proxyOrigin    = 'https://public-api.wordpress.com',

	ready          = false,
	supported      = true, // assume window.postMessage is supported
	usingPM        = false, // If we don't have window.postMessage, postmessage.js may be available
	structuredData = true, // supports passing of structured data

	bufferedOps    = [],   // store requests while we wait for the proxy iframe to initialize

	// Store `Deferred` objects for each pending request.
	deferreds      = {},

	// Store `this` context objects for each pending request, if given.
	callbackContexts = {},

	/**
	 * Firefox apparently doesn't like sending `File` instances cross-domain.
	 * It results in a "DataCloneError: The object could not be cloned." error.
	 * Apparently this is for "security purposes" but it's actually silly if that's
	 * the argument because we can just read the File manually into an ArrayBuffer
	 * and we can work around this "security restriction".
	 *
	 * See: https://bugzilla.mozilla.org/show_bug.cgi?id=722126#c8
	 */
	 hasFileSerializationBug = false,

	 // Can we pass structured data via postMessage or just strings?
	check = function( event ){
		structuredData = 'object' === typeof event.data;
		window.removeEventListener( 'message', check );
		buildProxy();
	},

	// Initialize the proxy iframe
	buildProxy = function() {
		// Start listening to messages
		if ( !usingPM ) {
			window.addEventListener( 'message', receive );
		} else {
			pm.bind( 'proxy', function( e ) { receive( e ); } );
		}

		proxy = document.createElement( 'iframe' );
		proxy.src = 'https://public-api.wordpress.com/wp-admin/rest-proxy/#' + origin;
		proxy.style.display = 'none';

		// Process any buffered API calls after the iframe proxy is ready
		proxy.addEventListener( 'load', function() {
			var request;
			ready = true;
			while ( request = bufferedOps.shift() ) {
				postRequest( request );
			}
		});

		var appendProxy = function() {
			document.body.appendChild( proxy );
		};

		// Bring it
		if (document.readyState === 'complete' || document.readyState !== 'loading') {
			appendProxy();
		} else {
			document.addEventListener('DOMContentLoaded', appendProxy);
		}
	},

	// Message event listener
	receive = function( e ){
		var data,
			deferred_id,
			deferred,
			context;

		if ( !usingPM ) {
			if ( e.origin !== proxyOrigin ) {
				return;
			}

			data = structuredData ? e.data : JSON.parse( e.data );
		} else {
			data = e;
		}

		if ( !data || !data.length ) {
			return;
		}

		deferred_id = data[ data.length - 1 ];

		if ( 'undefined' === typeof deferreds[deferred_id] ) {
			return;
		}

		deferred = deferreds[deferred_id];
		delete deferreds[deferred_id];

		context = callbackContexts[ deferred_id ];
		if ( context ) {
			// `resolveWith` takes args as an array.
			deferred.resolveWith.call( deferred, context, data.slice( 0, -1 ) );
			delete callbackContexts[ deferred_id ];
		} else {
			// `resolve` takes args as a list of parameters.
			deferred.resolve.apply( deferred, data.slice( 0, -1 ) );
		}
	},

	// Calls API
	perform = function() {
		var request = buildRequest.apply( null, arguments );

		postRequest( request );

		return deferreds[request.callback].promise();
	},

	// Buffers API request
	buffer = function() {
		var request = buildRequest.apply( null, arguments );

		bufferedOps.push( request );

		return deferreds[request.callback].promise();
	},

	// Submits the API request to the proxy iframe
	postRequest = function( request ) {
		var files = findFilesInRequest( request ),
	 		data = structuredData ? request : JSON.stringify( request );

		if ( hasFileSerializationBug && files.has_files ) {
			postAsArrayBuffer( request, files );
		} else {
			try {
				sendPostMessage( data );
			} catch( e ) {
				// were we trying to serialize a `File`?
				if ( files.has_files ) {

					// cache this check for the next API request
					hasFileSerializationBug = true;
					postAsArrayBuffer( request, files );
				} else {
					// not interested, rethrow
					throw e;
				}
			}
		}
	},

	sendPostMessage = function( data ) {
		if ( !usingPM ) {
			proxy.contentWindow.postMessage( data, proxyOrigin );
		} else if ( window.pm ) {
			pm( {
				data  : data,
				type  : 'proxy',
				target: proxy.contentWindow,
				url   : 'https://public-api.wordpress.com/wp-admin/rest-proxy/#' + origin,
				origin: proxyOrigin
			} );
		}
	},

	postAsArrayBuffer = function( request, files ) {
		if ( ! files.has_files )
			return;

		for(i=0; i<files.file_keys.length; ++i) {
			var reader = new FileReader(),
				key = request.formData[i][0],
				file = request.formData[i][1];

			reader.onload = function(e) {
				request.formData[i] = [ key, {
					fileContents: e.target.result,
					fileName : file.name,
					mimeType: file.type
				} ];

				var are_there_still_files = findFilesInRequest( request );
				if ( ! are_there_still_files.has_files ) {
					proxy.contentWindow.postMessage( request, proxyOrigin );
				}
			};

			reader.readAsArrayBuffer( file );
		}
	},

	findFilesInRequest = function( request ) {
		var files = {
			has_files : false,
			file_keys : []
		};

		if ( ! structuredData || ! request.formData || request.formData.length <= 0 )
			return files;

		for(i=0; i<request.formData.length; i++) {
			var arr = request.formData[i];
			var maybe_a_file = arr[1];
			if ( 'object' == typeof maybe_a_file && '[object File]' == Object.prototype.toString.call( maybe_a_file ) ) {
				files.has_files = true;
				files.file_keys.push( i );
			}
		}

		return files;
	},

	// Builds the postMessage request object
	buildRequest = function() {
		var args     = [].slice.call( arguments );
		    request  = args.pop(),
		    path     = args.pop(),
		    deferred = new Deferred(),
			deferred_id = Math.random();

		// @todo - remove this back-compat code
		if ( 'function' === typeof( request ) ) {
			deferred.done( request );
			request = path;
			path    = args.pop();
		}

		if ( 'string' === typeof( request ) ) {
			request = { path: request };
		}

		if ( path ) {
			request.path = path;
		}

		deferreds[deferred_id] = deferred;

		if ( request.context ) {
			callbackContexts[ deferred_id ] = request.context;
			// Trying to pass functions through `postMessage` is a bad time.
			request = extend( {}, request );
			delete request.context;
		}

		request.callback = deferred_id;
		request.supports_args = true; // supports receiving variable amount of arguments
		return request;
	};

	// Step 1: do we have postMessage? ( in IE8, typeof window.postMessage == 'object' )
	if ( [ 'function', 'object' ].indexOf( typeof window.postMessage ) >= 0 ) {
		// Step 2: Check if we can pass structured data or just strings
		window.addEventListener( 'message', check );
		window.postMessage( {}, origin );
	} else if ( window.pm ) {
		usingPM = true;
		// Step 2: We can always just used structured data.
		buildProxy();
	} else {
		supported = false;
	}

	window.WPCOM_Proxy_Request = function(){
		if ( !supported ) {
			throw( 'Browser does not support window.postMessage' );
		}

		if ( ready ) {
			// Make API request
			return perform.apply( null, arguments );
		} else {
			// Buffer API request
			return buffer.apply( null, arguments );
		}
	};

	window.WPCOM_Proxy_Rebuild = function() {
		if ( !ready )
			return;

		ready = false;
		proxy.parentNode.removeChild( proxy );

		buildProxy();
	};
})();
;
/*
 *  - wpLikes wraps all the proxied REST calls
 */
var wpLikes;

/*!
	https://gist.github.com/marlun78/2701678
	Underscore.js templates as a standalone implementation.
	JavaScript micro-templating, similar to John Resig's implementation.
	Underscore templates documentation: http://documentcloud.github.com/underscore/#template
	Modifyed by marlun78
*/
( function () {
	'use strict';

	// By default, Underscore uses ERB-style template delimiters, change the
	// following template settings to use alternative delimiters.
	var settings = {
		evaluate: /<%([\s\S]+?)%>/g,
		interpolate: /<%=([\s\S]+?)%>/g,
		escape: /<%-([\s\S]+?)%>/g,
	};

	// When customizing `templateSettings`, if you don't want to define an
	// interpolation, evaluation or escaping regex, we need one that is
	// guaranteed not to match.
	var noMatch = /.^/;

	// Certain characters need to be escaped so that they can be put into a
	// string literal.
	var escapes = {
		'\\': '\\',
		"'": "'",
		r: '\r',
		n: '\n',
		t: '\t',
		u2028: '\u2028',
		u2029: '\u2029',
	};

	for ( var p in escapes ) {
		escapes[ escapes[ p ] ] = p;
	}

	var escaper = /\\|'|\r|\n|\t|\u2028|\u2029/g;

	var tmpl = function ( text, data, objectName ) {
		settings.variable = objectName;

		// Compile the template source, taking care to escape characters that
		// cannot be included in a string literal and then unescape them in code
		// blocks.
		var source =
			"__p+='" +
			text
				.replace( escaper, function ( match ) {
					return '\\' + escapes[ match ];
				} )
				.replace( settings.escape || noMatch, function ( match, code ) {
					return "'+\nwindow.escapeHTML(" + unescape( code ) + ")+\n'";
				} )
				.replace( settings.interpolate || noMatch, function ( match, code ) {
					return "'+\n(" + unescape( code ) + ")+\n'";
				} )
				.replace( settings.evaluate || noMatch, function ( match, code ) {
					return "';\n" + unescape( code ) + "\n;__p+='";
				} ) +
			"';\n";

		// If a variable is not specified, place data values in local scope.
		if ( ! settings.variable ) {
			source = 'with(obj||{}){\n' + source + '}\n';
		}

		source =
			"var __p='';var print=function(){__p+=Array.prototype.join.call(arguments, '')};\n" +
			source +
			'return __p;\n';

		var render = new Function( settings.variable || 'obj', source );

		if ( data ) {
			return render( data );
		}

		var template = function ( templateData ) {
			return render.call( this, templateData );
		};

		// Provide the compiled function source as a convenience for build time
		// precompilation.
		template.source = 'function(' + ( settings.variable || 'obj' ) + '){\n' + source + '}';

		return template;
	};

	window.tmpl = tmpl;
} )();

/**
 * Escape function brought in from Underscore.js
 */
( function () {
	var escapeMap = {
		'&': '&amp;',
		'<': '&lt;',
		'>': '&gt;',
		'"': '&quot;',
		"'": '&#x27;',
		'`': '&#x60;',
	};

	var createEscaper = function ( map ) {
		var escaper = function ( match ) {
			return map[ match ];
		};

		var source = '(?:' + Object.keys( map ).join( '|' ) + ')';
		var testRegexp = RegExp( source );
		var replaceRegexp = RegExp( source, 'g' );
		return function ( string ) {
			string = string == null ? '' : '' + string;
			return testRegexp.test( string ) ? string.replace( replaceRegexp, escaper ) : string;
		};
	};

	window.escapeHTML = createEscaper( escapeMap );
} )();

( function () {
	var extWin;
	var i18n;

	wpLikes = {
		version: '',
		lang: 'en',
		langVersion: '',

		jsonAPIbase: 'https://public-api.wordpress.com/rest/v1',
		hasUpgradedProxy: false,
		isLoggedIn: false,
		masterReady: false,
		requests: {},
		me: false,
		askedMe: false,
		cache: [],
		adminBarEnabled: false,
		reblogsEnabled: false,

		batches: [],

		widgetDims: {},

		login_blog_id: false,
		login_post_id: false,
		login_comment_id: false,
		login_obj_id: false,
		login_domain: false,

		textStyles: {},
		linkStyles: {},
		adminBarStyles: {},

		likers: [],
		total: [],

		wpLikes: function () {
			var info = wpLikes.splitParams( location.hash.replace( /^#/, '' ) );
			if ( 'ver' in info ) {
				wpLikes.version = info.ver;
			}
		},

		resizeFrame: function ( name ) {
			var likeBox = window.parent.frames[ name ].document.querySelector( '.wpl-likebox' );
			var slim = this.hasClass( 'wpl-slim-likebox', likeBox );

			// Make sure slim likeboxes are actually inline-block - always
			if ( slim ) {
				var cssDisplay = likeBox.style.display;
				if ( cssDisplay !== 'inline-block' ) {
					likeBox.style.display = 'inline-block';
				}
			}

			var likeboxHeight = this.outerHeight( likeBox );
			var likeboxWidth = this.outerWidth( likeBox );

			wpLikes.postMessage(
				{
					action: 'resize',
					name: name,
					height: likeboxHeight,
					width: likeboxWidth,
				},
				parent,
				'resizeMessage'
			);
		},

		likePost: function ( blog_id, post_id, source, success, fail ) {
			return this.ajax( {
				type: 'POST',
				path: '/sites/' + blog_id + '/posts/' + post_id + '/likes/new',
				query: 'source=' + source,
				success: success,
				error: fail,
				blogId: blog_id,
				postId: post_id,
			} );
		},

		unlikePost: function ( blog_id, post_id, success, fail ) {
			return this.ajax( {
				type: 'POST',
				path: '/sites/' + blog_id + '/posts/' + post_id + '/likes/mine/delete',
				success: success,
				error: fail,
				blogId: blog_id,
				postId: post_id,
			} );
		},

		likeComment: function ( blog_id, comment_id, success, fail ) {
			if ( wpLikes.commentLikesKillSwitch ) {
				return;
			}
			return this.ajax( {
				type: 'POST',
				path: '/sites/' + blog_id + '/comments/' + comment_id + '/likes/new',
				success: success,
				error: fail,
				blogId: blog_id,
				commentId: comment_id,
			} );
		},

		unlikeComment: function ( blog_id, comment_id, success, fail ) {
			if ( wpLikes.commentLikesKillSwitch ) {
				return;
			}
			return this.ajax( {
				type: 'POST',
				path: '/sites/' + blog_id + '/comments/' + comment_id + '/likes/mine/delete',
				success: success,
				error: fail,
				blogId: blog_id,
				commentId: comment_id,
			} );
		},

		afterlikeFollow: function ( blog_id, success, fail ) {
			return this.ajax( {
				type: 'POST',
				path: '/sites/' + blog_id + '/follows/new',
				success: success,
				error: fail,
				blogId: blog_id,
			} );
		},

		getFollowingStatus: function ( blog_id, success, fail ) {
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/follows/mine',
				success: success,
				error: fail,
				blogId: blog_id,
			} );
		},

		getPost: function ( blog_id, post_id, success, fail ) {
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/posts/' + post_id,
				success: success,
				error: fail,
				blogId: blog_id,
				postId: post_id,
			} );
		},

		getPostLikeStatus: function ( blog_id, post_id, success, fail ) {
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/posts/' + post_id + '/likes/mine',
				success: success,
				error: fail,
				blogId: blog_id,
				postId: post_id,
			} );
		},

		getPostLikes: function ( blog_id, post_id, success, fail, fromCache ) {
			if ( typeof fromCache === 'undefined' ) {
				var info = wpLikes.splitParams( location.hash.replace( /^#/, '' ) );
				if ( 'ver' in info ) {
					wpLikes.version = info.ver;
				}
			}
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/posts/' + post_id + '/likes',
				success: success,
				error: fail,
				fromCache: fromCache,
				blogId: blog_id,
				postId: post_id,
			} );
		},

		getCommentLikeStatus: function ( blog_id, comment_id, success, fail ) {
			if ( wpLikes.commentLikesKillSwitch ) {
				return;
			}
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/comments/' + comment_id + '/likes/mine',
				success: success,
				error: fail,
				blogId: blog_id,
				commentId: comment_id,
			} );
		},

		getCommentLikes: function ( blog_id, comment_id, success, fail, fromCache ) {
			if ( wpLikes.commentLikesKillSwitch ) {
				return;
			}
			if ( typeof fromCache === 'undefined' ) {
				fromCache = true;
			}
			return this.ajax( {
				type: 'GET',
				path: '/sites/' + blog_id + '/comments/' + comment_id + '/likes',
				success: success,
				error: fail,
				fromCache: fromCache,
				blogId: blog_id,
				commentId: comment_id,
			} );
		},

		getMyInfo: function ( success, fail ) {
			if ( wpLikes.me ) {
				success( wpLikes.me, '/me' );
				return;
			}

			return this.ajax( {
				type: 'GET',
				path: '/me',
				success: success,
				error: fail,
			} );
		},

		splitParams: function ( queryString ) {
			var params = {};

			queryString.split( '&' ).forEach( function ( value ) {
				var pair = value.split( '=' );
				params[ pair[ 0 ] ] = decodeURIComponent( pair[ 1 ] );
			} );

			return params;
		},

		ajax: function ( options, batch ) {
			var request = {
				path: options.path,
				method: options.type,
				url: wpLikes.jsonAPIbase + options.path,
			};

			if ( batch && ! batch.batchFinished && options.path !== '/batch' ) {
				batch.batchWaiting.push( options );
				return;
			}

			if ( options.blogId && options.postId && options.path !== '/batch' ) {
				// Look for an initial batch for this post.
				wpLikes.batches.forEach( function ( initialBatch ) {
					if (
						initialBatch.blogId === options.blogId &&
						initialBatch.postId === options.postId &&
						! initialBatch.batchFinished
					) {
						initialBatch.batchWaiting.push( options );
						return;
					}
				} );
			}

			if ( options.blogId && options.commentId && options.path !== '/batch' ) {
				// Look for an initial batch for this comment.
				wpLikes.batches.forEach( function ( initialBatch ) {
					if (
						initialBatch.blogId === options.blogId &&
						initialBatch.commentId === options.commentId &&
						! initialBatch.batchFinished
					) {
						initialBatch.batchWaiting.push( options );
						return;
					}
				} );
			}

			if ( typeof options.fromCache === 'undefined' ) {
				options.fromCache = true;
			}

			if ( options.path in wpLikes.cache && options.fromCache ) {
				typeof options.success === 'function' &&
					options.success( wpLikes.cache[ options.path ], options.path );
				return;
			}

			if ( options.type.toLowerCase() === 'post' ) {
				request.body = options.data;
				request.query = options.query;
			} else {
				request.query = options.data;
			}

			var makeProxyCall = function () {
				return window.WPCOM_Proxy_Request( request, function ( response, statusCode ) {
					if ( statusCode === 200 ) {
						typeof options.success === 'function' && options.success( response, request.path );
					} else {
						typeof options.error === 'function' && options.error( statusCode, request.path );
					}
				} );
			};

			if ( wpLikes.hasUpgradedProxy ) {
				return makeProxyCall();
			}

			return window
				.WPCOM_Proxy_Request( { metaAPI: { accessAllUsersBlogs: true } } )
				.done( function () {
					wpLikes.hasUpgradedProxy = true;
					makeProxyCall();
				} );
		},

		/* postMessage */
		/* The messageType argument specifies the message type */
		/* Likes messages use likesMessage */
		/* An example of a message that doesn't use likesMessage is the resize request */
		postMessage: function ( message, target, messageType ) {
			if ( typeof message === 'string' ) {
				try {
					message = JSON.parse( message );
				} catch ( e ) {
					return;
				}
			}

			if ( typeof messageType === 'undefined' ) {
				messageType = 'likesMessage';
			}

			if ( target && typeof target.postMessage === 'function' ) {
				try {
					target.postMessage(
						JSON.stringify( {
							type: messageType,
							data: message,
						} ),
						'*'
					);
				} catch ( e ) {
					return;
				}
			}
		},

		openLoginWindow: function () {
			// Remove any lingering login window from any previous aborted login
			if ( extWin ) {
				if ( ! extWin.closed ) {
					extWin.close();
				}
				extWin = false;
			}

			// Remove any lingering cookie polling iframe from any previous aborted login
			var loginIframe = document.querySelector( '#wp-login-polling-iframe' );

			if ( loginIframe ) {
				loginIframe.parentNode.removeChild( loginIframe );
			}

			// Open new window for user to login in
			// We want to open it here (from the master iframe) so that our popup won't be blocked
			// (this keeps us in the context of the user's click)
			var authDomain = 'r-login.wordpress.com';

			if ( typeof wpLikes.login_domain === 'string' ) {
				authDomain = wpLikes.login_domain;
			}

			var url = 'https://' + authDomain + '/public.api/connect/?action=request&service=wordpress';

			if ( typeof wpLikes.login_domain === 'string' ) {
				url += '&domain=' + encodeURIComponent( wpLikes.login_domain );
			}

			if ( typeof wpLikes.login_blog_id !== 'undefined' ) {
				url += '&blog_id=' + encodeURIComponent( wpLikes.login_blog_id );
			}

			extWin = window.open(
				url,
				'likeconn',
				'status=0,toolbar=0,location=1,menubar=0,directories=0,resizable=1,scrollbars=1,height=660,width=500'
			);

			// Append cookie polling login iframe to original window to wait for user to finish logging in (or cancel)
			loginIframe = document.createElement( 'iframe' );
			loginIframe.id = 'wp-login-polling-iframe';
			loginIframe.src = 'https://r-login.wordpress.com/public.api/connect/?iframe=true';
			loginIframe.style.display = 'none';
			document.body.appendChild( loginIframe );
		},

		hasClass: function ( className, el ) {
			if ( el.classList ) {
				return el.classList.contains( className );
			}

			return new RegExp( '(^| )' + className + '( |$)', 'gi' ).test( el.className );
		},

		addClass: function ( className, el ) {
			if ( el.classList ) {
				el.classList.add( className );
			} else {
				el.className += ' ' + className;
			}
		},

		removeClass: function ( className, el ) {
			if ( el.classList ) {
				el.classList.remove( className );
			} else {
				el.className = el.className.replace(
					new RegExp( '(^|\\b)' + className.split( ' ' ).join( '|' ) + '(\\b|$)', 'gi' ),
					' '
				);
			}
		},

		outerWidth: function ( el ) {
			var width = el.offsetWidth;
			var style = getComputedStyle( el );
			if ( style ) {
				width += parseInt( style.marginLeft ) + parseInt( style.marginRight );
			}
			return width;
		},

		outerHeight: function ( el ) {
			var height = el.offsetHeight;
			var style = getComputedStyle( el );
			if ( style ) {
				height += parseInt( style.marginTop ) + parseInt( style.marginBottom );
			}
			return height;
		},

		triggerClick: function ( data, el ) {
			var event = new MouseEvent( 'click', {
				view: window,
				bubbles: true,
				cancelable: true,
			} );

			el.dispatchEvent( event );
		},

		readMessage: function ( msg ) {
			var event = msg.data;

			if ( typeof event.event === 'undefined' ) {
				return;
			} else if ( event.event === 'login' && event.success ) {
				// Remove any lingering login window
				if ( extWin ) {
					if ( ! extWin.closed ) {
						extWin.close();
					}
					extWin = false;
				}

				// Remove the cookie polling iframe that was added by openLoginWindow
				var pollingIframe = document.querySelector( '#wp-login-polling-iframe' );
				if ( pollingIframe ) {
					pollingIframe.parentNode.removeChild( pollingIframe );
				}

				// If the cookie or RLT token is available, then we must have auth'd successfully
				wpLikes.isLoggedIn = true;
				wpLikes.hasUpgradedProxy = false;
				window.WPCOM_Proxy_Rebuild();

				if ( wpLikes.login_post_id ) {
					wpLikes.getPostLikes(
						wpLikes.login_blog_id,
						wpLikes.login_post_id,
						function ( results ) {
							var slim = this.hasClass(
								'wpl-slim-likebox',
								window.parent.frames[
									'like-post-frame-' + wpLikes.login_obj_id
								].document.querySelector( '.wpl-likebox' )
							);
							wpLikes.updatePostFeedback(
								results,
								wpLikes.login_blog_id,
								wpLikes.login_post_id,
								slim,
								wpLikes.login_obj_id
							);

							if ( ! results.i_like ) {
								wpLikes.doLike(
									wpLikes.login_blog_id,
									wpLikes.login_post_id,
									wpLikes.login_obj_id
								);
							}

							var likeButton = window.parent.frames[
								'like-post-frame-' + wpLikes.login_obj_id
							].document.querySelector( '.wpl-button a.like, .wpl-button a.liked' );

							likeButton.onclick = function ( e ) {
								e.preventDefault();
								wpLikes.doLike(
									wpLikes.login_blog_id,
									wpLikes.login_post_id,
									wpLikes.login_obj_id
								);
							};
						}.bind( this ),
						function () {},
						false
					);
				}

				if ( wpLikes.login_comment_id && ! wpLikes.commentLikesKillSwitch ) {
					wpLikes.getCommentLikes(
						wpLikes.login_blog_id,
						wpLikes.login_comment_id,
						function ( results ) {
							var links = window.parent.frames[
								'like-comment-frame-' + wpLikes.login_obj_id
							].document.querySelectorAll( 'a.comment-like-link' );

							if ( links.length === 0 ) {
								return;
							}

							links.forEach(
								function ( link ) {
									this.addClass( 'loading', link );

									if ( ! results.i_like ) {
										wpLikes.likeComment(
											wpLikes.login_blog_id,
											wpLikes.login_comment_id,
											function () {
												link.parent().removeClass( 'comment-not-liked' );
												link.parent().addClass( 'comment-liked' );

												var feedback = getCommentLikeFeedback( true, results.found + 1 );
												link.textContent = feedback;
											}.bind( this )
										);
									} else {
										link.parent().removeClass( 'comment-not-liked' );
										link.parent().addClass( 'comment-liked' );

										var feedback = getCommentLikeFeedback( true, results.found );
										link.textContent = feedback;
									}

									link.removeClass( 'loading' );
								}.bind( this )
							);
						}.bind( this ),
						function () {},
						false
					);
				}
			} else if ( event.event === 'injectStyles' ) {
				wpLikes.textStyles = event.textStyles;
				wpLikes.linkStyles = event.linkStyles;

				if ( wpLikes.adminBarEnabled ) {
					wpLikes.adminBarStyles = event.adminBarStyles;
				}
			} else if ( event.event === 'initialBatch' ) {
				wpLikes.initialBatch( event.requests );
			} else if ( event.event === 'adminBarEnabled' ) {
				wpLikes.adminBarEnabled = true;
			} else if ( event.event === 'reblogsEnabled' ) {
				wpLikes.reblogsEnabled = true;
			} else if ( event.event === 'loadLikeWidget' ) {
				if ( window.parent.frames[ event.name ] !== undefined ) {
					var info = wpLikes.splitParams(
						window.parent.frames[ event.name ].location.hash.replace( /^#/, '' )
					);
					var path;
					var request;

					if ( info.obj_id && info.obj_id.match( /[^\w-]/ ) ) {
						return;
					}

					// This gets used for reverse remote login, we need to pass
					// the target login domain all the way down to the login
					// form.
					try {
						if ( typeof event.domain === 'string' ) {
							wpLikes.login_domain = event.domain;
						}
					} catch ( error ) {}

					if ( info.blog_id && info.post_id && info.origin ) {
						path = '/sites/' + info.blog_id + '/posts/' + info.post_id + '/likes';
						if ( typeof info.slim === 'undefined' ) {
							info.slim = false;
						}

						request = {
							type: 'post',
							blog_id: info.blog_id,
							post_id: info.post_id,
							obj_id: info.obj_id,
							width: event.width,
							slim: info.slim,
						};
						wpLikes.requests[ path ] = request;
						wpLikes.getPostLikes( info.blog_id, info.post_id, wpLikes.displayWidget );
					} else if (
						info.blog_id &&
						info.comment_id &&
						info.origin &&
						! wpLikes.commentLikesKillSwitch
					) {
						path = '/sites/' + info.blog_id + '/comments/' + info.comment_id + '/likes';
						request = {
							type: 'comment',
							blog_id: info.blog_id,
							comment_id: info.comment_id,
							obj_id: info.obj_id,
							width: event.width,
						};
						wpLikes.requests[ path ] = request;

						wpLikes.getCommentLikes( info.blog_id, info.comment_id, wpLikes.displayWidget );
					}
				}
			} else if ( event.event === 'didReblog' && 'obj_id' in event ) {
				// Update the display of the button
				var wplbuttonlink = window.parent.frames[
					'like-post-frame-' + event.obj_id
				].document.querySelector( '.wpl-button a.reblog' );
				this.removeClass( 'reblog', wplbuttonlink );
				this.addClass( 'reblogged', wplbuttonlink );

				wplbuttonlink.innerHTML = '<span>' + i18n.translate( 'Reblogged' ).fetch() + '</span> ';
				wplbuttonlink.style.display = null;
			}
		},

		handlePromptClicks: function ( blog_id, post_id, obj_id ) {
			var $doc = window.parent.frames[ 'like-post-frame-' + obj_id ].document;

			var commentLink = $doc.querySelector( '.wpl-comment > a' );
			if ( commentLink ) {
				commentLink.onclick = function () {
					// Bump stat and redirect
					new Image().src =
						document.location.protocol +
						'//pixel.wp.com/b.gif?v=wpcom-no-pv&x_follow-click-prompt=comment-prompt&baba=' +
						Math.random();
				};
			}

			var followLink = $doc.querySelector( '.wpl-follow a' );
			if ( followLink ) {
				this.setCss( followLink, wpLikes.linkStyles );
				followLink.onclick = function ( e ) {
					e.preventDefault();
					wpLikes.afterlikeFollow( blog_id );
					$doc.querySelector( '.wpl-follow' ).innerHTML = i18n.translate( 'Following.' ).fetch();
					return false;
				};
			}
		},

		siblings: function ( selector, el ) {
			return Array.prototype.filter.call( el.parentNode.children, function ( child ) {
				var matches = el.parentNode.querySelectorAll( selector );
				var i = matches.length;
				while ( --i >= 0 && matches.item( i ) !== child ) {
					// Do nothing.
				}
				return child !== el && i > -1;
			} );
		},

		doLike: function ( blog_id, post_id, obj_id ) {
			function postLikePrompts() {
				wpLikes.getFollowingStatus(
					blog_id,
					function ( result ) {
						var $doc = window.parent.frames[ 'like-post-frame-' + obj_id ].document;
						if ( $doc.offsetWidth < 350 ) {
							// If the contentWidth isn't wide enough, the prompts won't display properly.
							return;
						}
						if ( ! result.is_following ) {
							var followEl = $doc.querySelector( '.wpl-follow' );
							if ( followEl ) {
								followEl.style.display = null;
							}
							this.setCss( followEl.querySelector( 'a' ), wpLikes.linkStyles );
							wpLikes.handlePromptClicks( blog_id, post_id, obj_id );
						} else {
							wpLikes.getPost(
								blog_id,
								post_id,
								function ( post ) {
									if ( post.comments_open ) {
										var commentLink = $doc.querySelector( '.wpl-comment a' );
										if ( commentLink ) {
											this.setCss( commentLink, wpLikes.linkStyles );
											commentLink.href = post.URL + '#respond';
										}

										var comment = $doc.querySelector( '.wpl-comment' );
										if ( comment ) {
											comment.style.display = null;
										}
										wpLikes.handlePromptClicks( blog_id, post_id, obj_id );
									}
								}.bind( this )
							);
						}
					}.bind( this )
				);
			}

			if ( ! wpLikes.isLoggedIn ) {
				wpLikes.login_blog_id = blog_id;
				wpLikes.login_post_id = post_id;
				wpLikes.login_obj_id = obj_id;

				new Image().src =
					document.location.protocol +
					'//pixel.wp.com/b.gif?v=wpcom-no-pv&x_likes=loggedout_like_click&baba=' +
					Math.random();

				// User isn't logged in, so we should get them to do that.
				wpLikes.openLoginWindow();
				return;
			}

			/**
			 * After Like Prompts
			 * After liking a post, we show a "follow this blog"? prompt to get readers to subscribe to the blog.
			 * or a "comment on this post?" prompt if they are already following
			 */
			var followPromptText =
				' <span class="wpl-follow" style="display:none;"><a href="#">' +
				i18n.translate( 'Follow this Blog?' ).fetch() +
				'</a></span>';
			var commentPromptText =
				' <span class="wpl-comment" style="display:none;"><a href="#" target="_parent">' +
				i18n.translate( 'Comment on this post?' ).fetch() +
				'</a></span>';

			var wplbuttonlink = window.parent.frames[
				'like-post-frame-' + obj_id
			].document.querySelector( '.wpl-button a.like, .wpl-button a.liked' );
			var wplbutton = wplbuttonlink.parentNode;
			var wplcount = this.siblings( '.wpl-count', wplbutton )[ 0 ];
			var wplavatars = this.siblings( '.wpl-avatars', wplbutton );
			var wplcounttext = wplcount.querySelector( '.wpl-count-text' );

			var likeText = '';
			var countEl;
			var count;

			if ( this.hasClass( 'like', wplbuttonlink ) ) {
				var slim = this.hasClass( 'wpl-slim-likebox', wplbutton.parentNode );

				// Figure out what the feedback text should say
				if (
					wplcounttext &&
					i18n.translate( 'Be the first to like this.' ).fetch() === wplcounttext.innerHTML
				) {
					likeText =
						'<span class="wpl-count-text">' +
						i18n.translate( 'You like this.' ).fetch() +
						'</span>' +
						followPromptText +
						commentPromptText;
				} else if (
					wplcounttext &&
					i18n.translate( 'One blogger likes this.' ).fetch() === wplcounttext.innerHTML
				) {
					likeText =
						'<span class="wpl-count-text">' +
						i18n.translate( 'You and one other blogger like this.' ).fetch() +
						'</span>' +
						followPromptText +
						commentPromptText;
				} else {
					countEl = wplcount.querySelector( '.wpl-count-number' );
					if ( countEl ) {
						count = countEl.textContent;
						likeText =
							'<span class="wpl-count-text">' +
							i18n.sprintf(
								i18n
									.translate(
										'You and <a href="%1$s" id="%2$s">%3$s other bloggers</a> like this.'
									)
									.fetch(),
								'#',
								'other-gravatars',
								'<span class="wpl-count-number">' + count + '</span>'
							) +
							'</span>' +
							followPromptText +
							commentPromptText;
					}
				}

				// Update the display of the button
				this.removeClass( 'like', wplbuttonlink );
				this.addClass( 'liked', wplbuttonlink );
				this.removeClass( 'like', wplbutton );
				this.addClass( 'liked', wplbutton );

				if ( ! slim ) {
					wplcount.innerHTML = likeText;
					wplcount.style.display = null;
					this.setCss(
						window.parent.frames[ 'like-post-frame-' + obj_id ].document.body.querySelector(
							'.wpl-count a'
						),
						wpLikes.linkStyles
					);
				}

				postLikePrompts.bind( this ).call();

				if ( ! slim ) {
					wpLikes.getMyInfo(
						function ( me ) {
							me.css_class = 'wp-liker-me';

							wpLikes.likers[ blog_id + '-' + post_id ].unshift( me );

							if ( ! wplbutton.parentNode.querySelectorAll( '.wp-liker-me' ).length ) {
								if ( ! wplavatars.length ) {
									wplbutton.insertAdjacentHTML(
										'afterend',
										'<ul class="wpl-avatars">' +
											'<li class="wp-liker-me">' +
											'<a title="' +
											window.escapeHTML( me.display_name ) +
											'" href="' +
											window.escapeHTML( me.profile_URL ) +
											'" class="wpl-liker" rel="nofollow" target="_parent">' +
											'<img src="' +
											window.escapeHTML( me.avatar_URL ) +
											'" alt="' +
											window.escapeHTML( i18n.translate( 'My Grav.' ).fetch() ) +
											'" width="30" height="30" />' +
											'</a>' +
											'</li>' +
											'</ul>'
									);
								} else {
									wplavatars[ 0 ].insertAdjacentHTML(
										'afterbegin',
										'<li class="wp-liker-me">' +
											'<a title="' +
											window.escapeHTML( me.display_name ) +
											'" href="' +
											window.escapeHTML( me.profile_URL ) +
											'" class="wpl-liker" rel="nofollow" target="_parent">' +
											'<img src="' +
											window.escapeHTML( me.avatar_URL ) +
											'" alt="' +
											window.escapeHTML( i18n.translate( 'My Grav.' ).fetch() ) +
											'" width="30" height="30" style="padding-right: 3px;" />' +
											'</a>' +
											'</li>'
									);
								}
							}
						}.bind( this )
					);
				}

				wplbuttonlink.innerHTML = '<span>' + i18n.translate( 'Liked' ).fetch() + '</span> ';

				// Ask parent to resize the frame
				wpLikes.resizeFrame( 'like-post-frame-' + obj_id );

				if ( wpLikes.adminBarEnabled ) {
					var widgetDocument = window.parent.frames[ 'admin-bar-likes-widget' ].document;
					widgetDocument.querySelector( 'a.like' ).textContent = i18n.translate( 'Liked' ).fetch();
				}

				// ANNNNND like it
				if ( typeof arguments[ 3 ] !== 'undefined' && arguments[ 3 ] === 'adminbar' ) {
					wpLikes.likePost( blog_id, post_id, 'adminbar' );
				} else {
					wpLikes.likePost( blog_id, post_id, 'post_flair' );
				}
			} else if ( this.hasClass( 'liked', wplbuttonlink ) ) {
				this.removeClass( 'liked', wplbuttonlink );
				this.addClass( 'like', wplbuttonlink );

				this.removeClass( 'liked', wplbutton );
				this.addClass( 'like', wplbutton );

				if (
					wplcounttext &&
					i18n.translate( 'You like this.' ).fetch() === wplcounttext.innerHTML
				) {
					likeText =
						'<span class="wpl-count-text">' +
						i18n.translate( 'Be the first to like this.' ).fetch() +
						'</span>';
				} else if (
					wplcounttext &&
					i18n.translate( 'You and one other blogger like this.' ).fetch() ===
						wplcounttext.innerHTML
				) {
					likeText =
						'<span class="wpl-count-text">' +
						i18n.translate( 'One blogger likes this.' ).fetch() +
						'</span>';
				} else {
					countEl = wplcount.querySelector( '.wpl-count-number' );
					if ( countEl ) {
						count = countEl.textContent;
						likeText =
							'<span class="wpl-count-text">' +
							i18n.sprintf(
								i18n.translate( '<a href="%1$s" id="%2$s">%3$s bloggers</a> like this.' ).fetch(),
								'#',
								'other-gravatars',
								'<span class="wpl-count-number">' + count + '</span>'
							) +
							'</span>';
					}
				}

				wplcount.innerHTML = likeText;
				wplcount.style.display = null;
				this.setCss(
					window.parent.frames[ 'like-post-frame-' + obj_id ].document.body.querySelector(
						'.wpl-count a'
					),
					wpLikes.linkStyles
				);

				wpLikes.likers[ blog_id + '-' + post_id ].shift();

				var wpLikerMe = wplbutton.parentNode.querySelector( 'li.wp-liker-me' );
				if ( wpLikerMe ) {
					wpLikerMe.parentNode.removeChild( wpLikerMe );
				}

				wplbuttonlink.innerHTML = '<span>' + i18n.translate( 'Like' ).fetch() + '</span>';

				// Ask parent to resize the frames
				wpLikes.resizeFrame( 'like-post-frame-' + obj_id );

				if ( wpLikes.adminBarEnabled ) {
					window.parent.frames[ 'admin-bar-likes-widget' ].document.querySelector(
						'a.like'
					).textContent = i18n.translate( 'Like' ).fetch();
				}

				// ANNNNND unlike it
				wpLikes.unlikePost( blog_id, post_id );
			}
		},

		// replacement for jQuery(el).css({some: style})
		setCss: function ( el, styles ) {
			if ( ! el ) {
				return;
			}

			Object.keys( styles ).forEach( function ( key ) {
				el.style[ key ] = styles[ key ];
			} );
		},

		updatePostFeedback: function ( likes, blog_id, post_id, slim, obj_id ) {
			if ( ! obj_id ) {
				obj_id = blog_id + '-' + post_id;
			}

			var isLiked = likes.i_like;
			var canLike = likes.can_like;
			var label = '';
			var css_state = '';
			var feedback = '';

			var canReblog = false;
			var canUserReblog = false;
			var reblog_css_state = 'reblog';
			var reblog_feedback_no_html = i18n.translate( 'Reblog this post on your main site.' ).fetch();
			var reblog_label = i18n.translate( 'Reblog' ).fetch();
			var reblog_path = '/sites/' + blog_id + '/posts/' + post_id + '/reblogs/mine';

			if ( ! this.reblogsEnabled ) {
				canReblog = false;
			} else if ( reblog_path in this.cache ) {
				if ( this.cache[ reblog_path ].can_reblog ) {
					canReblog = true;
				}
				if ( this.cache[ reblog_path ].can_user_reblog ) {
					canUserReblog = true;
				}
				if ( this.cache[ reblog_path ].is_reblogged ) {
					reblog_css_state = 'reblogged';
					reblog_label = i18n.translate( 'Reblogged' ).fetch();
				}
			}

			// Figure out the button label and css class for this button
			if ( isLiked ) {
				label = i18n.translate( 'Liked' ).fetch();
				css_state = 'liked';
			} else {
				label = i18n.translate( 'Like' ).fetch();
				css_state = 'like';
			}

			var hasLikes = true;
			var likers;

			// Figure out the inital feedback text
			if ( likes.found === 0 ) {
				hasLikes = false;
				feedback = i18n.translate( 'Be the first to like this.' ).fetch();
			} else if ( likes.found === 1 ) {
				if ( isLiked ) {
					feedback = i18n.translate( 'You like this.' ).fetch();
				} else {
					feedback = i18n.translate( 'One blogger likes this.' ).fetch();
				}
			} else if ( isLiked ) {
				var user_count = likes.found - 1;
				if ( user_count !== 1 ) {
					feedback = i18n.sprintf(
						i18n
							.translate( 'You and <a href="%1$s" id="%2$s">%3$s other bloggers</a> like this.' )
							.fetch(),
						'#',
						'other-gravatars',
						'<span class="wpl-count-number">' + user_count + '</span>'
					);
				} else {
					feedback = i18n.translate( 'You and one other blogger like this.' ).fetch();
				}
			} else {
				feedback = i18n.sprintf(
					i18n.translate( '<a href="%1$s" id="%2$s">%3$s bloggers</a> like this.' ).fetch(),
					'#',
					'other-gravatars',
					'<span class="wpl-count-number">' + likes.found + '</span>'
				);
			}

			feedback = '<span class="wpl-count-text">' + feedback + '</span>';

			function createPostLikeTemplate() {
				var template;
				var cacheBuster;
				var widgetDocument;

				if ( wpLikes.version !== '' ) {
					cacheBuster = '?ver=' + wpLikes.version;
				}

				if ( wpLikes.adminBarEnabled ) {
					template = window.tmpl( document.querySelector( '#admin-bar-likes' ).innerHTML );
					widgetDocument = window.parent.frames[ 'admin-bar-likes-widget' ].document;

					widgetDocument.querySelector( '#target' ).innerHTML = template( {
						label: label,
						isRtl: wpLikes.adminBarStyles.isRtl,
					} );

					var style = document.createElement( 'link' );
					style.setAttribute( 'type', 'text/css' );
					style.setAttribute( 'rel', 'stylesheet' );
					style.setAttribute(
						'href',
						'//s0.wp.com/wp-includes/css/admin-bar.min.css' + cacheBuster
					);
					widgetDocument.querySelector( 'head' ).appendChild( style );

					if ( wpLikes.adminBarStyles.isRtl ) {
						style.setAttribute(
							'href',
							'//s0.wp.com/wp-content/mu-plugins/admin-bar/rtl/wpcom-admin-bar-rtl.css' +
								cacheBuster
						);
					} else {
						style.setAttribute(
							'href',
							'//s0.wp.com/wp-content/mu-plugins/admin-bar/wpcom-admin-bar.css' + cacheBuster
						);
					}
					widgetDocument.querySelector( 'head' ).appendChild( style );
				}

				if ( slim ) {
					template = window.tmpl( document.querySelector( '#slim-likes' ).innerHTML );
				} else {
					template = window.tmpl( document.querySelector( '#post-likes' ).innerHTML );
				}
				widgetDocument = window.parent.frames[ 'like-post-frame-' + obj_id ].document;
				widgetDocument.querySelector( '#target' ).innerHTML = template( {
					likers: likers && likers.slice( 0, 20 ),
					css_state: css_state,
					label: label,
					feedback: feedback,
					feedback_no_html: feedback.replace( /(<.*?>)/gi, '' ),
					hasLikes: hasLikes,
					reblog_css_state: reblog_css_state,
					reblog_feedback_no_html: reblog_feedback_no_html,
					canReblog: canReblog,
					canUserReblog: canUserReblog,
					canLike: canLike,
					reblog_label: reblog_label,
				} );

				this.setCss( widgetDocument.body, wpLikes.textStyles );
				this.setCss( widgetDocument.body.querySelector( '.wpl-count a' ), wpLikes.linkStyles );

				if ( wpLikes.textStyles.direction === 'rtl' ) {
					this.addClass( 'rtl', widgetDocument.body );
				}

				wpLikes.postMessage(
					{
						event: 'showLikeWidget',
						id: 'like-post-wrapper-' + obj_id,
						blog_id: blog_id,
						post_id: post_id,
						obj_id: obj_id,
					},
					parent
				);

				if ( wpLikes.adminBarEnabled ) {
					widgetDocument = window.parent.frames[ 'admin-bar-likes-widget' ].document;
					widgetDocument.querySelector( 'a.like' ).click(
						function () {
							var doc = window.parent.frames[ 'like-post-frame-' + obj_id ].document;
							this.triggerClick(
								{ source: 'adminbar' },
								doc.querySelector( '.wpl-button > a.like, .wpl-button > a.liked' )
							);
						}.bind( this )
					);
				}
			}

			// Build the likers array
			likers = likes.likes;
			if ( likers.length > 0 ) {
				var max_remove = likers.length - 90;
				for ( var i = likers.length - 1; i >= 0 && max_remove > 0; i-- ) {
					if (
						likers[ i ].default_avatar &&
						( ! wpLikes.me || wpLikes.me.ID !== likers[ i ].ID )
					) {
						likers.splice( i, 1 );
						max_remove--;
					}
				}
			}

			if ( wpLikes.me ) {
				wpLikes.isLoggedIn = true;

				for ( var j = 0; j < likers.length; j++ ) {
					if ( likers[ j ].ID === wpLikes.me.ID ) {
						likers[ j ].css_class = 'wp-liker-me';
						// Move this user's avatar to the front of the face pile
						likers.unshift( likers.splice( j, 1 )[ 0 ] );
						break;
					}
				}
			}

			wpLikes.likers[ blog_id + '-' + post_id ] = likers;
			wpLikes.total[ blog_id + '-' + post_id ] = likes.found;

			createPostLikeTemplate.bind( this ).call();
		},

		initialBatch: function ( requests ) {
			var info;
			var request;
			var path;

			var batch = {
				queue: [],
				batchFinished: false,
				batchWaiting: [],
				blogId: null,
				postId: null,
				commentId: null,
			};

			if ( ! wpLikes.me && ! wpLikes.askedMe ) {
				batch.queue.push( '/me' );
				wpLikes.askedMe = true;
			}

			for ( var i = 0; i < requests.length; i++ ) {
				info = requests[ i ];

				if ( info.obj_id && info.obj_id.match( /[^\w-]/ ) ) {
					continue;
				}

				if ( info.blog_id && info.post_id ) {
					batch.blogId = info.blog_id;
					batch.postId = info.post_id;

					path = '/sites/' + info.blog_id + '/posts/' + info.post_id + '/likes';
					request = {
						type: 'post',
						blog_id: info.blog_id,
						post_id: info.post_id,
						obj_id: info.obj_id,
						width: info.width,
					};
					wpLikes.requests[ path ] = request;
					batch.queue.push( path );
					path = '/sites/' + info.blog_id + '/posts/' + info.post_id + '/reblogs/mine';
					request = {
						blog_id: info.blog_id,
						post_id: info.post_id,
					};
					wpLikes.requests[ path ] = request;
					batch.queue.push( path );
				} else if ( info.blog_id && info.comment_id && ! wpLikes.commentLikesKillSwitch ) {
					batch.blogId = info.blog_id;
					batch.commentId = info.comment_id;

					path = '/sites/' + info.blog_id + '/comments/' + info.comment_id + '/likes';
					request = {
						type: 'comment',
						blog_id: info.blog_id,
						comment_id: info.comment_id,
						width: info.width,
					};
					wpLikes.requests[ path ] = request;
					batch.queue.push( path );
				}
			}

			var batchRequest = {
				path: '/batch',
				type: 'GET',
				url: 'https://public-api.wordpress.com/rest/v1/batch',
				data: '',
				success: function ( response ) {
					for ( var responsePath in response ) {
						if ( ! response[ responsePath ].error_data && ! response[ responsePath ].errors ) {
							if ( responsePath === '/me' ) {
								wpLikes.me = response[ responsePath ];
							} else {
								wpLikes.cache[ responsePath ] = response[ responsePath ];
							}
						}
					}

					batch.batchFinished = true;
					for ( var item in batch.batchWaiting ) {
						wpLikes.ajax( batch.batchWaiting[ item ], batch );
					}
				},
				error: function () {
					batch.batchFinished = true;
					for ( var item in batch.batchWaiting ) {
						wpLikes.ajax( batch.batchWaiting[ item ], batch );
					}
				},
			};

			var amp = '';
			for ( var j = 0; j < batch.queue.length; j++ ) {
				if ( j > 0 ) {
					amp = '&';
				}
				batchRequest.data += amp + 'urls[]=' + batch.queue[ j ];
			}

			wpLikes.batches.push( batch );
			wpLikes.ajax( batchRequest );
		},
	};

	// wpLikes.displayWidget is called when the ajax request for post or comment likes completes successfully
	// it is used to display the widget with the likes data
	wpLikes.displayWidget = function ( response, path ) {
		/**
		 * Translation
		 */
		var info = wpLikes.splitParams( location.hash.replace( /^#/, '' ) );
		if ( info.lang ) {
			wpLikes.lang = info.lang;
			wpLikes.langVersion = info.lang_ver ? info.lang_ver : info.ver;
		}

		var load_default = true;
		var json_locale_data;
		if ( wpLikes.lang !== 'en' ) {
			var xhr = new XMLHttpRequest();
			xhr.open(
				'GET',
				'/languages/' + wpLikes.lang + '-v1.1.json' + '?ver=' + wpLikes.langVersion,
				false
			);
			xhr.onload = function () {
				if ( xhr.status === 200 ) {
					var json = JSON.parse( xhr.responseText );
					json_locale_data = json;
					load_default = false;
				}
			};
			xhr.send();
		}
		if ( json_locale_data === null ) {
			load_default = true;
		}

		if ( load_default ) {
			json_locale_data = {
				'': {
					domain: 'messages',
					lang: wpLikes.lang,
					'plural-forms': 'nplurals=2; plural=(n !== 1);',
				},
			};
		}

		i18n = new window.Jed( { locale_data: { messages: json_locale_data }, domain: 'messages' } );

		if ( path in wpLikes.requests ) {
			if ( wpLikes.requests[ path ].type === 'post' ) {
				displayPostLikeWidget(
					wpLikes.requests[ path ].blog_id,
					wpLikes.requests[ path ].post_id,
					wpLikes.requests[ path ].width,
					wpLikes.requests[ path ].slim,
					response,
					wpLikes.requests[ path ].obj_id
				);
			}
			if ( wpLikes.requests[ path ].type === 'comment' ) {
				displayCommentLikeWidget(
					wpLikes.requests[ path ].blog_id,
					wpLikes.requests[ path ].comment_id,
					wpLikes.requests[ path ].width,
					response,
					wpLikes.requests[ path ].obj_id
				);
			}
		}
	};

	// displayPostLikeWidget is called when a post's likes data arrives via ajax (see wpLikes.displayWidget i.e. the ajax success handler)
	function displayPostLikeWidget( blog_id, post_id, width, slim, result, obj_id ) {
		if ( ! obj_id ) {
			obj_id = blog_id + '-' + post_id;
		}

		wpLikes.updatePostFeedback( result, blog_id, post_id, slim, obj_id );

		var likePostFrameDoc = window.parent.frames[ 'like-post-frame-' + obj_id ].document;

		function hasClass( className, el ) {
			if ( el.classList ) {
				return el.classList.contains( className );
			}
			return new RegExp( '(^| )' + className + '( |$)', 'gi' ).test( el.className );
		}

		// Add a click handler to handle the liking action
		var likeButton = likePostFrameDoc.querySelector( '.wpl-button a.like, .wpl-button a.liked' );
		if ( likeButton ) {
			likeButton.onclick = function ( e ) {
				e.preventDefault();
				var source = 'post_flair';
				if ( typeof arguments[ 1 ] !== 'undefined' && arguments[ 1 ].source === 'adminbar' ) {
					source = 'adminbar';
				}
				wpLikes.doLike( blog_id, post_id, obj_id, source );
			}.bind( this );
		}

		// Add a reblog handler to handle the reblog action
		var reblogButton = likePostFrameDoc.querySelector( '.wpl-button a.reblog' );
		if ( reblogButton ) {
			reblogButton.onclick = function ( e ) {
				e.preventDefault();
				if ( hasClass( 'reblog', reblogButton ) ) {
					wpLikes.postMessage( { event: 'clickReblogFlair', obj_id: obj_id, post_id: post_id }, window.parent );
				}
			}.bind( this );
		}

		if ( ! slim ) {
			// Handle the "n other bloggers" list
			var otherGravatars = likePostFrameDoc.querySelector( 'a#other-gravatars' );
			if ( otherGravatars ) {
				otherGravatars.onclick = function ( e ) {
					e.preventDefault();
					var $avatars = window.parent.frames[ 'like-post-frame-' + obj_id ].document.querySelector(
						'.wpl-avatars'
					);

					var likersToSend = 90;
					var myArrayId = -1;
					for (
						var i = 0;
						i < likersToSend && i < wpLikes.likers[ blog_id + '-' + post_id ].length;
						i++
					) {
						if ( wpLikes.likers[ blog_id + '-' + post_id ][ i ].css_class === 'wpl-liker-me' ) {
							myArrayId = i;
						}
						wpLikes.likers[ blog_id + '-' + post_id ][ i ].css_class = 'wpl-liker';
					}

					// Send a message to the likes master iframe (jetpack-likes.php) to update this frame's gravatars (likers)
					var data = {
						event: 'showOtherGravatars',
						likers: wpLikes.likers[ blog_id + '-' + post_id ].slice( 0, likersToSend ),
						total: wpLikes.total[ blog_id + '-' + post_id ],
						parent: 'like-post-frame-' + obj_id,
						width: $avatars.offsetWidth,
						position: {
							top: $avatars.offsetTop,
							left: $avatars.offsetLeft,
						},
					};

					wpLikes.postMessage( data, window.parent );

					if ( myArrayId >= 0 ) {
						wpLikes.likers[ blog_id + '-' + post_id ][ myArrayId ].css_class = 'wpl-liker-me';
					}
				};
			}
		}

		/**
		 * End Prompts
		 */
	}

	function getCommentLikeFeedback( isLiked, found ) {
		var feedback = '';
		var likers = '';
		if ( found === 0 ) {
			feedback = i18n.translate( 'Like' ).fetch();
		} else if ( found === 1 ) {
			if ( isLiked ) {
				feedback = i18n.translate( 'Liked by you' ).fetch();
			} else {
				likers = i18n.translate( '%d person' ).fetch( 1 );
				feedback = i18n.translate( 'Liked by %s' ).fetch( likers );
			}
		} else if ( isLiked ) {
			var userCount = found - 1;
			if ( userCount !== 1 ) {
				likers = i18n.translate( '%d other people' ).fetch( userCount );
				feedback = i18n.translate( 'Liked by you and %s' ).fetch( likers );
			} else {
				likers = i18n.translate( '%d other person' ).fetch( userCount );
				feedback = i18n.translate( 'Liked by you and %s' ).fetch( likers );
			}
		} else {
			likers = i18n.translate( '%d people' ).fetch( found );
			feedback = i18n.translate( 'Liked by %s' ).fetch( likers );
		}
		return feedback;
	}

	// Display the widget
	function displayCommentLikeWidget( blog_id, comment_id, width, likes, obj_id ) {
		if ( wpLikes.commentLikesKillSwitch ) {
			return;
		}

		if ( wpLikes.me ) {
			wpLikes.isLoggedIn = true;
		}

		var isLiked = likes.i_like;

		var label = '';
		var css_state = '';

		var feedback = getCommentLikeFeedback( isLiked, likes.found );

		// Figure out the button label and css class for this button
		if ( isLiked ) {
			label = feedback;
			css_state = 'comment-liked';
		} else {
			label = feedback;
			css_state = 'comment-not-liked';
		}

		var widgetDocument = window.parent.frames[ 'like-comment-frame-' + obj_id ].document;

		// Just the star in the iframe
		var template = window.tmpl( document.querySelector( '#comment-likes' ).innerHTML );
		widgetDocument.querySelector( '#target' ).innerHTML = template( {
			css_state: css_state,
			label: label,
		} );

		wpLikes.postMessage(
			{
				event: 'showCommentLikeWidget',
				id: 'like-comment-wrapper-' + obj_id,
				blog_id: blog_id,
				comment_id: comment_id,
				obj_id: obj_id,
			},
			window.parent
		);

		var likeLink = widgetDocument.querySelector( 'a.comment-like-link' );
		if ( likeLink ) {
			likeLink.onclick = function ( e ) {
				e.preventDefault();

				if ( ! wpLikes.isLoggedIn ) {
					wpLikes.login_blog_id = blog_id;
					wpLikes.login_comment_id = comment_id;
					wpLikes.login_obj_id = obj_id;

					new Image().src =
						document.location.protocol +
						'//pixel.wp.com/b.gif?v=wpcom-no-pv&x_likes=loggedout_comment_like_click&baba=' +
						Math.random();

					// User isn't logged in, so we should get them to do that.
					wpLikes.openLoginWindow();
					return;
				}

				function addClass( className, el ) {
					if ( el.classList ) {
						el.classList.add( className );
					} else {
						el.className += ' ' + className;
					}
				}

				function removeClass( className, el ) {
					if ( el.classList ) {
						el.classList.remove( className );
					} else {
						el.className = el.className.replace(
							new RegExp( '(^|\\b)' + className.split( ' ' ).join( '|' ) + '(\\b|$)', 'gi' ),
							' '
						);
					}
				}

				function hasClass( className, el ) {
					if ( el.classList ) {
						return el.classList.contains( className );
					}
					return new RegExp( '(^| )' + className + '( |$)', 'gi' ).test( el.className );
				}

				var link = e.target;
				addClass( 'loading', link );

				function updateCommentFeedback( action, i_like, count ) {
					if ( action === 'like' ) {
						removeClass( 'comment-not-liked', link.parentNode );
						addClass( 'comment-liked', link.parentNode );
					} else {
						removeClass( 'comment-liked', link.parentNode );
						addClass( 'comment-not-liked', link.parentNode );
					}

					feedback = getCommentLikeFeedback( i_like, count );
					link.textContent = feedback;

					wpLikes.postMessage(
						{
							event: 'showCommentLikeWidget',
							id: 'like-comment-wrapper-' + obj_id,
							blog_id: blog_id,
							comment_id: comment_id,
							obj_id: obj_id,
						},
						window.parent
					);
				}

				if ( hasClass( 'comment-not-liked', link.parentNode ) ) {
					wpLikes.likeComment( blog_id, comment_id, function ( r ) {
						updateCommentFeedback( 'like', true, r.like_count );
						removeClass( 'loading', link );
					} );
				} else {
					wpLikes.unlikeComment( blog_id, comment_id, function ( r ) {
						updateCommentFeedback( 'unlike', false, r.like_count );
						removeClass( 'loading', link );
					} );
				}

				return false;
			};
		}
	}

	// Since we can't know definitively when an iframe has finished loading
	function updateWidgetDimensions() {
		for ( var name in wpLikes.widgetDims ) {
			var widgetDocument = window.parent.frames[ name ].document;
			var likeboxWidth = this.outerWidth( widgetDocument.querySelector( '.wpl-likebox' ) );
			var likeboxHeight = this.outerHeight( widgetDocument.querySelector( '.wpl-likebox' ) );

			// For now, we only care about width changes really
			if ( likeboxWidth > 0 && likeboxWidth !== wpLikes.widgetDims[ name ].w ) {
				wpLikes.widgetDims[ name ].w = likeboxWidth;
				wpLikes.widgetDims[ name ].h = likeboxHeight;
				wpLikes.resizeFrame( name );
			}
		}
	}

	wpLikes.wpLikes();
	window.addEventListener( 'message', function ( e ) {
		var message = e && e.data;
		if ( typeof message === 'string' ) {
			try {
				message = JSON.parse( message );
			} catch ( err ) {
				return;
			}
		}

		var type = message && message.type;

		if ( type === 'likesMessage' || type === 'loginMessage' ) {
			wpLikes.readMessage( message );
		}
	} );

	window.addEventListener( 'load', function () {
		wpLikes.postMessage( { event: 'masterReady' }, parent );
	} );

	setInterval( updateWidgetDimensions, 500 );
} )();
;


==> biblio/Continuity_of_the_infimum___Bubbles__Bad__Ripples__Good_files/saved_resource_3_ <==
#jp-post-flair{padding-top:.5em}div.sharedaddy,#content div.sharedaddy,#main div.sharedaddy{clear:both}div.sharedaddy h3.sd-title{margin:0 0 1em;display:inline-block;line-height:1.2;font-size:9pt;font-weight:700}body.highlander-light h3.sd-title:before{border-top:1px solid rgba(0,0,0,.2)}body.highlander-dark h3.sd-title:before{border-top:1px solid rgba(255,255,255,.4)}.sd-sharing{margin-bottom:1em}.sd-content ul{padding:0 !important;margin:0 !important;list-style:none !important}.sd-content ul li{display:inline-block}.sd-content ul li.share-deprecated{opacity:.5}.sd-content ul li.share-deprecated a span{text-decoration:line-through}.sd-block.sd-gplus{margin:0 0 .5em}.sd-gplus .sd-content{font-size:12px}.sd-content .share-email-error .share-email-error-title{margin:.5em 0}.sd-content .share-email-error .share-email-error-text{font-family:"Open Sans",sans-serif;font-size:12px;margin:.5em 0}.sd-social-icon .sd-content ul li a.sd-button,.sd-social-text .sd-content ul li a.sd-button,.sd-content ul li a.sd-button,.sd-content ul li .option a.share-ustom,.sd-content ul li.preview-item div.option.option-smart-off a,.sd-content ul li.advanced a.share-more,.sd-social-icon-text .sd-content ul li a.sd-button,.sd-social-official .sd-content>ul>li>a.sd-button,#sharing_email .sharing_send,.sd-social-official .sd-content>ul>li .digg_button>a{text-decoration:none !important;display:inline-block;font-size:13px;font-family:"Open Sans",sans-serif;font-weight:500;border-radius:4px;color:#2c3338 !important;background:#fff;box-shadow:0 1px 2px rgba(0,0,0,.12),0 0 0 1px rgba(0,0,0,.12);text-shadow:none;line-height:23px;padding:5px 11px 4px 9px}.sd-social-official .sd-content ul li a.sd-button,.sd-social-official .sd-content ul li.preview-item div.option.option-smart-off a{align-items:center;display:flex;font-size:12px;line-height:12px;padding:1px 6px 0 5px;min-height:20px}.sd-social-official .sd-content ul.preview li a.sd-button,.sd-social-official .sd-content ul.preview li.preview-item div.option.option-smart-off a{position:relative;top:2px}.sd-content ul li a.sd-button>span,.sd-content ul li .option a.share-ustom span,.sd-content ul li.preview-item div.option.option-smart-off a span,.sd-content ul li.advanced a.share-more span,.sd-social-icon-text .sd-content ul li a.sd-button>span,.sd-social-official .sd-content>ul>li>a.sd-button span,.sd-social-official .sd-content>ul>li .digg_button>a span{line-height:23px;margin-left:6px}.sd-social-icon .sd-content ul li a.sd-button>span{margin-left:0}.sd-social-text .sd-content ul li a.sd-button span{margin-left:3px}.sd-social-official .sd-content ul li a.sd-button>span,.sd-social-official .sd-content ul li.preview-item div.option.option-smart-off a span{line-height:12px;margin-left:3px}.sd-social-official .sd-content>ul>li>a.sd-button:before,.sd-social-official .sd-content>ul>li .digg_button>a:before,.sd-social-official .sd-content .sharing-hidden .inner>ul>li>a.sd-button:before,.sd-social-official .sd-content .sharing-hidden .inner>ul>li .digg_button>a:before{margin-bottom:-1px}.sd-social-icon .sd-content ul li a.sd-button:hover,.sd-social-icon .sd-content ul li a.sd-button:active,.sd-social-text .sd-content ul li a.sd-button:hover,.sd-social-text .sd-content ul li a.sd-button:active,.sd-social-icon-text .sd-content ul li a.sd-button:hover,.sd-social-icon-text .sd-content ul li a.sd-button:active,.sd-social-official .sd-content>ul>li>a.sd-button:hover,.sd-social-official .sd-content>ul>li>a.sd-button:active,.sd-social-official .sd-content>ul>li .digg_button>a:hover,.sd-social-official .sd-content>ul>li .digg_button>a:active{box-shadow:0 1px 2px rgba(0,0,0,.22),0 0 0 1px rgba(0,0,0,.22)}.sd-social-icon .sd-content ul li a.sd-button:active,.sd-social-text .sd-content ul li a.sd-button:active,.sd-social-icon-text .sd-content ul li a.sd-button:active,.sd-social-official .sd-content>ul>li>a.sd-button:active,.sd-social-official .sd-content>ul>li .digg_button>a:active{box-shadow:inset 0 1px 0 rgba(0,0,0,.16)}.sd-content ul li a.sd-button:before{display:inline-block;-webkit-font-smoothing:antialiased;-moz-osx-font-smoothing:grayscale;font:normal 18px/1 'social-logos';vertical-align:top;text-align:center}.sd-social-icon-text ul li a.sd-button:before{position:relative;top:2px}@media screen and (-webkit-min-device-pixel-ratio:0){.sd-content ul li a.sd-button:before{position:relative;top:2px}}.sd-social-official ul li a.sd-button:before{position:relative;top:-2px}@media screen and (-webkit-min-device-pixel-ratio:0){.sd-social-official ul li a.sd-button:before{top:0}}.sd-content ul li{margin:0 8px 12px 0;padding:0}.jp-sharing-input-touch .sd-content ul li{padding-left:10px}.sd-content ul li.preview-item.no-icon a.sd-button span{margin-left:0}.sd-social-text .sd-content ul li a:before,.sd-content ul li.no-icon a:before{display:none}body .sd-social-text .sd-content ul li.share-custom a span,body .sd-content ul li.share-custom.no-icon a span{background-image:none;background-position:-500px -500px !important;background-repeat:no-repeat !important;padding-left:0;height:0;line-height:inherit}.sd-social-icon .sd-content ul li a.share-more{position:relative;top:-4px}@media screen and (-webkit-min-device-pixel-ratio:0){.sd-social-icon .sd-content ul li a.share-more{top:2px}}@-moz-document url-prefix(){.sd-social-icon .sd-content ul li a.share-more{top:2px}}.sd-social-icon .sd-content ul li a.share-more span{margin-left:3px}.sd-social-icon .sd-content ul li.share-print a:before,.sd-social-text .sd-content ul li.share-print a:before,.sd-content ul li.share-print div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-print a:before,.sd-social-official .sd-content li.share-print a:before{content:'\f469'}.sd-social-icon .sd-content ul li.share-email a:before,.sd-social-text .sd-content ul li.share-email a:before,.sd-content ul li.share-email div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-email a:before,.sd-social-official .sd-content li.share-email a:before{content:'\f410'}.sd-social-icon .sd-content ul li.share-linkedin a:before,.sd-social-text .sd-content ul li.share-linkedin a:before,.sd-content ul li.share-linkedin div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-linkedin a:before{content:'\f207'}.sd-social-icon .sd-content ul li.share-twitter a:before,.sd-social-text .sd-content ul li.share-twitter a:before,.sd-content ul li.share-twitter div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-twitter a:before{content:'\f202'}.sd-social-icon .sd-content ul li.share-reddit a:before,.sd-social-text .sd-content ul li.share-reddit a:before,.sd-content ul li.share-reddit div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-reddit a:before{content:'\f222'}.sd-social-icon .sd-content ul li.share-tumblr a:before,.sd-social-text .sd-content ul li.share-tumblr a:before,.sd-content ul li.share-tumblr div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-tumblr a:before{content:'\f607'}.sd-social-icon .sd-content ul li.share-pocket a:before,.sd-social-text .sd-content ul li.share-pocket a:before,.sd-content ul li.share-pocket div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-pocket a:before{content:'\f224'}.sd-social-icon .sd-content ul li.share-pinterest a:before,.sd-social-text .sd-content ul li.share-pinterest a:before,.sd-content ul li.share-pinterest div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-pinterest a:before{content:'\f210'}.sd-social-icon .sd-content ul li.share-facebook a:before,.sd-social-text .sd-content ul li.share-facebook a:before,.sd-content ul li.share-facebook div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-facebook a:before{content:'\f203'}.sd-social-icon .sd-content ul li.share-press-this a:before,.sd-social-text .sd-content ul li.share-press-this a:before,.sd-content ul li.share-press-this div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-press-this a:before,.sd-social-official .sd-content li.share-press-this a:before{content:'\f205'}.sd-social-official .sd-content li.share-press-this a:before{color:#2ba1cb}.sd-social-icon .sd-content ul li.share-telegram a:before,.sd-social-text .sd-content ul li.share-telegram a:before,.sd-content ul li.share-telegram div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-telegram a:before,.sd-social-official .sd-content li.share-telegram a:before{content:'\f606'}.sd-social-official .sd-content li.share-telegram a:before{color:#08c}.sd-social-icon .sd-content ul li.share-skype a:before,.sd-social-text .sd-content ul li.share-skype a:before,.sd-content ul li.share-skype div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-skype a:before{content:'\f220'}.sd-social-icon .sd-content ul a.share-more:before,.sd-social-text .sd-content ul a.share-more:before,.sd-content ul li.advanced a.share-more:before,.sd-social-icon-text .sd-content a.share-more:before,.sd-social-official .sd-content a.share-more:before{content:'\f415'}.sd-social-official .sd-content a.share-more:before{color:#2ba1cb}.sd-social-icon .sd-content ul li.share-jetpack-whatsapp a:before,.sd-social-text .sd-content ul li.share-jetpack-whatsapp a:before,.sd-content ul li.share-jetpack-whatsapp div.option.option-smart-off a:before,.sd-social-icon-text .sd-content li.share-jetpack-whatsapp a:before,.sd-social-official .sd-content li.share-jetpack-whatsapp a:before{content:'\f608'}.sd-social-official .sd-content li.share-jetpack-whatsapp a:before{color:#43d854}.sd-social-icon .sd-content ul li[class*=share-].share-jetpack-whatsapp a.sd-button{background:#43d854;color:#fff !important}.sd-social-icon .sd-content ul li.share-deprecated a:before,.sd-social-icon-text .sd-content li.share-deprecated a:before,.sd-social-official .sd-content li.share-deprecated a:before,.sd-content ul li.share-deprecated div.option.option-smart-off a:before{width:1em;height:1em;content:"\1F6AB"}.sd-social .sd-button .share-count{background:#2ea2cc;color:#fff;-moz-border-radius:10px;border-radius:10px;display:inline-block;text-align:center;font-size:10px;padding:1px 3px;line-height:1}.sd-social-official .sd-content>ul>li>a.sd-button span{line-height:1}.sd-social-official .sd-content ul{display:flex;flex-wrap:wrap}.sd-social-official .sd-content ul:after{content:".";display:block;height:0;clear:both;visibility:hidden}.sd-social-official .sd-content li.share-press-this a{margin:0 0 5px}.sd-social-official .sd-content ul>li{display:flex;max-height:18px}.sd-social-official .sd-content ul>li .option-smart-off{margin-right:8px}.sd-social-official .fb-share-button>span{vertical-align:top !important}.sd-social-official .sd-content .pocket_button iframe{width:98px}.reddit_button iframe{margin-top:1px}.pocket_button iframe,.pinterest_button,.twitter_button,.linkedin_button>span{margin:0 !important}.linkedin_button>span,.pinterest_button a{display:block !important}.sd-social-official .sd-content .share-skype{min-width:55px}body .sd-social-official li.share-print,body .sd-social-official li.share-email a,body .sd-social-official li.share-custom a,body .sd-social-official li a.share-more,body .sd-social-official li.share-digg a,body .sd-social-official li.share-press-this a{position:relative;top:0}body .sd-social-icon .sd-content li.share-custom>a{padding:2px 3px 0;position:relative;top:4px}body .sd-social-icon .sd-content li.share-custom a span,body .sd-social-icon-text .sd-content li.share-custom a span,body .sd-social-text .sd-content li.share-custom a span,body .sd-social-official .sd-content li.share-custom a span,body .sd-content ul li.share-custom a.share-icon span{background-size:16px 16px;background-repeat:no-repeat;margin-left:0;padding:0 0 0 19px;display:inline-block;height:21px;line-height:16px}body .sd-social-icon .sd-content li.share-custom a span{width:0}body .sd-social-icon .sd-content li.share-custom a span{padding-left:16px !important}.sharing-hidden .inner{position:absolute;z-index:2;border:1px solid #ccc;padding:10px;background:#fff;box-shadow:0px 5px 20px rgba(0,0,0,.2);-webkit-border-radius:2px;-moz-border-radius:2px;border-radius:2px;margin-top:5px;max-width:400px}.sharing-hidden .inner ul{margin:0 !important}.sd-social-official .sd-content .sharing-hidden ul>li.share-end{clear:both;margin:0 !important;height:0 !important}.sharing-hidden .inner:before,.sharing-hidden .inner:after{position:absolute;z-index:1;top:-8px;left:20px;width:0;height:0;border-left:6px solid transparent;border-right:6px solid transparent;border-bottom:8px solid #ccc;content:"";display:block}.sharing-hidden .inner:after{z-index:2;top:-7px;border-left:6px solid transparent;border-right:6px solid transparent;border-bottom:8px solid #fff}.sharing-hidden ul{margin:0}.sd-social-icon .sd-content ul li[class*=share-] a,.sd-social-icon .sd-content ul li[class*=share-] a:hover,.sd-social-icon .sd-content ul li[class*=share-] div.option a{border-radius:50%;-webkit-border-radius:50%;border:0;box-shadow:none;padding:7px;position:relative;top:-2px;line-height:1;width:auto;height:auto;margin-bottom:0;max-width:32px}.sd-social-icon .sd-content ul li[class*=share-] a.sd-button>span,.sd-social-icon .sd-content ul li[class*=share-] div.option a span{line-height:1}.sd-social-icon .sd-content ul li[class*=share-] a:hover,.sd-social-icon .sd-content ul li[class*=share-] div.option a:hover{border:none;opacity:.6}.sd-social-icon .sd-content ul li[class*=share-] a.sd-button:before{top:0}.sd-social-icon .sd-content ul li[class*=share-] a.sd-button.share-custom{padding:8px 8px 6px;top:5px}.sd-social-icon .sd-content ul li a.sd-button.share-more{margin-left:10px}.sd-social-icon .sd-content ul li:first-child a.sd-button.share-more{margin-left:0}.sd-social-icon .sd-button span.share-count{position:absolute;bottom:0;right:0;border-radius:0;background:#555;font-size:9px}.sd-social-icon .sd-content ul li[class*=share-] a.sd-button{background:#e9e9e9;margin-top:2px;text-indent:0}.sd-social-icon .sd-content ul li[class*=share-].share-tumblr a.sd-button{background:#2c4762;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-facebook a.sd-button{background:#1877f2;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-twitter a.sd-button{background:#00acee;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-pinterest a.sd-button{background:#ca1f27;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-digg a.sd-button{color:#555 !important}.sd-social-icon .sd-content ul li[class*=share-].share-press-this a.sd-button{background:#4f94d4;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-telegram a.sd-button{background:#08c;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-linkedin a.sd-button{background:#0077b5;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-pocket a.sd-button{background:#ee4056;color:#fff !important}.sd-social-icon .sd-content ul li[class*=share-].share-reddit a.sd-button{background:#cee3f8;color:#555 !important}.sd-social-icon .sd-content ul li[class*=share-].share-skype a.sd-button{background:#00aff0;color:#fff !important}.sharing-screen-reader-text{clip:rect(1px,1px,1px,1px);position:absolute !important;height:1px;width:1px;overflow:hidden}.sharing-screen-reader-text:hover,.sharing-screen-reader-text:active,.sharing-screen-reader-text:focus{background-color:#f0f0f1;border-radius:3px;box-shadow:0 0 2px 2px rgba(0,0,0,.6);clip:auto !important;color:#21759b;display:block;font-size:14px;font-weight:700;height:auto;left:5px;line-height:normal;padding:15px 23px 14px;text-decoration:none;top:5px;width:auto;z-index:100000}#jetpack-source_f_name{display:none!important;position:absolute !important;left:-9000px}.sd-content .share-customize-link{margin-top:8px;line-height:11px}.sd-content .share-customize-link a{font-size:11px;font-family:"Open Sans",sans-serif}@media print{.sharedaddy.sd-sharing-enabled{display:none}}@font-face{font-family:"social-logos";src:url(/wp-content/mu-plugins/jetpack-plugin/production/_inc/social-logos/social-logos.woff2) format('woff2'),url(/wp-content/mu-plugins/jetpack-plugin/production/_inc/social-logos/social-logos.woff) format('woff'),url(/wp-content/mu-plugins/jetpack-plugin/production/_inc/social-logos/social-logos.ttf) format('truetype');font-weight:400;font-style:normal}.social-logo{font-family:"social-logos";display:inline-block;vertical-align:middle;line-height:1;font-weight:400;font-style:normal;speak:none;text-decoration:inherit;text-transform:none;text-rendering:auto;-webkit-font-smoothing:antialiased;-moz-osx-font-smoothing:grayscale}.social-logo__amazon:before{content:"\f600"}.social-logo__behance:before{content:"\f101"}.social-logo__blogger-alt:before{content:"\f601"}.social-logo__blogger:before{content:"\f602"}.social-logo__codepen:before{content:"\f216"}.social-logo__dribbble:before{content:"\f201"}.social-logo__dropbox:before{content:"\f225"}.social-logo__eventbrite:before{content:"\f603"}.social-logo__facebook:before{content:"\f203"}.social-logo__feed:before{content:"\f413"}.social-logo__flickr:before{content:"\f211"}.social-logo__foursquare:before{content:"\f226"}.social-logo__ghost:before{content:"\f61c"}.social-logo__github:before{content:"\f200"}.social-logo__google-alt:before{content:"\f102"}.social-logo__google-plus-alt:before{content:"\f218"}.social-logo__google-plus:before{content:"\f206"}.social-logo__google:before{content:"\f103"}.social-logo__instagram:before{content:"\f215"}.social-logo__link:before{content:"\f109"}.social-logo__linkedin:before{content:"\f207"}.social-logo__mail:before{content:"\f410"}.social-logo__mastodon:before{content:"\f10a"}.social-logo__medium-alt:before{content:"\f106"}.social-logo__medium:before{content:"\f623"}.social-logo__patreon:before{content:"\f105"}.social-logo__pinterest-alt:before{content:"\f210"}.social-logo__pinterest:before{content:"\f209"}.social-logo__pocket:before{content:"\f224"}.social-logo__polldaddy:before{content:"\f217"}.social-logo__print:before{content:"\f469"}.social-logo__reddit:before{content:"\f222"}.social-logo__share:before{content:"\f415"}.social-logo__skype:before{content:"\f220"}.social-logo__spotify:before{content:"\f515"}.social-logo__squarespace:before{content:"\f605"}.social-logo__stumbleupon:before{content:"\f223"}.social-logo__telegram:before{content:"\f606"}.social-logo__tiktok-alt:before{content:"\f107"}.social-logo__tiktok:before{content:"\f108"}.social-logo__tumblr-alt:before{content:"\f607"}.social-logo__tumblr:before{content:"\f214"}.social-logo__twitch:before{content:"\f516"}.social-logo__twitter-alt:before{content:"\f202"}.social-logo__twitter:before{content:"\f610"}.social-logo__vimeo:before{content:"\f212"}.social-logo__whatsapp:before{content:"\f608"}.social-logo__woocommerce:before{content:"\f104"}.social-logo__wordpress:before{content:"\f205"}.social-logo__xanga:before{content:"\f609"}.social-logo__youtube:before{content:"\f213"}img.latex{border:none;vertical-align:middle}.video-player{border:0;margin:auto;padding:5px;text-align:center;max-width:100%}.hidden{display:none}.screen-reader-text{position:absolute;left:-1000em}.comment object,.comment embed,.embed-vimeo iframe,.embed-youtube iframe{max-width:100%}.simple-homepage{display:none}

==> biblio/Continuity_of_the_infimum___Bubbles__Bad__Ripples__Good_files/saved_resource_4_ <==
( function ( g ) {

  var t = {
      PLATFORM_WINDOWS: 'windows',
      PLATFORM_IPHONE: 'iphone',
      PLATFORM_IPOD: 'ipod',
      PLATFORM_IPAD: 'ipad',
      PLATFORM_BLACKBERRY: 'blackberry',
      PLATFORM_BLACKBERRY_10: 'blackberry_10',
      PLATFORM_SYMBIAN: 'symbian_series60',
      PLATFORM_SYMBIAN_S40: 'symbian_series40',
      PLATFORM_J2ME_MIDP: 'j2me_midp',
      PLATFORM_ANDROID: 'android',
      PLATFORM_ANDROID_TABLET: 'android_tablet',
      PLATFORM_FIREFOX_OS: 'firefoxOS',
      PLATFORM_MOBILE_GENERIC: 'mobile_generic',

      userAgent : false, // Shortcut to the browser User Agent String.
      matchedPlatformName : false, // Matched platform name. False otherwise.
      matchedUserAgentName : false, // Matched UA String. False otherwise.

      init: function() {
        try {
          t.userAgent = g.navigator.userAgent.toLowerCase();
          t.getPlatformName();
          t.getMobileUserAgentName();
        }	catch ( e ) {
          console.error( e );
        }
      },

      initForTest: function( userAgent ) {
        t.matchedPlatformName = false;
        t.matchedUserAgentName = false;
        try {
          t.userAgent = userAgent.toLowerCase();
          t.getPlatformName();
          t.getMobileUserAgentName();
        }	catch ( e ) {
          console.error( e );
        }
      },

      /**
       * This method detects the mobile User Agent name.
       */
      getMobileUserAgentName: function() {
        if ( t.matchedUserAgentName !== false )
          return t.matchedUserAgentName;

        if ( t.userAgent === false )
          return false;

        if ( t.isChromeForIOS() )
          t.matchedUserAgentName = 'chrome-for-ios';
        else if ( t.isTwitterForIpad() )
          t.matchedUserAgentName =  'twitter-for-ipad';
        else if ( t.isTwitterForIphone() )
          t.matchedUserAgentName =  'twitter-for-iphone';
        else if ( t.isIPhoneOrIPod() )
          t.matchedUserAgentName = 'iphone';
        else if ( t.isIPad() )
          t.matchedUserAgentName = 'ipad';
        else if ( t.isAndroidTablet() )
          t.matchedUserAgentName = 'android_tablet';
        else if ( t.isAndroid() )
          t.matchedUserAgentName = 'android';
        else if ( t.isBlackberry10() )
          t.matchedUserAgentName = 'blackberry_10';
        else if ( has( 'blackberry' ) )
          t.matchedUserAgentName = 'blackberry';
        else if ( t.isBlackberryTablet() )
          t.matchedUserAgentName = 'blackberry_tablet';
        else if ( t.isWindowsPhone7() )
          t.matchedUserAgentName = 'win7';
        else if ( t.isWindowsPhone8() )
          t.matchedUserAgentName = 'winphone8';
        else if ( t.isOperaMini() )
          t.matchedUserAgentName = 'opera-mini';
        else if ( t.isOperaMobile() )
          t.matchedUserAgentName = 'opera-mobi';
        else if ( t.isKindleFire() )
          t.matchedUserAgentName = 'kindle-fire';
        else if ( t.isSymbianPlatform() )
          t.matchedUserAgentName = 'series60';
        else if ( t.isFirefoxMobile() )
          t.matchedUserAgentName = 'firefox_mobile';
        else if ( t.isFirefoxOS() )
          t.matchedUserAgentName = 'firefoxOS';
        else if ( t.isFacebookForIphone() )
          t.matchedUserAgentName = 'facebook-for-iphone';
        else if ( t.isFacebookForIpad() )
          t.matchedUserAgentName = 'facebook-for-ipad';
        else if ( t.isWordPressForIos() )
          t.matchedUserAgentName = 'ios-app';
        else if ( has( 'iphone' ) )
          t.matchedUserAgentName = 'iphone-unknown';
        else if ( has( 'ipad' ) )
          t.matchedUserAgentName = 'ipad-unknown';

        return t.matchedUserAgentName;
      },

      /**
       * This method detects the mobile platform name.
       */
      getPlatformName : function() {
        if ( t.matchedPlatformName !== false )
          return t.matchedPlatformName;

        if ( t.userAgent === false )
          return false;

        if ( has( 'windows ce' ) || has( 'windows phone' ) ) {
          t.matchedPlatformName = t.PLATFORM_WINDOWS;
        } else if ( has( 'ipad' ) ) {
          t.matchedPlatformName = t.PLATFORM_IPAD;
        } else if ( has( 'ipod' ) ) {
          t.matchedPlatformName = t.PLATFORM_IPOD;
        } else if ( has( 'iphone' ) ) {
          t.matchedPlatformName = t.PLATFORM_IPHONE;
        } else if ( has( 'android' ) ) {
          if ( t.isAndroidTablet() )
            t.matchedPlatformName = t.PLATFORM_ANDROID_TABLET;
          else
            t.matchedPlatformName = t.PLATFORM_ANDROID;
        } else if ( t.isKindleFire() ) {
          t.matchedPlatformName = t.PLATFORM_ANDROID_TABLET;
        } else if ( t.isBlackberry10() ) {
          t.matchedPlatformName = t.PLATFORM_BLACKBERRY_10;
        } else if ( has( 'blackberry' ) ) {
          t.matchedPlatformName = t.PLATFORM_BLACKBERRY;
        } else if ( t.isBlackberryTablet() ) {
          t.matchedPlatformName = t.PLATFORM_BLACKBERRY;
        } else if ( t.isSymbianPlatform() ) {
          t.matchedPlatformName = t.PLATFORM_SYMBIAN;
        } else if ( t.isSymbianS40Platform() ) {
          t.matchedPlatformName = t.PLATFORM_SYMBIAN_S40;
        } else if ( t.isJ2MEPlatform() ) {
          t.matchedPlatformName = t.PLATFORM_J2ME_MIDP;
        } else if ( t.isFirefoxOS() ) {
          t.matchedPlatformName = t.PLATFORM_FIREFOX_OS;
        } else if ( t.isFirefoxMobile() ) {
          t.matchedPlatformName = t.PLATFORM_MOBILE_GENERIC;
        }

        return t.matchedPlatformName;
      },


      /**
       * Detect the BlackBerry OS version.
       *
       * Note: This is for smartphones only. Does not work on BB tablets.
       */
      getBlackBerryOSVersion : check( function() {
        if ( t.isBlackberry10() )
          return '10';

        if ( ! has( 'blackberry' ) )
          return false;

        var rv = -1; // Return value assumes failure.
        var re;

        if ( has( 'webkit' ) ) { // Detecting the BB OS version for devices running OS 6.0 or higher
          re = /Version\/([\d\.]+)/i;
        } else {
          // BlackBerry devices <= 5.XX
          re = /BlackBerry\w+\/([\d\.]+)/i;
        }
        if ( re.exec( t.userAgent ) != null )
          rv =  RegExp.$1.toString();

        return rv === -1 ? false : rv;
      } ),

      /**
       * Detects if the current UA is iPhone Mobile Safari or another iPhone or iPod Touch Browser.
       */
      isIPhoneOrIPod : check( function() {
        return has( 'safari' ) && ( has( 'iphone' ) || has( 'ipod' ) );
      } ),

      /**
       * Detects if the current device is an iPad.
       */
      isIPad : check( function() {
        return has( 'ipad' ) && has( 'safari' );
      } ),


      /**
      *  Detects if the current UA is Chrome for iOS
      */
      isChromeForIOS : check( function() {
        return t.isIPhoneOrIPod() && has( 'crios/' );
      } ),

      /**
       * Detects if the current browser is the Native Android browser.
       */
      isAndroid : check( function() {
        if ( has( 'android' ) ) {
          return ! ( t.isOperaMini() || t.isOperaMobile() || t.isFirefoxMobile() );
        }
      } ),

      /**
       * Detects if the current browser is the Native Android Tablet browser.
       */
       isAndroidTablet : check( function() {
        if ( has( 'android' ) && ! has( 'mobile' ) ) {
          return ! ( t.isOperaMini() || t.isOperaMobile() || t.isFirefoxMobile() );
        }
      } ),


      /**
       * Detects if the current browser is Opera Mobile
       */
      isOperaMobile : check( function() {
        return has( 'opera' ) && has( 'mobi' );
      } ),

      /**
       * Detects if the current browser is Opera Mini
       */
      isOperaMini : check( function() {
        return has( 'opera' ) && has( 'mini' );
      } ),


      /**
       * isBlackberry10() can be used to check the User Agent for a BlackBerry 10 device.
       */
      isBlackberry10 : check( function() {
        return has( 'bb10' ) && has( 'mobile' );
      } ),

      /**
       * isBlackberryTablet() can be used to check the User Agent for a RIM blackberry tablet
       */
      isBlackberryTablet : check( function() {
        return has( 'playbook' ) && has( 'rim tablet' );
      } ),

      /**
       * Detects if the current browser is a Windows Phone 7 device.
       */
      isWindowsPhone7 : check( function () {
        return has( 'windows phone os 7' );
      } ),

      /**
       * Detects if the current browser is a Windows Phone 8 device.
       */
      isWindowsPhone8 : check( function () {
        return has( 'windows phone 8' );
      } ),

      /**
       * Detects if the device platform is J2ME.
       */
      isJ2MEPlatform : check( function () {
        return has( 'j2me/midp' ) || ( has( 'midp' ) && has( 'cldc' ) );
      } ),


      /**
       * Detects if the device platform is the Symbian Series 40.
       */
      isSymbianS40Platform : check( function() {
        if ( has( 'series40' ) ) {
          return has( 'nokia' ) || has( 'ovibrowser' ) || has( 'nokiabrowser' );
        }
      } ),


      /**
       * Detects if the device platform is the Symbian Series 60.
       */
      isSymbianPlatform : check( function() {
        if ( has( 'webkit' ) ) {
          // First, test for WebKit, then make sure it's either Symbian or S60.
          return has( 'symbian' ) || has( 'series60' );
        } else if ( has( 'symbianos' ) && has( 'series60' ) ) {
          return true;
        } else if ( has( 'nokia' ) && has( 'series60' ) ) {
          return true;
        } else if ( has( 'opera mini' ) ) {
          return has( 'symbianos' ) || has( 'symbos' ) || has( 'series 60' );
        }
      } ),


      /**
       * Detects if the current browser is the Kindle Fire Native browser.
       */
      isKindleFire : check( function() {
        return has( 'silk/' ) && has( 'silk-accelerated=' );
      } ),

      /**
       * Detects if the current browser is Firefox Mobile (Fennec)
       */
      isFirefoxMobile : check( function() {
        return has( 'fennec' );
      } ),


      /**
       * Detects if the current browser is the native FirefoxOS browser
       */
      isFirefoxOS : check( function() {
        return has( 'mozilla' ) && has( 'mobile' ) && has( 'gecko' ) && has( 'firefox' );
      } ),


      /**
       * Detects if the current UA is Facebook for iPad
       */
      isFacebookForIpad : check( function() {
        if ( ! has( 'ipad' ) )
          return false;

        return has( 'facebook' ) || has( 'fbforiphone' ) || has( 'fban/fbios;' );
      } ),

      /**
       * Detects if the current UA is Facebook for iPhone
       */
      isFacebookForIphone : check( function() {
        if ( ! has( 'iphone' ) )
          return false;

        return ( has( 'facebook' ) && ! has( 'ipad' ) ) ||
          ( has( 'fbforiphone' ) && ! has( 'tablet' ) ) ||
          ( has( 'fban/fbios;' ) && ! has( 'tablet' ) ); // FB app v5.0 or higher
      } ),

      /**
       * Detects if the current UA is Twitter for iPhone
       */
      isTwitterForIphone : check( function() {
        if ( has( 'ipad' ) )
          return false;

        return has( 'twitter for iphone' );
      } ),

      /**
       * Detects if the current UA is Twitter for iPad
       */
      isTwitterForIpad : check( function() {
        return has( 'twitter for ipad' ) || ( has( 'ipad' ) && has( 'twitter for iphone' ) );
      } ),


      /**
       * Detects if the current UA is WordPress for iOS
       */
      isWordPressForIos : check( function() {
        return has( 'wp-iphone' );
      } )
  };

  function has( str ) {
    return t.userAgent.indexOf( str ) != -1;
  }

  function check( fn ) {
    return function() {
      return t.userAgent === false ? false : fn() || false;
    }
  }

  g.wpcom_mobile_user_agent_info = t;

} )( typeof window !== 'undefined' ? window : this );
;
!function(){"use strict";var t={response:null,getEndpointURL:function(t){var e,s="undefined"!=typeof wp&&wp.customize&&wp.customize.settings&&wp.customize.settings.url&&wp.customize.settings.url.self;s?(e=document.createElement("a")).href=wp.customize.settings.url.self:e=document.location,"string"==typeof t&&t.match(/^https?:\/\//)&&((e=document.createElement("a")).href=t);var a="relatedposts=1",o=document.querySelector("#jp-relatedposts");if(!o)return!1;o.hasAttribute("data-exclude")&&(a+="&relatedposts_exclude="+o.getAttribute("data-exclude")),s&&(a+="&jetpackrpcustomize=1");var r=e.pathname;return"/"!==r[0]&&(r="/"+r),""===e.search?r+"?"+a:r+e.search+"&"+a},getAnchor:function(t,e){var s=t.title,a=document.createElement("a");a.setAttribute("class",e),a.setAttribute("href",t.url),a.setAttribute("title",s),a.setAttribute("data-origin",t.url_meta.origin),a.setAttribute("data-position",t.url_meta.position),""!==t.rel&&a.setAttribute("rel",t.rel);var o=document.createElement("div");o.appendChild(a);var r=o.innerHTML;return[r.substring(0,r.length-4),"</a>"]},generateMinimalHtml:function(t,e){var s=this,a="";return t.forEach((function(t,o){var r=s.getAnchor(t,"jp-relatedposts-post-a"),p="jp-relatedposts-post jp-relatedposts-post"+o;t.classes.length>0&&(p+=" "+t.classes.join(" ")),a+='<p class="'+p+'" data-post-id="'+t.id+'" data-post-format="'+t.format+'">',a+='<span class="jp-relatedposts-post-title">'+r[0]+t.title+r[1]+"</span>",e.showDate&&(a+='<time class="jp-relatedposts-post-date" datetime="'+t.date+'">'+t.date+"</time>"),e.showContext&&(a+='<span class="jp-relatedposts-post-context">'+t.context+"</span>"),a+="</p>"})),'<div class="jp-relatedposts-items jp-relatedposts-items-minimal jp-relatedposts-'+e.layout+' ">'+a+"</div>"},generateVisualHtml:function(t,e){var s=this,a="";return t.forEach((function(t,o){var r=s.getAnchor(t,"jp-relatedposts-post-a"),p="jp-relatedposts-post jp-relatedposts-post"+o;t.classes.length>0&&(p+=" "+t.classes.join(" ")),t.img.src?p+=" jp-relatedposts-post-thumbs":p+=" jp-relatedposts-post-nothumbs";var n=document.createElement("p");n.innerHTML=t.excerpt;var i=n.textContent;if(a+='<div class="'+p+'" data-post-id="'+t.id+'" data-post-format="'+t.format+'">',t.img.src)a+=r[0]+'<img class="jp-relatedposts-post-img" loading="lazy" src="'+t.img.src+'" width="'+t.img.width+'" height="'+t.img.height+'" alt="'+t.img.alt_text+'" />'+r[1];else{var l=s.getAnchor(t,"jp-relatedposts-post-a jp-relatedposts-post-aoverlay");a+=l[0]+l[1]}a+="<"+related_posts_js_options.post_heading+' class="jp-relatedposts-post-title">'+r[0]+t.title+r[1]+"</"+related_posts_js_options.post_heading+">",a+='<p class="jp-relatedposts-post-excerpt">'+i+"</p>",e.showDate&&(a+='<time class="jp-relatedposts-post-date" datetime="'+t.date+'">'+t.date+"</time>"),e.showContext&&(a+='<p class="jp-relatedposts-post-context">'+t.context+"</p>"),a+="</div>"})),'<div class="jp-relatedposts-items jp-relatedposts-items-visual jp-relatedposts-'+e.layout+' ">'+a+"</div>"},setVisualExcerptHeights:function(){var t=document.querySelectorAll("#jp-relatedposts .jp-relatedposts-post-nothumbs .jp-relatedposts-post-excerpt");if(t.length)for(var e=getComputedStyle(t[0]),s=parseInt(e.fontSize,10),a=parseInt(e.lineHeight,10),o=0;o<t.length;o++)t[o].style.maxHeight=5*a/s+"em"},getTrackedUrl:function(t){var e="relatedposts_hit=1";e+="&relatedposts_origin="+t.getAttribute("data-origin"),e+="&relatedposts_position="+t.getAttribute("data-position");var s=t.pathname;return"/"!==s[0]&&(s="/"+s),""===t.search?s+"?"+e:s+t.search+"&"+e},cleanupTrackedUrl:function(){if("function"==typeof history.replaceState){var t=document.location.search.replace(/\brelatedposts_[a-z]+=[0-9]*&?\b/gi,"");"?"===t&&(t=""),document.location.search!==t&&history.replaceState({},document.title,document.location.pathname+t)}}};function e(){t.setVisualExcerptHeights();var e=document.querySelectorAll("#jp-relatedposts a.jp-relatedposts-post-a");Array.prototype.forEach.call(e,(function(e){document.addEventListener("click",(function(){e.href=t.getTrackedUrl(e)}))}))}function s(){t.cleanupTrackedUrl();var s=t.getEndpointURL(),a=document.querySelector("#jp-relatedposts");if(s)if(document.querySelectorAll("#jp-relatedposts .jp-relatedposts-post").length)e();else{var o=new XMLHttpRequest;o.open("GET",s,!0),o.setRequestHeader("x-requested-with","XMLHttpRequest"),o.onreadystatechange=function(){if(this.readyState===XMLHttpRequest.DONE&&200===this.status)try{var s=JSON.parse(o.responseText);if(0===s.items.length||0===a.length)return;t.response=s;var r,p,n={};"undefined"!=typeof wp&&wp.customize?(p=wp.customize.instance("jetpack_relatedposts[show_thumbnails]").get(),n.showDate=wp.customize.instance("jetpack_relatedposts[show_date]").get(),n.showContext=wp.customize.instance("jetpack_relatedposts[show_context]").get(),n.layout=wp.customize.instance("jetpack_relatedposts[layout]").get()):(p=s.show_thumbnails,n.showDate=s.show_date,n.showContext=s.show_context,n.layout=s.layout),r=p?t.generateVisualHtml(s.items,n):t.generateMinimalHtml(s.items,n);var i=document.createElement("div");if(a.appendChild(i),i.outerHTML=r,n.showDate){var l=a.querySelectorAll(".jp-relatedposts-post-date");Array.prototype.forEach.call(l,(function(t){t.style.display="block"}))}a.style.display="block",e()}catch(t){}},o.send()}}function a(){"undefined"!=typeof wp&&wp.customize?(wp.customize.selectiveRefresh&&wp.customize.selectiveRefresh.bind("partial-content-rendered",(function(t){"jetpack_relatedposts"===t.partial.id&&s()})),wp.customize.bind("preview-ready",s)):s()}"loading"!==document.readyState?a():document.addEventListener("DOMContentLoaded",a)}();;
// listen for rlt authentication events and pass them to children of this document.
( function() {
	var currentToken;
	var parentOrigin;
	var iframeOrigins;
	var initializationListeners = [];
	var hasBeenInitialized = false;
	var RLT_KEY = 'jetpack:wpcomRLT';

	// IE11 compat version that doesn't require on `new URL( src )`
	function getOriginFromUrl( url ) {
		var parser = document.createElement('a');
		parser.href = url;
		return parser.origin;
	}

	// run on `load` for suitable iframes, this injects the current token if available
	function rltIframeInjector( event ) {
		if ( ! currentToken ) {
			return;
		}
		rltInjectToken( currentToken, event.target.contentWindow, getOriginFromUrl( event.target.src ) );
	}

	// run on DOMContentLoaded or later
	function rltMonitorIframes() {
		// wait until suitable iframes are loaded before trying to inject the RLT
		var iframes = document.querySelectorAll( "iframe" );
		for( var i=0; i<iframes.length; i++ ) {
			var iframe = iframes[i];
			if ( rltShouldAuthorizeIframe( iframe ) ) {
				iframe.addEventListener('load', rltIframeInjector);
			}
		}

		// listen for newly-created iframes, since some are injected dynamically
		var observer = new MutationObserver(function( mutationsList, observer ) {
			for(var i=0; i<mutationsList.length; i++) {
				var mutation = mutationsList[i];
				if (mutation.type === 'childList') {
					for(var j=0; j<mutation.addedNodes.length; j++) {
						var node = mutation.addedNodes[j];
						if (node instanceof HTMLElement && node.nodeName === 'IFRAME' && rltShouldAuthorizeIframe(node)) {
							node.addEventListener('load', rltIframeInjector);
						}
					}
				}
			}
		});

		observer.observe(document.body, { subtree: true, childList: true });
	}

	// should we inject RLT into this iframe?
	function rltShouldAuthorizeIframe( iframe ) {
		if ( ! Array.isArray( iframeOrigins ) ) {
			return;
		}
		return iframeOrigins.indexOf( getOriginFromUrl( iframe.src ) ) >= 0;
	}

	function rltInvalidateWindowToken( token, target, origin ) {
		if ( target && typeof target.postMessage === 'function' ) {
			try {
				target.postMessage( JSON.stringify( {
					type: 'rltMessage',
					data: {
						event: 'invalidate',
						token: token,
						sourceOrigin: window.location.origin,
					},
				} ), origin );
			} catch ( err ) {
				return;
			}
		}
	}

	/**
	 * PUBLIC METHODS
	 */
	window.rltInvalidateToken = function( token, sourceOrigin ) {
		// invalidate in current context
		if ( token === currentToken ) {
			currentToken = null;
		}

		// remove from localstorage, but only if in a top level window, not iframe
		try {
			if ( window.location === window.parent.location && window.localStorage ) {
				if ( window.localStorage.getItem(RLT_KEY) === token ) {
					window.localStorage.removeItem(RLT_KEY);
				}
			}
		} catch( e ) {
			console.info("localstorage access for invalidate denied - probably blocked third-party access", window.location.href);
		}

		// invalidate in iframes
		var iframes = document.querySelectorAll("iframe");
		for( var i=0; i<iframes.length; i++ ) {
			var iframe = iframes[i];
			var iframeOrigin = getOriginFromUrl( iframe.src );
			if ( iframeOrigin !== sourceOrigin && rltShouldAuthorizeIframe( iframe ) ) {
				rltInvalidateWindowToken( token, iframe.contentWindow, iframeOrigin );
			}
		}

		// invalidate in parent
		if ( parentOrigin && parentOrigin !== sourceOrigin && window.parent ) {
			rltInvalidateWindowToken( token, window.parent, parentOrigin );
		}
	}

	window.rltInjectToken = function( token, target, origin ) {
		if ( target && typeof target.postMessage === 'function' ) {
			try {
				target.postMessage( JSON.stringify( {
					type: 'loginMessage',
					data: {
						event: 'login',
						success: true,
						type: 'rlt',
						token: token,
						sourceOrigin: window.location.origin,
					},
				} ), origin );
			} catch ( err ) {
				return;
			}
		}
	};

	window.rltIsAuthenticated = function() {
		return !! currentToken;
	};

	window.rltGetToken = function() {
		return currentToken;
	};

	window.rltAddInitializationListener = function( listener ) {
		// if RLT is already initialized, call the listener immediately
		if ( hasBeenInitialized ) {
			listener( currentToken );
		} else {
			initializationListeners.push( listener );
		}
	};

	// store the token in localStorage
	window.rltStoreToken = function( token ) {
		currentToken = token;
		try {
			if ( window.location === window.parent.location && window.localStorage ) {
				window.localStorage.setItem( RLT_KEY, token );
			}
		} catch( e ) {
			console.info("localstorage access denied - probably blocked third-party access", window.location.href);
		}
	}

	window.rltInitialize = function( config ) {
		if ( ! config || typeof window.postMessage !== 'function' ) {
			return;
		}

		currentToken  = config.token;
		iframeOrigins = config.iframeOrigins;
		parentOrigin  = config.parentOrigin; // needed?

		// load token from localStorage if possible, but only in top level window
		try {
			if ( ! currentToken && window.location === window.parent.location && window.localStorage ) {
				currentToken = window.localStorage.getItem(RLT_KEY);
			}
		} catch( e ) {
			console.info("localstorage access denied - probably blocked third-party access", window.location.href);
		}

		// listen for RLT events from approved origins
		window.addEventListener( 'message', function( e ) {
			var message = e && e.data;
			if ( typeof message === 'string' ) {
				try {
					message = JSON.parse( message );
				} catch ( err ) {
					return;
				}
			}

			var type = message && message.type;
			var data = message && message.data;

			if ( type !== 'loginMessage' ) {
				return;
			}

			if ( data && data.type === 'rlt' && data.token !== currentToken ) {

				// put into localStorage if running in top-level window (not iframe)
				rltStoreToken( data.token );

				// send to allowlisted iframes
				var iframes = document.querySelectorAll("iframe");
				for( var i=0; i<iframes.length; i++ ) {
					var iframe = iframes[i];
					if ( rltShouldAuthorizeIframe( iframe ) ) {
						rltInjectToken( currentToken, iframe.contentWindow, getOriginFromUrl( iframe.src ) );
					}
				}

				// send to the parent, unless the event was sent _by_ the parent
				if ( parentOrigin && parentOrigin !== data.sourceOrigin && window.parent ) {
					rltInjectToken( currentToken, window.parent, parentOrigin );
				}
			}
		} );

		// listen for RLT events from approved origins
		window.addEventListener( 'message', function( e ) {
			var message = e && e.data;
			if ( typeof message === 'string' ) {
				try {
					message = JSON.parse( message );
				} catch ( err ) {
					return;
				}
			}

			var type = message && message.type;
			var data = message && message.data;

			if ( type !== 'rltMessage' ) {
				return;
			}

			if ( data && data.event === 'invalidate' && data.token === currentToken ) {
				rltInvalidateToken( data.token );
			}
		} );

		if ( iframeOrigins ) {
			if ( document.readyState !== 'loading' ) {
				rltMonitorIframes();
			} else {
				window.addEventListener( 'DOMContentLoaded', rltMonitorIframes );
			}
		}

		initializationListeners.forEach( function( listener ) {
			listener( currentToken );
		} );

		initializationListeners = [];

		hasBeenInitialized = true;
	};
} )();
;


==> biblio/Continuity_of_the_infimum___Bubbles__Bad__Ripples__Good_files/saved_resource_5_ <==
// https://www.npmjs.com/package/autosize/v/5.0.1, with the global renamed to `textarea_autosize`.
!function(e,t){"object"==typeof exports&&"undefined"!=typeof module?module.exports=t():"function"==typeof define&&define.amd?define(t):(e||self).textarea_autosize=t()}(this,function(){var e,t,n="function"==typeof Map?new Map:(e=[],t=[],{has:function(t){return e.indexOf(t)>-1},get:function(n){return t[e.indexOf(n)]},set:function(n,o){-1===e.indexOf(n)&&(e.push(n),t.push(o))},delete:function(n){var o=e.indexOf(n);o>-1&&(e.splice(o,1),t.splice(o,1))}}),o=function(e){return new Event(e,{bubbles:!0})};try{new Event("test")}catch(e){o=function(e){var t=document.createEvent("Event");return t.initEvent(e,!0,!1),t}}function r(e){var t=n.get(e);t&&t.destroy()}function i(e){var t=n.get(e);t&&t.update()}var l=null;return"undefined"==typeof window||"function"!=typeof window.getComputedStyle?((l=function(e){return e}).destroy=function(e){return e},l.update=function(e){return e}):((l=function(e,t){return e&&Array.prototype.forEach.call(e.length?e:[e],function(e){return function(e){if(e&&e.nodeName&&"TEXTAREA"===e.nodeName&&!n.has(e)){var t,r=null,i=null,l=null,d=function(){e.clientWidth!==i&&c()},u=function(t){window.removeEventListener("resize",d,!1),e.removeEventListener("input",c,!1),e.removeEventListener("keyup",c,!1),e.removeEventListener("autosize:destroy",u,!1),e.removeEventListener("autosize:update",c,!1),Object.keys(t).forEach(function(n){e.style[n]=t[n]}),n.delete(e)}.bind(e,{height:e.style.height,resize:e.style.resize,overflowY:e.style.overflowY,overflowX:e.style.overflowX,wordWrap:e.style.wordWrap});e.addEventListener("autosize:destroy",u,!1),"onpropertychange"in e&&"oninput"in e&&e.addEventListener("keyup",c,!1),window.addEventListener("resize",d,!1),e.addEventListener("input",c,!1),e.addEventListener("autosize:update",c,!1),e.style.overflowX="hidden",e.style.wordWrap="break-word",n.set(e,{destroy:u,update:c}),"vertical"===(t=window.getComputedStyle(e,null)).resize?e.style.resize="none":"both"===t.resize&&(e.style.resize="horizontal"),r="content-box"===t.boxSizing?-(parseFloat(t.paddingTop)+parseFloat(t.paddingBottom)):parseFloat(t.borderTopWidth)+parseFloat(t.borderBottomWidth),isNaN(r)&&(r=0),c()}function a(t){var n=e.style.width;e.style.width="0px",e.style.width=n,e.style.overflowY=t}function s(){if(0!==e.scrollHeight){var t=function(e){for(var t=[];e&&e.parentNode&&e.parentNode instanceof Element;)e.parentNode.scrollTop&&t.push({node:e.parentNode,scrollTop:e.parentNode.scrollTop}),e=e.parentNode;return t}(e),n=document.documentElement&&document.documentElement.scrollTop;e.style.height="",e.style.height=e.scrollHeight+r+"px",i=e.clientWidth,t.forEach(function(e){e.node.scrollTop=e.scrollTop}),n&&(document.documentElement.scrollTop=n)}}function c(){s();var t=Math.round(parseFloat(e.style.height)),n=window.getComputedStyle(e,null),r="content-box"===n.boxSizing?Math.round(parseFloat(n.height)):e.offsetHeight;if(r<t?"hidden"===n.overflowY&&(a("scroll"),s(),r="content-box"===n.boxSizing?Math.round(parseFloat(window.getComputedStyle(e,null).height)):e.offsetHeight):"hidden"!==n.overflowY&&(a("hidden"),s(),r="content-box"===n.boxSizing?Math.round(parseFloat(window.getComputedStyle(e,null).height)):e.offsetHeight),l!==r){l=r;var i=o("autosize:resized");try{e.dispatchEvent(i)}catch(e){}}}}(e)}),e}).destroy=function(e){return e&&Array.prototype.forEach.call(e.length?e:[e],r),e},l.update=function(e){return e&&Array.prototype.forEach.call(e.length?e:[e],i),e}),l});
;
(function () {
	'use strict';

	function getPostAs() {
		const postAs = document.querySelector('#hc_post_as');
		return postAs && postAs.value;
	}

	function setPostAs(value) {
		const postAs = document.querySelector('#hc_post_as');
		if (postAs) {
			postAs.value = value;
		}
	}

	function isGuest() {
		return getPostAs() === 'guest';
	}

	function hide(el) {
		if (!el) {
			return;
		}

		el.style.display = 'none';
	}

	function show(el, forceDisplay) {
		if (!el) {
			return;
		}

		el.style.removeProperty('display');
		if (forceDisplay){
			el.style.display = forceDisplay;
		}
	}

	function applyStyles(el, styles) {
		if (!el) {
			return;
		}

		Object.keys(styles || {}).forEach(prop => (el.style[prop] = styles[prop]));
	}

	function getElementOffset(el) {
		if (!el) {
			return;
		}

		const rect = el.getBoundingClientRect();
		return {
			top: rect.top + window.pageYOffset,
			left: rect.left + window.pageXOffset,
		};
	}

	function getHeightWithMargins(el) {
		if (!el) {
			return 0;
		}

		const style = getComputedStyle(el);
		return (
			el.offsetHeight +
			(parseInt(style.marginTop, 10) || 0) +
			(parseInt(style.marginBottom, 10) || 0)
		);
	}

	function getWidthWithMargins(el) {
		if (!el) {
			return 0;
		}

		const style = getComputedStyle(el);
		return (
			el.offsetWidth +
			(parseInt(style.marginLeft, 10) || 0) +
			(parseInt(style.marginRight, 10) || 0)
		);
	}

	const prefersReducedMotion = window.matchMedia('(prefers-reduced-motion: reduce)').matches;

	function animate({ el, props = {}, duration = 100, cb = () => {} } = {}) {
		if (!el) {
			return;
		}

		// Convert property names to kebab case.
		props = Object.fromEntries(
			Object.entries(props).map(([prop, val]) => [
				prop.replace(/[A-Z]/g, l => `-${l.toLowerCase()}`),
				val,
			])
		);

		const currentStyles = getComputedStyle(el);
		const transitioningProperties = Object.keys(props);
		const currentProps = Object.fromEntries(
			Object.entries(props).map(([key]) => [key, currentStyles[key]])
		);

		let willAnythingChange = false;
		Object.keys(props).forEach(key => {
			willAnythingChange = willAnythingChange || currentProps[key] !== props[key];
		});

		if (prefersReducedMotion || !willAnythingChange) {
			applyStyles(el, props);
			cb();
			return;
		}

		applyStyles(el, {
			...currentProps,
			transitionProperty: transitioningProperties.join(', '),
			transitionDuration: `${duration}ms`,
		});

		let timeout;

		// Double rAF after setting styles, for browser compatibility.
		requestAnimationFrame(() => {
			requestAnimationFrame(() => {
				applyStyles(el, props);
				const handler = e => {
					if (!e || (e.target === el && transitioningProperties.includes(e.propertyName))) {
						el.style.removeProperty('transition-property');
						el.style.removeProperty('transition-duration');
						el.removeEventListener('transitionend', handler);
						el.removeEventListener('transitioncancel', handler);
						clearTimeout(timeout);
						cb();
					}
				};
				el.addEventListener('transitionend', handler);
				el.addEventListener('transitioncancel', handler);
				timeout = setTimeout(handler, duration + 50); // Fail-safe, in case there is no transition.
			});
		});
	}

	function fadeIn({ el, duration, cb = () => {} } = {}) {
		if (!el) {
			return;
		}

		el.style.removeProperty('display');
		el.style.opacity = '0';

		animate({
			el,
			props: { opacity: '1' },
			duration,
			cb: () => {
				el.style.removeProperty('opacity');
				cb();
			},
		});
	}

	function fadeOut({ el, duration, cb = () => {} } = {}) {
		if (!el) {
			return;
		}

		el.style.removeProperty('display');
		el.style.opacity = '1';

		animate({
			el,
			props: { opacity: '0' },
			duration,
			cb: () => {
				el.style.display = 'none';
				el.style.removeProperty('opacity');
				cb();
			},
		});
	}

	function slideDown({ el, duration, cb = () => {} } = {}) {
		if (!el) {
			return;
		}

		el.style.removeProperty('display');
		const finalHeight = getComputedStyle(el).height;
		el.style.height = '0';

		animate({
			el,
			props: { height: finalHeight },
			duration,
			cb: () => {
				el.style.removeProperty('height');
				cb();
			},
		});
	}

	function slideUp({ el, duration, initialDisplay, cb = () => {} } = {}) {
		if (!el) {
			return;
		}

		if (initialDisplay !== undefined) {
			el.style.display = initialDisplay;
		} else {
			el.style.removeProperty('display');
		}

		animate({
			el,
			props: { height: 0 },
			duration,
			cb: () => {
				el.style.display = 'none';
				el.style.removeProperty('height');
				cb();
			},
		});
	}

	function createTooltip(
		anchor,
		tooltipId,
		contents,
		offset = { top: 0, left: 0 },
		rtlOffset = { top: 0, left: 0 }
	) {
		if (anchor) {
			anchor.addEventListener('mouseenter', () => {
				const pos = getElementOffset(anchor);
				let style;
				if (HighlanderComments.text_direction === 'rtl') {
					style = `top:${pos.top + rtlOffset.top}px; left:${pos.left + rtlOffset.left}px;`;
				} else {
					style = `top:${pos.top + offset.top}px; left:${pos.left + offset.left}px;`;
				}

				const popup = document.createElement('div');
				popup.id = tooltipId;
				popup.classList.add('highlander-tooltip');
				document.body.appendChild(popup);
				popup.innerHTML = contents;
				popup.style = style;
			});

			anchor.addEventListener('mouseleave', () => {
				const popup = document.querySelector(`#${tooltipId}`);
				fadeOut({
					el: popup,
					cb: () => {
						popup.remove();
						document.querySelectorAll('.highlander-tooltip').forEach(el => el.remove);
					},
				});
			});
		}
	}

	function addIframe({ classes = [], src } = {}) {
		const iframe = document.createElement('iframe');
		if (classes.length) {
			iframe.classList.add(...classes);
		}
		iframe.height = '1';
		iframe.width = '1';
		iframe.style.display = 'none';
		iframe.src = src;
		document.body.appendChild(iframe);
	}

	function getCommentList() {
		const list = document.querySelectorAll(
			'#thecomments, .thecomments, #commentlist, #comment-list, #comments-list, .commentlist, .comment-list, .comments-list, .com-list, #comments'
		);
		return list.length ? list[list.length - 1] : null;
	}

	const HighlanderComments = {
		...(window.HighlanderComments || {}),
		commentList: null,

		initialHeight: 70,

		cookies: {
			facebook: 'wpc_fbc',
			twitter: 'wpc_tc',
			wordpress: 'wpc_wpc',
		},
		popups: {
			facebook: ',height=400,width=600',
			twitter: ',height=515,width=600',
			wordpress: ',height=500,width=500',
		},
		temp_cookie_data: '',
		currentParent: false,
		currentParentId: false,
		currentParentMargins: {},
		keyCodeReturn: 13,

		resizeCallback: function () {},

		init: function () {
			// Firefox saves form data across reloads and this breaks
			// the dynamic labels when tabbing around the form
			document.getElementById("commentform")?.reset()

			document.querySelectorAll('#respond').forEach(el => el.classList.add('js'));

			HighlanderComments.commentList = getCommentList();

			document
				.querySelectorAll('#comment-form-nascar a')
				.forEach(el => el.addEventListener('click', HighlanderComments.clickService));

			document
				.querySelectorAll('#postas-wordpress, #postas-facebook, #postas-twitter')
				.forEach(el => el.addEventListener('click', HighlanderComments.clickExternalTab));

			window.addEventListener('message', e => {
				if (e.origin !== 'https://public-api.wordpress.com') {
					return;
				}

				let message = e && e.data;
				if (typeof message === 'string') {
					try {
						message = JSON.parse(message);
					} catch (err) {
						return;
					}
				}
			});

			document.querySelectorAll('.comment-form-field input, textarea#comment').forEach(el => {
				if (el.value !== '') {
					HighlanderComments.hideLabels(el);
				}
			});

			document.querySelectorAll('div.comment-form-fields input').forEach(el => {
				el.addEventListener('change', () => HighlanderComments.toggleLabel(el));
				el.addEventListener('focus', () => HighlanderComments.hideLabels(el));
				el.addEventListener('blur', () => HighlanderComments.showLabels(el));
			});

			document.querySelectorAll('div.comment-form-fields label').forEach(el =>
				el.addEventListener('click', () => {
					HighlanderComments.hideLabels(
						el.parentElement && el.parentElement.querySelectorAll('.comment-form-input input')
					);
				})
			);

			document.querySelectorAll('#email').forEach(el =>
				el.addEventListener('blur', () => {
					HighlanderComments.updateAvatarWithGravatar( el.value );

					const author = document.querySelector('#author');

					if (window.Gravatar && author && !author.value) {
						Gravatar.autofill(el.value, {
							displayName: 'author',
							url: 'url', // Their first available link, or profile URL if none
						});

						const afd = Gravatar.autofill_data;
						Gravatar.autofill_data = function (hash) {
							afd.call(Gravatar, hash);
							document
								.querySelectorAll('input#url')
								.forEach(el => el.dispatchEvent(new Event('change')));
							author.dispatchEvent(new Event('change'));
							author.dispatchEvent(new MouseEvent('click'));
						};
					}
				})
			);

			const textArea = document.querySelector('textarea#comment');

			if (!textArea) {
				return;
			}

			if (window.textarea_autosize) {
				textArea.addEventListener('autosize:resized', HighlanderComments.resizeCallback);
				window.textarea_autosize(textArea);
			}

			textArea.style.resize = 'none';
			textArea.dispatchEvent(new Event('change'));

			textArea.addEventListener('focus', () => HighlanderComments.hideLabels(textArea));
			textArea.addEventListener('blur', () => HighlanderComments.showLabels(textArea));

			textArea.addEventListener('keydown', e => {
				if (e.code === 'Tab') {
					e.preventDefault();

					let focusSel = '#comment-submit';
					if (isGuest()) {
						focusSel =
							HighlanderComments.comment_registration === '1' ? '#postas-wordpress' : '#email';
					}
					document.querySelectorAll(focusSel).forEach(el => el.focus());
				}

				if (HighlanderComments.isCommandOrControlKeyDown(e) && e.code === 'Enter') {
					document
						.querySelectorAll('#comment-submit')
						.forEach(el => el.dispatchEvent(new MouseEvent('click')));
				}
			});

			// Client-side form validation
			const form = document.querySelector('#commentform');
			form.addEventListener('submit', e => {
				let verified = true;
				// Comment text required
				if (textArea.value === '') {
					document.querySelectorAll('label[for="comment"]').forEach(el => {
						fadeOut({
							el,
							cb: () => {
								el.textContent = HighlanderComments.enterACommentError;
								fadeIn({
									el,
									cb: () => {
										el.classList.add('error');
									},
								});
							},
						});
					});

					document.querySelectorAll('#comment-form-comment').forEach(el => {
						el.classList.add('error');
						textArea.addEventListener('focus', () => el.classList.remove('error'), {
							once: true,
						});
					});
					verified = false;
				}

				// Only exists if email/name are required
				if (
					isGuest() &&
					(document.querySelector('#comment-form-guest label span[class="required"]') ||
						document.querySelector('#comment-form-guest label[class="error"]'))
				) {
					function handleMissingField(name, error) {
						document.querySelectorAll(`label[for="${name}"]`).forEach(el => {
							fadeOut({
								el,
								cb: () => {
									el.innerHTML = error;
									fadeIn({ el, cb: () => el.classList.add('error') });
								},
							});
						});
						document
							.querySelectorAll(`div.comment-form-${name} .comment-form-input`)
							.forEach(el => el.classList.add('error'));
						document
							.querySelectorAll(`input#${name}`)
							.forEach(el =>
								el.addEventListener(
									'focus',
									() => el.parentElement && el.parentElement.classList.remove('error'),
									{ once: true }
								)
							);

						verified = false;
					}

					const email = document.querySelector('#email') && document.querySelector('#email').value;
					if (email === '' || !email.match(/^.*@.*\..*$/)) {
						let error;
						if (email === '') {
							error = HighlanderComments.enterEmailError;
						} else {
							error = '<span class="nopublish">' + HighlanderComments.invalidEmailError + '</span>';
						}
						handleMissingField('email', error);
					}

					const author =
						document.querySelector('#author') && document.querySelector('#author').value;
					if (author === '') {
						const error = HighlanderComments.enterAuthorError;
						handleMissingField('author', error);
					}
				}

				// Don't allow "guest" comments if auth is required
				if (HighlanderComments.comment_registration === '1' && isGuest()) {
					document.querySelectorAll('#comment-form-nascar > p').forEach(el => {
						el.classList.add('error');
						fadeOut({ el, cb: () => fadeIn(el) });
					});
					verified = false;
				}

				// Set a cookie to remember which was the last used tab
				HighlanderComments.writeCookie('hc_post_as', getPostAs(), 7, '.wordpress.com');

				if (!verified) {
					e.preventDefault();
					return;
				}

				HighlanderComments.clickSubmit();
			});

			// Set up the identity block based on WP options, logged in state, etc
			if (HighlanderComments.comment_registration === '1') {
				// Must be logged in to comment (guest commenting not allowed)
				document.querySelectorAll('#comment-form-guest').forEach(el => hide(el));
				if (!HighlanderComments.isJetpack && !HighlanderComments.userIsLoggedIn) {
					// Force to guest posting if they're not logged in, which should actually not allow itself
					HighlanderComments.clickGuestTab();
					document
						.querySelectorAll('#comment-form-wordpress')
						.forEach(el => el.classList.remove('selected'));
					setPostAs('guest');
				}
			} else {
				// Guest commenting is allowed
				if (
					HighlanderComments.userIsLoggedIn &&
					document.querySelector('#comment-form-wordpress.selected')
				) {
					// User is logged in and we're looking at the WP UI already, get rid of guest commenting
					hide(document.querySelector('#comment-form-guest'));
				}
			}
			const selected = document.querySelector('.comment-form-service.selected');
			if (selected && !selected.matches('#comment-form-guest')) {
				// Something other than Guest is selected, hide the auth strip
				hide(document.querySelector('#comment-form-nascar'));
			}

			if (typeof addComment !== 'undefined') {
				HighlanderComments._moveForm = addComment.moveForm;
				addComment.moveForm = HighlanderComments.moveForm;
			}

			// Hover Tooltips
			// Don't show our tooltip if we're going to show a Gravatar hovercard
			if ( ! window.Gravatar || window.Gravatar.disabled ) {
				createTooltip(
					document.querySelector('#comment-form-guest .comment-form-avatar'),
					'hltt-grav',
					HighlanderComments.gravatarFromEmail,
					{ top: -10, left: 35 },
					{ top: -10, left: -130 }
				);
			}

			createTooltip(
				document.querySelector('#comment-form-nascar ul'),
				'hltt-auth',
				HighlanderComments.logInToExternalAccount,
				{ top: -12, left: -155 },
				{ top: -12, left: 155 }
			);
		},

		isCommandOrControlKeyDown: function (event) {
			// event.metaKey will be true if Command key (⌘) or Windows key is down.
			return event.ctrlKey || event.metaKey;
		},

		_moveForm: null,
		moveForm: function (commId, parentId, respondId, postId) {
			if (HighlanderComments._moveForm === null) {
				return;
			}

			const respond = document.querySelector(`#${respondId}`);
			if (!respond) {
				return;
			}

			respond.style.marginLeft = 0;
			respond.style.marginRight = 0;

			const t = this;

			let r = false;
			let rHeight;

			if (HighlanderComments.currentParent) {
				if (parentId === HighlanderComments.currentParentId) {
					return false;
				}

				const wTop = window.scrollY;
				const commElOffset = getElementOffset(document.querySelector(`#${commId}`));
				const cTop = commElOffset && commElOffset.top;
				const rTop = getElementOffset(respond).top;

				if (rTop <= cTop) {
					rHeight = getHeightWithMargins(respond);
					const placeholder = document.createElement('div');
					placeholder.id = 'highlander-placeholder';
					applyStyles(placeholder, {
						margin: 0,
						padding: 0,
						border: 0,
						height: `${rHeight}px`,
						visibility: 'hidden',
						position: getComputedStyle(respond).position,
					});
					respond.before(placeholder);
				}

				r = HighlanderComments._moveForm.call(t, commId, parentId, respondId, postId);
				if (r !== false) {
					return r;
				}

				applyStyles(HighlanderComments.currentParent, HighlanderComments.currentParentMargins);

				document.querySelectorAll('#highlander-placeholder').forEach(el => el.remove());

				if (rTop <= cTop) {
					try {
						window.scrollTo({ left: window.scrollX, top: wTop - rHeight, behavior: 'smooth' });
					} catch (err) {
						window.scrollTo(window.scrollX, wTop - rHeight);
					}
				}

				HighlanderComments.moveFormNow.call(t, commId, parentId, respondId);
			} else {
				r = HighlanderComments._moveForm.call(t, commId, parentId, respondId, postId);
				if (r === false) {
					HighlanderComments.moveFormNow.call(t, commId, parentId, respondId);
				}
			}

			return r;
		},

		moveFormNow: function (commId, parentId, respondId) {
			const comment = document.querySelector(`#comment-${parentId}`);
			let currentParent = comment && comment.closest('.highlander-comment');

			if (!currentParent) {
				currentParent = comment && comment.closest('.comment');
			}
			HighlanderComments.currentParentId = parentId;

			const respond = document.querySelector(`#${respondId}`);

			if (!currentParent || !respond) {
				return;
			}

			if (!currentParent.querySelector(`#${respondId}`)) {
				const el = currentParent.parentElement;
				let betterParent = el.closest('.children');
				if (!betterParent) {
					betterParent = el.closest('.highlander-comment');
					if (!betterParent) {
						betterParent = el.closest('.comment');
					}
				}

				if (betterParent) {
					currentParent = betterParent;
				}
			}

			const style = getComputedStyle(currentParent);
			const currentParentMargins = {
				backgroundColor: style.backgroundColor,
				marginLeft: style.marginLeft,
				marginRight: style.marginRight,
			};

			// Register the new values.
			HighlanderComments.currentParent = currentParent;
			HighlanderComments.currentParentMargins = currentParentMargins;

			let autoWidth = false;

			const offOrder =
				HighlanderComments.text_direction === 'rtl' ? ['Left', 'Right'] : ['Right', 'Left'];

			const parentOffset = getElementOffset(currentParent);

			offOrder.forEach(v => {
				const outerWidth = getWidthWithMargins(currentParent);

				if (currentParentMargins[`margin${v}`] === '0px') {
					const oldOff = parentOffset.left + v === 'Right' ? outerWidth : 0;
					currentParent.style[`margin${v}`] = '0px';
					let newOff = parentOffset.left + v === 'Right' ? outerWidth : 0;
					if (oldOff !== newOff) {
						newOff = v === 'Right' ? newOff - oldOff : oldOff - newOff;
						currentParent.style[`margin${v}`] = newOff;
						currentParentMargins[`margin${v}`] = newOff;
						autoWidth = true;
					}
				}
			});

			if (autoWidth) {
				currentParent.width = 'auto';
				currentParentMargins.width = 'auto';
			}

			const rgbaTransparent = /rgba.*,\s*0\s*\)/;

			if (
				currentParentMargins.backgroundColor === 'transparent' ||
				currentParentMargins.backgroundColor.match(rgbaTransparent)
			) {
				let el = currentParent;
				let bg = 'transparent';
				let bgi = getComputedStyle(el).backgroundImage;

				while (
					bgi === 'none' &&
					el.parentNode &&
					el.parentNode !== document &&
					(bg === 'transparent' || bg.match(rgbaTransparent))
				) {
					el = el.parentNode;
					bgi = getComputedStyle(el).backgroundImage;
					bg = getComputedStyle(el).backgroundColor;
				}

				currentParent.style.backgroundColor = bg;
			}

			const cancel = document.getElementById('cancel-comment-reply-link');
			let listOffsetSource = HighlanderComments.commentList;

			let redoMargins = false;
			let grandWidth;

			// Re-initialize the commentList if it was not found during init
			if (!listOffsetSource) {
				listOffsetSource = HighlanderComments.commentList = getCommentList();
			}

			let cp = HighlanderComments.currentParent;
			while (cp !== HighlanderComments.commentList && cp !== document) {
				const style = getComputedStyle(cp);
				if (style.overflow === 'hidden' || style.overflowX === 'hidden') {
					listOffsetSource = cp;
					break;
				}

				cp = cp.parentElement;
			}

			const listOffset = getElementOffset(listOffsetSource);

			HighlanderComments._unmoveForm = cancel.onclick;
			cancel.onclick = function () {
				return HighlanderComments.unmoveForm.call(this);
			};

			if (currentParentMargins.marginLeft.toString().includes('%')) {
				grandWidth = currentParent.parentElement.offsetWidth;
				currentParentMargins.marginLeft =
					(parseFloat(currentParentMargins.marginLeft) / 100) * grandWidth;
				redoMargins = true;
			}

			if (currentParentMargins.marginRight.toString().includes('%')) {
				grandWidth = currentParent.parentElement.offsetWidth;
				currentParentMargins.marginRight =
					(parseFloat(currentParentMargins.marginRight) / 100) * grandWidth;
				redoMargins = true;
			}

			if (redoMargins) {
				applyStyles(currentParent, currentParentMargins);
			}

			const currentMargins = {
				left: parseInt(getComputedStyle(currentParent).marginLeft, 10),
				right: parseInt(getComputedStyle(currentParent).marginRight, 10),
			};

			listOffset.right = listOffset.left + getWidthWithMargins(listOffsetSource);
			parentOffset.left -= currentMargins.left;
			parentOffset.right = parentOffset.left + getWidthWithMargins(currentParent);

			hide(respond);
			animate({
				el: currentParent,
				props: {
					marginLeft: `${currentMargins.left - (parentOffset.left - listOffset.left)}px`,
					marginRight: `${currentMargins.right - (listOffset.right - parentOffset.right)}px`,
				},
				duration: 300,
				cb: () => {
					slideDown({
						el: respond,
						duration: 300,
						cb: () => {
							document.querySelectorAll(`#${commId} .comment-reply-link`).forEach(el => el.focus());
							document.querySelectorAll('#comment').forEach(el => el.focus());
							HighlanderComments.resizeCallback();

							const clearDiv = document.createElement('div');
							clearDiv.classList.add('clear');
							clearDiv.id = 'threaded-clear';
							respond.querySelector('form').after(clearDiv);
						},
					});
				},
			});
		},

		_unmoveForm: null,
		unmoveForm: function () {
			const r = HighlanderComments._unmoveForm.call(this);
			if (r !== false) {
				return r;
			}

			animate({
				el: HighlanderComments.currentParent,
				props: HighlanderComments.currentParentMargins,
				duration: 300,
				cb: () => {
					applyStyles(HighlanderComments.currentParent, HighlanderComments.currentParentMargins);
					HighlanderComments.currentParent = false;
					HighlanderComments.currentParentId = false;
				},
			});

			show(document.querySelector('#respond'));
			document.querySelectorAll('#respond div#threaded-clear').forEach(el => el.remove());
			HighlanderComments.resizeCallback();

			return r;
		},

		// Escape an input string.
		HTMLToText: function (string) {
			const temp = document.createElement('span');
			temp.textContent = string;
			return `${temp.innerHTML}`;
		},

		switchAccount: function () {
			document.querySelectorAll('.comment-form-service').forEach(el => {
				el.classList.remove('selected');
				hide(el);
			});

			setPostAs('guest');
			document
				.querySelectorAll('#comment-form-nascar > p')
				.forEach(el => el.classList.remove('error'));
			show(document.querySelector('#comment-form-nascar'));

			if (HighlanderComments.comment_registration === '1') {
				hide(document.querySelector('#comment-form-guest')); // Guest commenting not allowed
				HighlanderComments.resizeCallback();
			} else {
				slideDown({
					el: document.querySelector('#comment-form-guest'),
					cb: HighlanderComments.resizeCallback,
				});
				HighlanderComments.clickGuestTab();
			}
		},

		setConnectingToText: function (serviceFriendlyName) {
			document
				.querySelectorAll('#comment-form-load-service p')
				.forEach(
					el =>
						(el.textContent = HighlanderComments.connectingToText.replace(
							'%s',
							serviceFriendlyName
						))
				);
		},

		updateLoadServiceVisibility: function (tab) {
			document.querySelectorAll('.comment-form-service').forEach(el => {
				el.style.visibility = 'visible';
				el.classList.remove('selected');

				if (el.matches(tab)) {
					show(el, 'block');
				} else {
					hide(el);
				}
			});
		},

		clickService: function (e) {
			e.preventDefault();

			const tab = this.href.replace(/^.*#/, '#').split(':');

			if (tab[0] === '#comment-form-load-service' && tab[1]) {
				HighlanderComments.setConnectingToText(tab[1]);
			} else {
				setPostAs(tab[0].split('-').pop());
			}

			HighlanderComments.updateLoadServiceVisibility('#comment-form-load-service');

			document
				.querySelectorAll('#comment-form-nascar li.selected')
				.forEach(el => el.classList.remove('selected'));
			e.target.closest('li').classList.add('selected');
			HighlanderComments.resizeCallback();
		},

		setServiceSelected: function (service) {
			HighlanderComments.updateLoadServiceVisibility('#comment-form-load-service');
			document
				.querySelectorAll('#comment-form-nascar li.selected')
				.forEach(el => el.classList.remove('selected'));
			document.querySelectorAll(`#postas-${service}`).forEach(el => el.parentElement.classList.add('selected'));
			hide(document.querySelector('#comment-form-nascar'));
			HighlanderComments.resizeCallback();
		},

		clickGuestTab: function (e) {
			const guest = document.querySelector('#comment-form-guest');

			if (HighlanderComments.comment_registration === '1') {
				hide(guest);
			} else {
				guest.classList.add('selected');
			}

			const email = document.querySelector('#email');
			if (email && email.value.includes('@twitter.example.com')) {
				email.value = '';
				email.blur();
			}

			HighlanderComments.updateAvatarWithGravatar( email && email.value );

			// Reenable subscription options
			document.querySelectorAll('#comment-form-subscribe').forEach(el => {
				el.style.opacity = 1;
				el.querySelectorAll('input').forEach(input => input.removeAttribute('disabled'));
			});
			HighlanderComments.resizeCallback();
		},

		updateAvatarWithGravatar: function ( emailValue ) {
			const gravBase =
				('https:' === location.protocol ? 'https://secure' : 'http://www') +
				'.gravatar.com/avatar/';

			// When Avatars are disabled, Gravatar can be undefined, so we check against that first
			// and fall back to an unknown gravatar if it isn't
			let gravSource = gravBase + 'ad516503a11cd5ca435acc9bb6523536?s=54&forcedefault=1';

			if ( typeof Gravatar !== 'undefined' && emailValue ) {
				gravSource = gravBase + Gravatar.md5( emailValue.toLowerCase().trim() ) + '?s=25';
			}

			if (HighlanderComments.gravDefault !== 'gravatar_default') {
				gravSource += '&d=' + encodeURIComponent(HighlanderComments.gravDefault);
			}

			document
				.querySelectorAll('#comment-form-guest .comment-form-avatar img')
				.forEach(el => el.setAttribute('src', gravSource));
		},

		getServiceData: function (service) {
			const data = HighlanderComments.readCookie(HighlanderComments.cookies[service]);

			if (data === null || typeof data.email === 'undefined' || ! data.email ) {
				return false;
			}
			return data;
		},

		ext_win: false,
		ext_win_check: false,
		pollExternalWindow: function (service, from_tab) {
			if (!HighlanderComments.ext_win || HighlanderComments.ext_win.closed) {
				// If the cookie is available, then we must have auth'd successfully
				const foo = HighlanderComments.getServiceData(service);
				if (HighlanderComments.getServiceData(service)) {
					HighlanderComments.doExternalLoggedIn(service);
					return;
				}
				HighlanderComments.doExternalCanceled(service, from_tab);
				HighlanderComments.ext_win = false;
				clearInterval(HighlanderComments.ext_win_check);
			}
		},

		cancelExternalWindow: function () {
			if (HighlanderComments.ext_win) {
				HighlanderComments.ext_win.close();
			}
			HighlanderComments.doExternalCanceled(getPostAs(), true);
		},

		clickExternalTab: function (e) {
			if (typeof e === 'undefined') {
				return;
			}

			let fromTab = 1;
			let service;
			if (typeof e === 'string') {
				service = e;
			} else {
				service = e.currentTarget.id.split('-')[1];
				if (!e.currentTarget.matches('a')) {
					fromTab = 0;
				}
			}

			slideUp({
				el: document.querySelector('#comment-form-guest'),
				initialDisplay: 'block',
				cb: () => {
					hide(document.querySelector('#comment-form-nascar'));

					HighlanderComments.resizeCallback();

					clearInterval(HighlanderComments.ext_win_check);
					document.querySelectorAll('.highlander-tooltip').forEach(el => el.remove());

					if (
						// Found commenting cookies
						HighlanderComments.readCookie(HighlanderComments.cookies[service]) !== null &&
						// WordPress tab, and we're logged in
						((service === 'wordpress' && HighlanderComments.userIsLoggedIn) ||
							// Not WordPress tab
							service !== 'wordpress')
					) {
						if (fromTab) {
							HighlanderComments.doExternalLoggedIn(service);
						}
					} else {
						HighlanderComments.ext_win = window.open(
							`${HighlanderComments.connectURL}&service=${service}`,
							'highconn',
							`status=0,toolbar=0,location=1,menubar=0,directories=0,resizable=1,scrollbars=0${HighlanderComments.popups[service]}`
						);

						HighlanderComments.ext_win_check = setInterval(
							() => HighlanderComments.pollExternalWindow(service, fromTab),
							100
						);
					}
				},
			});
		},

		doExternalLoggedIn: function (service, postedData ) {
			clearInterval(HighlanderComments.ext_win_check);

			const data = typeof postedData === 'object' && postedData.email
				? postedData
				: HighlanderComments.getServiceData(service);

			if (typeof data !== 'object') {
				return;
			}

			if (service === 'wordpress') {
				// Allow subscription options
				document.querySelectorAll('#comment-form-subscribe').forEach(el => {
					el.style.opacity = '1';
					el.querySelectorAll('input').forEach(input => input.removeAttribute('disabled'));
				});

				// Set up Gravatar and flag as logged in. Load a page to trigger cookies etc
				document
					.querySelectorAll(`#comment-form-${service} .comment-form-avatar img`)
					.forEach(el => el.setAttribute('src', data.avatar));
				HighlanderComments.userIsLoggedIn = true;
				if (!HighlanderComments.isJetpack) {
					addIframe({
						src: `${HighlanderComments.homeURL}highlander.login/`,
						classes: ['highlander-auth-init'],
					});
				}
			} else if (service === 'facebook') {
				document
					.querySelectorAll(`#comment-form-${service} .comment-form-avatar img`)
					.forEach(el => el.setAttribute('src', data.avatar));
			} else {
				if (service === 'twitter') {
					// Disable subscription options for Twitter since we don't have an email
					document.querySelectorAll('#comment-form-subscribe').forEach(el => {
						el.style.opacity = '0.5';
						el.querySelectorAll('input').forEach(input => {
							input.disabled = true;
							input.removeAttribute('checked');
						});
					});
				}

				// Run all external avatars through ImgPress to resize them
				let url = data.avatar;
				try {
					if (data.avatar.match(/^(https?:)?\/\/i[012]\.wp\.com\//)) {
						url = data.avatar.replace(/^https?:/, location.protocol);
					} else if (data.avatar.match(/^(https?:)?\/\/(.*?\.)gravatar\.com\//)) {
						url = data.avatar.replace(/^https?:/, location.protocol);
					} else {
						const avatarURL = new URL(data.avatar, location);

						url = `${location.protocol}//i0.wp.com/${avatarURL.host}${avatarURL.pathname}?`;
						if (host === 'graph.facebook.com' && query.length) {
							url += 'q=' + encodeURIComponent(query) + '&';
						}
						url += 'resize=25%2C25';
					}
				} catch (error) {
					url = data.avatar;
				}

				document
					.querySelectorAll(`#comment-form-${service} .comment-form-avatar img`)
					.forEach(el => el.setAttribute('src', url));
			}

			document.querySelectorAll('#email').forEach(el => {
				el.value = data.email;
				el.dispatchEvent(new Event('change'));
			});
			document.querySelectorAll('#author').forEach(el => {
				el.value = data.name;
				el.dispatchEvent(new Event('change'));
			});
			document.querySelectorAll('#url').forEach(el => {
				el.value = data.link;
				el.dispatchEvent(new Event('change'));
				el.dispatchEvent(new MouseEvent('click'));
			});
			document.querySelectorAll(`#${service}-avatar`).forEach(el => (el.value = data.avatar));
			document.querySelectorAll(`#${service}-user_id`).forEach(el => (el.value = data.uid));

			setPostAs(service);

			// The child of the li.selected can be a <A> (WP, FB, Twitter) or an <IFRAME> (Google)
			const selectedLink = document.querySelector('#comment-form-nascar li.selected a');
			const selectedIFrame = document.querySelector('#comment-form-nascar li.selected iframe');

			if (
				(selectedLink && service === selectedLink.id.replace('postas-', ''))
			) {
				hide(document.querySelector('#comment-form-load-service'));
				show(document.querySelector(`#comment-form-${service}`), 'block');
				document
					.querySelectorAll(`#comment-form-${service} .comment-form-posting-as strong`)
					.forEach(el => (el.textContent = data.name + ':'));
				HighlanderComments.resizeCallback();
			}
		},

		doExternalCanceled: function (service, from_tab) {
			if (from_tab) {
				let gravSource = `${
					location.protocol === 'https:' ? 'https://secure' : 'http://www'
				}.gravatar.com/avatar/ad516503a11cd5ca435acc9bb6523536?s=25`;
				if (HighlanderComments.gravDefault !== 'gravatar_default') {
					gravSource += '&d=' + encodeURIComponent(HighlanderComments.gravDefault);
				}
				document
					.querySelectorAll(`#comment-form-${service} .comment-form-avatar img`)
					.forEach(el => el.setAttribute('src', gravSource));
				document.querySelectorAll(`.comment-meta-${service}`).forEach(el => (el.value = ''));
				document
					.querySelectorAll(`#postas-${service} span`)
					.forEach(el => (el.innerHTML = '&nbsp; &nbsp; &nbsp;'));
				hide(document.querySelector(`#comment-form-${service}`));
				HighlanderComments.switchAccount();
			}
		},

		doExternalLogout: function (service) {
			let hostname;
			if (document.location.hostname.includes('.wordpress.com')) {
				hostname = 'wordpress.com';
			} else {
				hostname = document.location.hostname;
			}

			HighlanderComments.writeCookie(HighlanderComments.cookies[service], '', -10, hostname);
			HighlanderComments.doExternalCanceled(service, true);

			if (service === 'wordpress') {
				HighlanderComments.userIsLoggedIn = false;
				addIframe({ src: HighlanderComments.logoutURL });
			}
		},

		clickSubmit: function (e) {
			document.querySelectorAll('#respond input#comment-submit').forEach(el => {
				el.value = HighlanderComments.HTMLToText(HighlanderComments.submittingText);
				el.classList.add('disabled');
				el.disabled = true;
				const p = document.createElement('p');
				p.id = 'comment-form-submitting';
				el.before(p);
				el.remove();
				p.appendChild(el);
			});
		},

		toggleLabel: function (inputs) {
			if (window.innerWidth && window.innerWidth <= 450) {
				return;
			}

			inputs = inputs instanceof Node ? [inputs] : inputs;
			inputs.forEach(input => {
				const parent = input.closest('div.comment-form-field');
				if (parent) {
					parent
						.querySelectorAll('label')
						.forEach(label => (label.style.opacity = input.value.length ? 0.05 : 1));
				}
			});
		},

		hideLabels: function (inputs) {
			inputs = inputs instanceof Node ? [inputs] : inputs;
			inputs.forEach(input => {
				if (window.innerWidth === 0 || (window.innerWidth > 450 && !input.placeholder)) {
					const parent = input.closest('div.comment-form-field');
					if (parent) {
						if (!input.value.length) {
							parent.querySelectorAll('label').forEach(label => fadeOut({ el: label }));
						} else {
							parent.querySelectorAll('label').forEach(label => hide(label));
						}
					}
				}

				input.parentElement.classList.add('active');
			});
		},

		showLabels: function (inputs) {
			inputs = inputs instanceof Node ? [inputs] : inputs;
			inputs.forEach(input => {
				if (window.innerWidth === 0 || (window.innerWidth > 450 && !input.placeholder)) {
					const parent = input.closest('div.comment-form-field');
					if (parent) {
						if (!input.value.length) {
							parent.querySelectorAll('label').forEach(label => fadeIn({ el: label }));
						} else {
							parent.querySelectorAll('label').forEach(label => show(label));
						}
					}
				}

				input.parentElement.classList.remove('active');
			});
		},

		/* Read the contents of a named cookie, assuming they are query-string-style
    delimited, and return them as a JS hash. */
		readCookie: function (c) {
			const nameEQ = c + '=';
			let cookieStrings = document.cookie.split(';');

			for (let i = 0; i < cookieStrings.length; i++) {
				let cookieString = cookieStrings[i];
				while (cookieString.charAt(0) === ' ') {
					cookieString = cookieString.substring(1, cookieString.length);
				}
				if (cookieString.indexOf(nameEQ) === 0) {
					const chunk = cookieString.substring(nameEQ.length, cookieString.length);
					const pairs = chunk.split('&');
					let cookie_data = {};
					for (let num = pairs.length - 1; num >= 0; num--) {
						const pair = pairs[num].split('=');
						cookie_data[pair[0]] = decodeURIComponent(pair[1]);
					}
					return cookie_data;
				}
			}
			return null;
		},

		writeCookie: function (name, value, days, domain) {
			let expires;
			if (days) {
				const date = new Date();
				date.setTime(date.getTime() + days * 24 * 60 * 60 * 1000);
				expires = '; expires=' + date.toGMTString();
			} else {
				expires = '';
			}

			if (domain) {
				domain = '; domain=' + domain;
			} else {
				domain = '';
			}

			HighlanderComments.temp_cookie_data = document.cookie =
				name + '=' + value + expires + '; path=/' + domain;
		},
	};

	window.HighlanderComments = HighlanderComments;

	if (document.readyState !== 'loading') {
		HighlanderComments.init();
	} else {
		document.addEventListener('DOMContentLoaded', HighlanderComments.init);
	}
})();
;


==> biblio/Continuity_of_the_infimum___Bubbles__Bad__Ripples__Good_files/saved_resource_6_ <==
const FRONTEND_SELECTOR = '.wp-block-jetpack-contact-form-container';
const EDITOR_SELECTOR = '[data-type="jetpack/contact-form"]';

const iframeCanvas = document.querySelector( 'iframe[name="editor-canvas"]' );
const doc = iframeCanvas ? iframeCanvas.contentDocument : document;
const bodyNode = doc.querySelector( 'body' );

//Fallback in case the page load event takes to long to fire up
const fallbackTimer = setTimeout( () => {
	handleFormStyles();
}, 3000 );

window.addEventListener( 'load', () => {
	const observer = new MutationObserver( () => {
		handleFormStyles();
	} );

	//Make sure to execute at least once if not triggered by the observer
	setTimeout( () => {
		handleFormStyles();

		observer.observe( document.querySelector( 'body' ), {
			childList: true,
			subtree: true,
		} );
	}, 100 );
} );

function handleFormStyles() {
	generateStyleVariables( FRONTEND_SELECTOR );
	generateStyleVariables( EDITOR_SELECTOR );
}

function generateStyleVariables( selector, outputSelector = 'body' ) {
	const STYLE_PROBE_CLASS = 'contact-form__style-probe';
	const STYLE_PROBE_STYLE =
		'position: absolute; z-index: -1; width: 1px; height: 1px; visibility: hidden';
	const HTML = `
		<div class="contact-form" style="">
			<div class="wp-block-button is-style-outline">
				<div class="wp-block-button__link">Test</div>
			</div>
			<div class="jetpack-field">
				<input class="jetpack-field__input" type="text">
			</div>
		</div>
	`;

	setTimeout( () => {
		clearTimeout( fallbackTimer );
		bodyNode.classList.add( 'contact-form-styles-loaded' );
	}, 200 );

	if ( ! doc.querySelectorAll( selector ).length ) {
		return;
	}

	let styleProbe = doc.querySelector( `.${ STYLE_PROBE_CLASS }` );
	const outputContainer = doc.querySelector( outputSelector );

	if ( styleProbe ) {
		const node = styleProbe.querySelector( 'input[type="text"]' );
		const inputBorder = window.getComputedStyle( node ).border;
		const currentInputBorder = outputContainer.style.getPropertyValue(
			'--jetpack--contact-form--border'
		);

		if ( inputBorder === currentInputBorder ) {
			return;
		}
	}

	styleProbe = doc.createElement( 'div' );
	styleProbe.className = STYLE_PROBE_CLASS;
	styleProbe.style = STYLE_PROBE_STYLE;
	styleProbe.innerHTML = HTML;

	const container = doc.querySelector( selector );
	container.appendChild( styleProbe );

	const buttonNode = styleProbe.querySelector( '.wp-block-button__link' );
	const inputNode = styleProbe.querySelector( 'input[type="text"]' );

	const backgroundColor = getBackgroundColor( bodyNode );
	const inputBackground = getBackgroundColor( inputNode );
	const primaryColor = window.getComputedStyle( buttonNode ).borderColor;

	const {
		color: textColor,
		padding: inputPadding,
		paddingTop: inputPaddingTop,
		paddingLeft: inputPaddingLeft,
		border,
		borderColor,
		borderWidth,
		borderStyle,
		borderRadius,
		fontSize,
		fontFamily,
		lineHeight,
	} = window.getComputedStyle( inputNode );

	outputContainer.style.setProperty( '--jetpack--contact-form--primary-color', primaryColor );
	outputContainer.style.setProperty( '--jetpack--contact-form--background-color', backgroundColor );
	outputContainer.style.setProperty( '--jetpack--contact-form--text-color', textColor );
	outputContainer.style.setProperty( '--jetpack--contact-form--border', border );
	outputContainer.style.setProperty( '--jetpack--contact-form--border-color', borderColor );
	outputContainer.style.setProperty( '--jetpack--contact-form--border-size', borderWidth );
	outputContainer.style.setProperty( '--jetpack--contact-form--border-style', borderStyle );
	outputContainer.style.setProperty( '--jetpack--contact-form--border-radius', borderRadius );
	outputContainer.style.setProperty( '--jetpack--contact-form--input-background', inputBackground );
	outputContainer.style.setProperty( '--jetpack--contact-form--input-padding', inputPadding );
	outputContainer.style.setProperty(
		'--jetpack--contact-form--input-padding-top',
		inputPaddingTop
	);
	outputContainer.style.setProperty(
		'--jetpack--contact-form--input-padding-left',
		inputPaddingLeft
	);
	outputContainer.style.setProperty( '--jetpack--contact-form--font-size', fontSize );
	outputContainer.style.setProperty( '--jetpack--contact-form--font-family', fontFamily );
	outputContainer.style.setProperty( '--jetpack--contact-form--line-height', lineHeight );
}

function getBackgroundColor( backgroundColorNode ) {
	let backgroundColor = window.getComputedStyle( backgroundColorNode ).backgroundColor;
	while (
		backgroundColor === 'rgba(0, 0, 0, 0)' &&
		backgroundColorNode.parentNode &&
		backgroundColorNode.parentNode.nodeType === window.Node.ELEMENT_NODE
	) {
		backgroundColorNode = backgroundColorNode.parentNode;
		backgroundColor = window.getComputedStyle( backgroundColorNode ).backgroundColor;
	}
	return backgroundColor;
}
;
/* Detect-zoom
 * -----------
 * Cross Browser Zoom and Pixel Ratio Detector
 * Version 1.0.4 | Apr 1 2013
 * dual-licensed under the WTFPL and MIT license
 * Maintained by https://github/tombigel
 * Original developer https://github.com/yonran
 */

//AMD and CommonJS initialization copied from https://github.com/zohararad/audio5js
(function (root, ns, factory) {
    "use strict";

    if (typeof (module) !== 'undefined' && module.exports) { // CommonJS
        module.exports = factory(ns, root);
    } else if (typeof (define) === 'function' && define.amd) { // AMD
        define("factory", function () {
            return factory(ns, root);
        });
    } else {
        root[ns] = factory(ns, root);
    }

}(window, 'detectZoom', function () {

    /**
     * Use devicePixelRatio if supported by the browser
     * @return {Number}
     * @private
     */
    var devicePixelRatio = function () {
        return window.devicePixelRatio || 1;
    };

    /**
     * Fallback function to set default values
     * @return {Object}
     * @private
     */
    var fallback = function () {
        return {
            zoom: 1,
            devicePxPerCssPx: 1
        };
    };
    /**
     * IE 8 and 9: no trick needed!
     * TODO: Test on IE10 and Windows 8 RT
     * @return {Object}
     * @private
     **/
    var ie8 = function () {
        var zoom = Math.round((screen.deviceXDPI / screen.logicalXDPI) * 100) / 100;
        return {
            zoom: zoom,
            devicePxPerCssPx: zoom * devicePixelRatio()
        };
    };

    /**
     * For IE10 we need to change our technique again...
     * thanks https://github.com/stefanvanburen
     * @return {Object}
     * @private
     */
    var ie10 = function () {
        var zoom = Math.round((document.documentElement.offsetHeight / window.innerHeight) * 100) / 100;
        return {
            zoom: zoom,
            devicePxPerCssPx: zoom * devicePixelRatio()
        };
    };

    /**
     * Mobile WebKit
     * the trick: window.innerWIdth is in CSS pixels, while
     * screen.width and screen.height are in system pixels.
     * And there are no scrollbars to mess up the measurement.
     * @return {Object}
     * @private
     */
    var webkitMobile = function () {
        var deviceWidth = (Math.abs(window.orientation) == 90) ? screen.height : screen.width;
        var zoom = deviceWidth / window.innerWidth;
        return {
            zoom: zoom,
            devicePxPerCssPx: zoom * devicePixelRatio()
        };
    };

    /**
     * Desktop Webkit
     * the trick: an element's clientHeight is in CSS pixels, while you can
     * set its line-height in system pixels using font-size and
     * -webkit-text-size-adjust:none.
     * device-pixel-ratio: http://www.webkit.org/blog/55/high-dpi-web-sites/
     *
     * Previous trick (used before http://trac.webkit.org/changeset/100847):
     * documentElement.scrollWidth is in CSS pixels, while
     * document.width was in system pixels. Note that this is the
     * layout width of the document, which is slightly different from viewport
     * because document width does not include scrollbars and might be wider
     * due to big elements.
     * @return {Object}
     * @private
     */
    var webkit = function () {
        var important = function (str) {
            return str.replace(/;/g, " !important;");
        };

        var div = document.createElement('div');
        div.innerHTML = "1<br>2<br>3<br>4<br>5<br>6<br>7<br>8<br>9<br>0";
        div.setAttribute('style', important('font: 100px/1em sans-serif; -webkit-text-size-adjust: none; text-size-adjust: none; height: auto; width: 1em; padding: 0; overflow: visible;'));

        // The container exists so that the div will be laid out in its own flow
        // while not impacting the layout, viewport size, or display of the
        // webpage as a whole.
        // Add !important and relevant CSS rule resets
        // so that other rules cannot affect the results.
        var container = document.createElement('div');
        container.setAttribute('style', important('width:0; height:0; overflow:hidden; visibility:hidden; position: absolute;'));
        container.appendChild(div);

        document.body.appendChild(container);
        var zoom = 1000 / div.clientHeight;
        zoom = Math.round(zoom * 100) / 100;
        document.body.removeChild(container);

        return{
            zoom: zoom,
            devicePxPerCssPx: zoom * devicePixelRatio()
        };
    };

    /**
     * no real trick; device-pixel-ratio is the ratio of device dpi / css dpi.
     * (Note that this is a different interpretation than Webkit's device
     * pixel ratio, which is the ratio device dpi / system dpi).
     *
     * Also, for Mozilla, there is no difference between the zoom factor and the device ratio.
     *
     * @return {Object}
     * @private
     */
    var firefox4 = function () {
        var zoom = mediaQueryBinarySearch('min--moz-device-pixel-ratio', '', 0, 10, 20, 0.0001);
        zoom = Math.round(zoom * 100) / 100;
        return {
            zoom: zoom,
            devicePxPerCssPx: zoom
        };
    };

    /**
     * Firefox 18.x
     * Mozilla added support for devicePixelRatio to Firefox 18,
     * but it is affected by the zoom level, so, like in older
     * Firefox we can't tell if we are in zoom mode or in a device
     * with a different pixel ratio
     * @return {Object}
     * @private
     */
    var firefox18 = function () {
        return {
            zoom: firefox4().zoom,
            devicePxPerCssPx: devicePixelRatio()
        };
    };

    /**
     * works starting Opera 11.11
     * the trick: outerWidth is the viewport width including scrollbars in
     * system px, while innerWidth is the viewport width including scrollbars
     * in CSS px
     * @return {Object}
     * @private
     */
    var opera11 = function () {
        var zoom = window.top.outerWidth / window.top.innerWidth;
        zoom = Math.round(zoom * 100) / 100;
        return {
            zoom: zoom,
            devicePxPerCssPx: zoom * devicePixelRatio()
        };
    };

    /**
     * Use a binary search through media queries to find zoom level in Firefox
     * @param property
     * @param unit
     * @param a
     * @param b
     * @param maxIter
     * @param epsilon
     * @return {Number}
     */
    var mediaQueryBinarySearch = function (property, unit, a, b, maxIter, epsilon) {
        var matchMedia;
        var head, style, div;
        if (window.matchMedia) {
            matchMedia = window.matchMedia;
        } else {
            head = document.getElementsByTagName('head')[0];
            style = document.createElement('style');
            head.appendChild(style);

            div = document.createElement('div');
            div.className = 'mediaQueryBinarySearch';
            div.style.display = 'none';
            document.body.appendChild(div);

            matchMedia = function (query) {
                style.sheet.insertRule('@media ' + query + '{.mediaQueryBinarySearch ' + '{text-decoration: underline} }', 0);
                var matched = getComputedStyle(div, null).textDecoration == 'underline';
                style.sheet.deleteRule(0);
                return {matches: matched};
            };
        }
        var ratio = binarySearch(a, b, maxIter);
        if (div) {
            head.removeChild(style);
            document.body.removeChild(div);
        }
        return ratio;

        function binarySearch(a, b, maxIter) {
            var mid = (a + b) / 2;
            if (maxIter <= 0 || b - a < epsilon) {
                return mid;
            }
            var query = "(" + property + ":" + mid + unit + ")";
            if (matchMedia(query).matches) {
                return binarySearch(mid, b, maxIter - 1);
            } else {
                return binarySearch(a, mid, maxIter - 1);
            }
        }
    };

    /**
     * Generate detection function
     * @private
     */
    var detectFunction = (function () {
        var func = fallback;
        //IE8+
        if (!isNaN(screen.logicalXDPI) && !isNaN(screen.systemXDPI)) {
            func = ie8;
        }
        // IE10+ / Touch
        else if (window.navigator.msMaxTouchPoints) {
            func = ie10;
        }
        //Mobile Webkit
        else if ('orientation' in window && typeof document.body.style.webkitMarquee === 'string') {
            func = webkitMobile;
        }
        //WebKit
        else if (typeof document.body.style.webkitMarquee === 'string') {
            func = webkit;
        }
        //Opera
        else if (navigator.userAgent.indexOf('Opera') >= 0) {
            func = opera11;
        }
        //Last one is Firefox
        //FF 18.x
        else if (window.devicePixelRatio) {
            func = firefox18;
        }
        //FF 4.0 - 17.x
        else if (firefox4().zoom > 0.001) {
            func = firefox4;
        }

        return func;
    }());


    return ({

        /**
         * Ratios.zoom shorthand
         * @return {Number} Zoom level
         */
        zoom: function () {
            return detectFunction().zoom;
        },

        /**
         * Ratios.devicePxPerCssPx shorthand
         * @return {Number} devicePxPerCssPx level
         */
        device: function () {
            return detectFunction().devicePxPerCssPx;
        }
    });
}));

var wpcom_img_zoomer = {
        clientHintSupport: {
                gravatar: false,
                files: false,
                photon: false,
                mshots: false,
                staticAssets: false,
                latex: false,
                imgpress: false,
        },
	useHints: false,
	zoomed: false,
	timer: null,
	interval: 1000, // zoom polling interval in millisecond

	// Should we apply width/height attributes to control the image size?
	imgNeedsSizeAtts: function( img ) {
		// Do not overwrite existing width/height attributes.
		if ( img.getAttribute('width') !== null || img.getAttribute('height') !== null )
			return false;
		// Do not apply the attributes if the image is already constrained by a parent element.
		if ( img.width < img.naturalWidth || img.height < img.naturalHeight )
			return false;
		return true;
	},

        hintsFor: function( service ) {
                if ( this.useHints === false ) {
                        return false;
                }
                if ( this.hints() === false ) {
                        return false;
                }
                if ( typeof this.clientHintSupport[service] === "undefined" ) {
                        return false;
                }
                if ( this.clientHintSupport[service] === true ) {
                        return true;
                }
                return false;
        },

	hints: function() {
		try {
			var chrome = window.navigator.userAgent.match(/\sChrome\/([0-9]+)\.[.0-9]+\s/)
			if (chrome !== null) {
				var version = parseInt(chrome[1], 10)
				if (isNaN(version) === false && version >= 46) {
					return true
				}
			}
		} catch (e) {
			return false
		}
		return false
	},

	init: function() {
		var t = this;
		try{
			t.zoomImages();
			t.timer = setInterval( function() { t.zoomImages(); }, t.interval );
		}
		catch(e){
		}
	},

	stop: function() {
		if ( this.timer )
			clearInterval( this.timer );
	},

	getScale: function() {
		var scale = detectZoom.device();
		// Round up to 1.5 or the next integer below the cap.
		if      ( scale <= 1.0 ) scale = 1.0;
		else if ( scale <= 1.5 ) scale = 1.5;
		else if ( scale <= 2.0 ) scale = 2.0;
		else if ( scale <= 3.0 ) scale = 3.0;
		else if ( scale <= 4.0 ) scale = 4.0;
		else                     scale = 5.0;
		return scale;
	},

	shouldZoom: function( scale ) {
		var t = this;
		// Do not operate on hidden frames.
		if ( "innerWidth" in window && !window.innerWidth )
			return false;
		// Don't do anything until scale > 1
		if ( scale == 1.0 && t.zoomed == false )
			return false;
		return true;
	},

	zoomImages: function() {
		var t = this;
		var scale = t.getScale();
		if ( ! t.shouldZoom( scale ) ){
			return;
		}
		t.zoomed = true;
		// Loop through all the <img> elements on the page.
		var imgs = document.getElementsByTagName("img");

		for ( var i = 0; i < imgs.length; i++ ) {
			// Wait for original images to load
			if ( "complete" in imgs[i] && ! imgs[i].complete )
				continue;

			// Skip images that have srcset attributes.
			if ( imgs[i].hasAttribute('srcset') ) {
				continue;
			}

			// Skip images that don't need processing.
			var imgScale = imgs[i].getAttribute("scale");
			if ( imgScale == scale || imgScale == "0" )
				continue;

			// Skip images that have already failed at this scale
			var scaleFail = imgs[i].getAttribute("scale-fail");
			if ( scaleFail && scaleFail <= scale )
				continue;

			// Skip images that have no dimensions yet.
			if ( ! ( imgs[i].width && imgs[i].height ) )
				continue;

			// Skip images from Lazy Load plugins
			if ( ! imgScale && imgs[i].getAttribute("data-lazy-src") && (imgs[i].getAttribute("data-lazy-src") !== imgs[i].getAttribute("src")))
				continue;

			if ( t.scaleImage( imgs[i], scale ) ) {
				// Mark the img as having been processed at this scale.
				imgs[i].setAttribute("scale", scale);
			}
			else {
				// Set the flag to skip this image.
				imgs[i].setAttribute("scale", "0");
			}
		}
	},

	scaleImage: function( img, scale ) {
		var t = this;
		var newSrc = img.src;

                var isFiles = false;
                var isLatex = false;
                var isPhoton = false;

		// Skip slideshow images
		if ( img.parentNode.className.match(/slideshow-slide/) )
			return false;

		// Skip CoBlocks Lightbox images
		if ( img.parentNode.className.match(/coblocks-lightbox__image/) )
			return false;

		// Scale gravatars that have ?s= or ?size=
		if ( img.src.match( /^https?:\/\/([^\/]*\.)?gravatar\.com\/.+[?&](s|size)=/ ) ) {
                        if ( this.hintsFor( "gravatar" ) === true ) {
                                return false;
                        }
			newSrc = img.src.replace( /([?&](s|size)=)(\d+)/, function( $0, $1, $2, $3 ) {
				// Stash the original size
				var originalAtt = "originals",
				originalSize = img.getAttribute(originalAtt);
				if ( originalSize === null ) {
					originalSize = $3;
					img.setAttribute(originalAtt, originalSize);
					if ( t.imgNeedsSizeAtts( img ) ) {
						// Fix width and height attributes to rendered dimensions.
						img.width = img.width;
						img.height = img.height;
					}
				}
				// Get the width/height of the image in CSS pixels
				var size = img.clientWidth;
				// Convert CSS pixels to device pixels
				var targetSize = Math.ceil(img.clientWidth * scale);
				// Don't go smaller than the original size
				targetSize = Math.max( targetSize, originalSize );
				// Don't go larger than the service supports
				targetSize = Math.min( targetSize, 512 );
				return $1 + targetSize;
			});
		}

		// Scale mshots that have width
		else if ( img.src.match(/^https?:\/\/([^\/]+\.)*(wordpress|wp)\.com\/mshots\/.+[?&]w=\d+/) ) {
                        if ( this.hintsFor( "mshots" ) === true ) {
                                return false;
                        }
			newSrc = img.src.replace( /([?&]w=)(\d+)/, function($0, $1, $2) {
				// Stash the original size
				var originalAtt = 'originalw', originalSize = img.getAttribute(originalAtt);
				if ( originalSize === null ) {
					originalSize = $2;
					img.setAttribute(originalAtt, originalSize);
					if ( t.imgNeedsSizeAtts( img ) ) {
						// Fix width and height attributes to rendered dimensions.
						img.width = img.width;
						img.height = img.height;
					}
				}
				// Get the width of the image in CSS pixels
				var size = img.clientWidth;
				// Convert CSS pixels to device pixels
				var targetSize = Math.ceil(size * scale);
				// Don't go smaller than the original size
				targetSize = Math.max( targetSize, originalSize );
				// Don't go bigger unless the current one is actually lacking
				if ( scale > img.getAttribute("scale") && targetSize <= img.naturalWidth )
					targetSize = $2;
				if ( $2 != targetSize )
					return $1 + targetSize;
				return $0;
			});

			// Update height attribute to match width
			newSrc = newSrc.replace( /([?&]h=)(\d+)/, function($0, $1, $2) {
				if ( newSrc == img.src ) {
					return $0;
				}
				// Stash the original size
				var originalAtt = 'originalh', originalSize = img.getAttribute(originalAtt);
				if ( originalSize === null ) {
					originalSize = $2;
					img.setAttribute(originalAtt, originalSize);
				}
				// Get the height of the image in CSS pixels
				var size = img.clientHeight;
				// Convert CSS pixels to device pixels
				var targetSize = Math.ceil(size * scale);
				// Don't go smaller than the original size
				targetSize = Math.max( targetSize, originalSize );
				// Don't go bigger unless the current one is actually lacking
				if ( scale > img.getAttribute("scale") && targetSize <= img.naturalHeight )
					targetSize = $2;
				if ( $2 != targetSize )
					return $1 + targetSize;
				return $0;
			});
		}

		// Scale simple imgpress queries (s0.wp.com) that only specify w/h/fit
		else if ( img.src.match(/^https?:\/\/([^\/.]+\.)*(wp|wordpress)\.com\/imgpress\?(.+)/) ) {
                        if ( this.hintsFor( "imgpress" ) === true ) {
                                return false; 
                        }
			var imgpressSafeFunctions = ["zoom", "url", "h", "w", "fit", "filter", "brightness", "contrast", "colorize", "smooth", "unsharpmask"];
			// Search the query string for unsupported functions.
			var qs = RegExp.$3.split('&');
			for ( var q in qs ) {
				q = qs[q].split('=')[0];
				if ( imgpressSafeFunctions.indexOf(q) == -1 ) {
					return false;
				}
			}
			// Fix width and height attributes to rendered dimensions.
			img.width = img.width;
			img.height = img.height;
			// Compute new src
			if ( scale == 1 )
				newSrc = img.src.replace(/\?(zoom=[^&]+&)?/, '?');
			else
				newSrc = img.src.replace(/\?(zoom=[^&]+&)?/, '?zoom=' + scale + '&');
		}

		// Scale files.wordpress.com, LaTeX, or Photon images (i#.wp.com)
		else if (
			( isFiles = img.src.match(/^https?:\/\/([^\/]+)\.files\.wordpress\.com\/.+[?&][wh]=/) ) ||
			( isLatex = img.src.match(/^https?:\/\/([^\/.]+\.)*(wp|wordpress)\.com\/latex\.php\?(latex|zoom)=(.+)/) ) ||
			( isPhoton = img.src.match(/^https?:\/\/i[\d]{1}\.wp\.com\/(.+)/) )
		) {
                        if ( false !== isFiles && this.hintsFor( "files" ) === true ) {
                                return false
                        }
                        if ( false !== isLatex && this.hintsFor( "latex" ) === true ) {
                                return false
                        }
                        if ( false !== isPhoton && this.hintsFor( "photon" ) === true ) {
                                return false
                        }
			// Fix width and height attributes to rendered dimensions.
			img.width = img.width;
			img.height = img.height;
			// Compute new src
			if ( scale == 1 ) {
				newSrc = img.src.replace(/\?(zoom=[^&]+&)?/, '?');
			} else {
				newSrc = img.src;

				var url_var = newSrc.match( /([?&]w=)(\d+)/ );
				if ( url_var !== null && url_var[2] ) {
					newSrc = newSrc.replace( url_var[0], url_var[1] + img.width );
				}

				url_var = newSrc.match( /([?&]h=)(\d+)/ );
				if ( url_var !== null && url_var[2] ) {
					newSrc = newSrc.replace( url_var[0], url_var[1] + img.height );
				}

				var zoom_arg = '&zoom=2';
				if ( !newSrc.match( /\?/ ) ) {
					zoom_arg = '?zoom=2';
				}
				img.setAttribute( 'srcset', newSrc + zoom_arg + ' ' + scale + 'x' );
			}
		}

		// Scale static assets that have a name matching *-1x.png or *@1x.png
		else if ( img.src.match(/^https?:\/\/[^\/]+\/.*[-@]([12])x\.(gif|jpeg|jpg|png)(\?|$)/) ) {
                        if ( this.hintsFor( "staticAssets" ) === true ) {
                                return false; 
                        }
			// Fix width and height attributes to rendered dimensions.
			img.width = img.width;
			img.height = img.height;
			var currentSize = RegExp.$1, newSize = currentSize;
			if ( scale <= 1 )
				newSize = 1;
			else
				newSize = 2;
			if ( currentSize != newSize )
				newSrc = img.src.replace(/([-@])[12]x\.(gif|jpeg|jpg|png)(\?|$)/, '$1'+newSize+'x.$2$3');
		}

		else {
			return false;
		}

		// Don't set img.src unless it has changed. This avoids unnecessary reloads.
		if ( newSrc != img.src ) {
			// Store the original img.src
			var prevSrc, origSrc = img.getAttribute("src-orig");
			if ( !origSrc ) {
				origSrc = img.src;
				img.setAttribute("src-orig", origSrc);
			}
			// In case of error, revert img.src
			prevSrc = img.src;
			img.onerror = function(){
				img.src = prevSrc;
				if ( img.getAttribute("scale-fail") < scale )
					img.setAttribute("scale-fail", scale);
				img.onerror = null;
			};
			// Finally load the new image
			img.src = newSrc;
		}

		return true;
	}
};

wpcom_img_zoomer.init();
;
/* global wpcom_reblog */

var jetpackLikesWidgetBatch = [];
var jetpackLikesMasterReady = false;

// Due to performance problems on pages with a large number of widget iframes that need to be loaded,
// we are limiting the processing at any instant to unloaded widgets that are currently in viewport,
// plus this constant that will allow processing of widgets above and bellow the current fold.
// This aim of it is to improve the UX and hide the transition from unloaded to loaded state from users.
var jetpackLikesLookAhead = 2000; // pixels

// Keeps track of loaded comment likes widget so we can unload them when they are scrolled out of view.
var jetpackCommentLikesLoadedWidgets = [];

var jetpackLikesDocReadyPromise = new Promise( resolve => {
	if ( document.readyState !== 'loading' ) {
		resolve();
	} else {
		window.addEventListener( 'DOMContentLoaded', () => resolve() );
	}
} );

function JetpackLikesPostMessage( message, target ) {
	if ( typeof message === 'string' ) {
		try {
			message = JSON.parse( message );
		} catch ( e ) {
			return;
		}
	}

	if ( target && typeof target.postMessage === 'function' ) {
		try {
			target.postMessage(
				JSON.stringify( {
					type: 'likesMessage',
					data: message,
				} ),
				'*'
			);
		} catch ( e ) {
			return;
		}
	}
}

function JetpackLikesBatchHandler() {
	const requests = [];
	document.querySelectorAll( 'div.jetpack-likes-widget-unloaded' ).forEach( widget => {
		if ( jetpackLikesWidgetBatch.indexOf( widget.id ) > -1 ) {
			return;
		}

		if ( ! jetpackIsScrolledIntoView( widget ) ) {
			return;
		}

		jetpackLikesWidgetBatch.push( widget.id );

		var regex = /like-(post|comment)-wrapper-(\d+)-(\d+)-(\w+)/,
			match = regex.exec( widget.id ),
			info;

		if ( ! match || match.length !== 5 ) {
			return;
		}

		info = {
			blog_id: match[ 2 ],
			width: widget.width,
		};

		if ( 'post' === match[ 1 ] ) {
			info.post_id = match[ 3 ];
		} else if ( 'comment' === match[ 1 ] ) {
			info.comment_id = match[ 3 ];
		}

		info.obj_id = match[ 4 ];

		requests.push( info );
	} );

	if ( requests.length > 0 ) {
		JetpackLikesPostMessage(
			{ event: 'initialBatch', requests: requests },
			window.frames[ 'likes-master' ]
		);
	}
}

function JetpackLikesMessageListener( event ) {
	let message = event && event.data;
	if ( typeof message === 'string' ) {
		try {
			message = JSON.parse( message );
		} catch ( err ) {
			return;
		}
	}

	const type = message && message.type;
	const data = message && message.data;

	if ( type !== 'likesMessage' || typeof data.event === 'undefined' ) {
		return;
	}

	// We only allow messages from one origin
	const allowedOrigin = 'https://widgets.wp.com';
	if ( allowedOrigin !== event.origin ) {
		return;
	}

	switch ( data.event ) {
		case 'masterReady':
			jetpackLikesDocReadyPromise.then( () => {
				jetpackLikesMasterReady = true;

				const stylesData = {
					event: 'injectStyles',
				};
				const sdTextColor = document.querySelector( '.sd-text-color' );
				const sdLinkColor = document.querySelector( '.sd-link-color' );
				const sdTextColorStyles = ( sdTextColor && getComputedStyle( sdTextColor ) ) || {};
				const sdLinkColorStyles = ( sdLinkColor && getComputedStyle( sdLinkColor ) ) || {};

				if ( document.querySelectorAll( 'iframe.admin-bar-likes-widget' ).length > 0 ) {
					JetpackLikesPostMessage( { event: 'adminBarEnabled' }, window.frames[ 'likes-master' ] );

					const bgSource = document.querySelector(
						'#wpadminbar .quicklinks li#wp-admin-bar-wpl-like > a'
					);

					const wpAdminBar = document.querySelector( '#wpadminbar' );

					stylesData.adminBarStyles = {
						background: bgSource && getComputedStyle( bgSource ).background,
						isRtl: wpAdminBar && getComputedStyle( wpAdminBar ).direction === 'rtl',
					};
				}

				// enable reblogs if they are enabled for the page
				if ( document.body.classList.contains( 'jetpack-reblog-enabled' ) ) {
					JetpackLikesPostMessage( { event: 'reblogsEnabled' }, window.frames[ 'likes-master' ] );
				}

				stylesData.textStyles = {
					color: sdTextColorStyles[ 'color' ],
					fontFamily: sdTextColorStyles[ 'font-family' ],
					fontSize: sdTextColorStyles[ 'font-size' ],
					direction: sdTextColorStyles[ 'direction' ],
					fontWeight: sdTextColorStyles[ 'font-weight' ],
					fontStyle: sdTextColorStyles[ 'font-style' ],
					textDecoration: sdTextColorStyles[ 'text-decoration' ],
				};

				stylesData.linkStyles = {
					color: sdLinkColorStyles[ 'color' ],
					fontFamily: sdLinkColorStyles[ 'font-family' ],
					fontSize: sdLinkColorStyles[ 'font-size' ],
					textDecoration: sdLinkColorStyles[ 'text-decoration' ],
					fontWeight: sdLinkColorStyles[ 'font-weight' ],
					fontStyle: sdLinkColorStyles[ 'font-style' ],
				};

				JetpackLikesPostMessage( stylesData, window.frames[ 'likes-master' ] );

				JetpackLikesBatchHandler();
			} );

			break;

		case 'showLikeWidget': {
			const placeholder = document.querySelector( `#${ data.id } .likes-widget-placeholder` );
			if ( placeholder ) {
				placeholder.style.display = 'none';
			}
			break;
		}

		case 'showCommentLikeWidget': {
			const placeholder = document.querySelector( `#${ data.id } .likes-widget-placeholder` );
			if ( placeholder ) {
				placeholder.style.display = 'none';
			}
			break;
		}

		case 'killCommentLikes':
			// If kill switch for comment likes is enabled remove all widgets wrappers and `Loading...` placeholders.
			document
				.querySelectorAll( '.jetpack-comment-likes-widget-wrapper' )
				.forEach( wrapper => wrapper.remove() );
			break;

		case 'clickReblogFlair':
			if ( wpcom_reblog && typeof wpcom_reblog.toggle_reblog_box_flair === 'function' ) {
				wpcom_reblog.toggle_reblog_box_flair( data.obj_id, data.post_id );
			}
			break;

		case 'showOtherGravatars': {
			const container = document.querySelector( '#likes-other-gravatars' );
			if ( ! container ) {
				break;
			}

			const list = container.querySelector( 'ul' );

			container.style.display = 'none';
			list.innerHTML = '';

			container
				.querySelectorAll( '.likes-text span' )
				.forEach( item => ( item.textContent = data.total ) );

			( data.likers || [] ).forEach( liker => {
				if ( liker.profile_URL.substr( 0, 4 ) !== 'http' ) {
					// We only display gravatars with http or https schema
					return;
				}

				const element = document.createElement( 'li' );
				element.innerHTML = `
					<a href="${ encodeURI( liker.profile_URL ) }" rel="nofollow" target="_parent" class="wpl-liker">
						<img src="${ encodeURI( liker.avatar_URL ) }"
							alt=""
							style="width: 30px; height: 30px; padding-right: 3px;" />
					</a>
				`;

				list.append( element );

				// Add some extra attributes through native methods, to ensure strings are sanitized.
				element.classList.add( liker.css_class );
				element.querySelector( 'img' ).alt = liker.name;
			} );

			const el = document.querySelector( `*[name='${ data.parent }']` );
			const rect = el.getBoundingClientRect();
			const win = el.ownerDocument.defaultView;
			const offset = {
				top: rect.top + win.pageYOffset,
				left: rect.left + win.pageXOffset,
			};

			container.style.left = offset.left + data.position.left - 10 + 'px';
			container.style.top = offset.top + data.position.top - 33 + 'px';

			const rowLength = Math.floor( data.width / 37 );
			let height = Math.ceil( data.likers.length / rowLength ) * 37 + 13;
			if ( height > 204 ) {
				height = 204;
			}

			const containerWidth = rowLength * 37 - 7;
			container.style.height = height + 'px';
			container.style.width = containerWidth + 'px';

			const listWidth = rowLength * 37;
			list.style.width = listWidth + 'px';

			container.style.display = 'block';

			const scrollbarWidth = list.offsetWidth - list.clientWidth;
			if ( scrollbarWidth > 0 ) {
				container.style.width = containerWidth + scrollbarWidth + 'px';
				list.style.width = listWidth + scrollbarWidth + 'px';
			}
		}
	}
}

window.addEventListener( 'message', JetpackLikesMessageListener );

document.addEventListener( 'click', e => {
	const container = document.querySelector( '#likes-other-gravatars' );

	if ( container && ! container.contains( e.target ) ) {
		container.style.display = 'none';
	}
} );

function JetpackLikesWidgetQueueHandler() {
	var wrapperID;

	if ( ! jetpackLikesMasterReady ) {
		setTimeout( JetpackLikesWidgetQueueHandler, 500 );
		return;
	}

	// Restore widgets to initial unloaded state when they are scrolled out of view.
	jetpackUnloadScrolledOutWidgets();

	var unloadedWidgetsInView = jetpackGetUnloadedWidgetsInView();

	if ( unloadedWidgetsInView.length > 0 ) {
		// Grab any unloaded widgets for a batch request
		JetpackLikesBatchHandler();
	}

	for ( var i = 0, length = unloadedWidgetsInView.length; i <= length - 1; i++ ) {
		wrapperID = unloadedWidgetsInView[ i ].id;

		if ( ! wrapperID ) {
			continue;
		}

		jetpackLoadLikeWidgetIframe( wrapperID );
	}
}

function jetpackLoadLikeWidgetIframe( wrapperID ) {
	if ( typeof wrapperID === 'undefined' ) {
		return;
	}

	const wrapper = document.querySelector( '#' + wrapperID );
	wrapper.querySelectorAll( 'iframe' ).forEach( iFrame => iFrame.remove() );

	const placeholder = wrapper.querySelector( '.likes-widget-placeholder' );

	// Post like iframe
	if ( placeholder && placeholder.classList.contains( 'post-likes-widget-placeholder' ) ) {
		const postLikesFrame = document.createElement( 'iframe' );

		postLikesFrame.classList.add( 'post-likes-widget', 'jetpack-likes-widget' );
		postLikesFrame.name = wrapper.dataset.name;
		postLikesFrame.src = wrapper.dataset.src;
		postLikesFrame.height = '55px';
		postLikesFrame.width = '100%';
		postLikesFrame.frameBorder = '0';
		postLikesFrame.scrolling = 'no';
		postLikesFrame.title = wrapper.dataset.title;

		placeholder.after( postLikesFrame );
	}

	// Comment like iframe
	if ( placeholder.classList.contains( 'comment-likes-widget-placeholder' ) ) {
		const commentLikesFrame = document.createElement( 'iframe' );

		commentLikesFrame.class = 'comment-likes-widget-frame jetpack-likes-widget-frame';
		commentLikesFrame.name = wrapper.dataset.name;
		commentLikesFrame.src = wrapper.dataset.src;
		commentLikesFrame.height = '18px';
		commentLikesFrame.width = '100%';
		commentLikesFrame.frameBorder = '0';
		commentLikesFrame.scrolling = 'no';

		wrapper.querySelector( '.comment-like-feedback' ).after( commentLikesFrame );

		jetpackCommentLikesLoadedWidgets.push( commentLikesFrame );
	}

	wrapper.classList.remove( 'jetpack-likes-widget-unloaded' );
	wrapper.classList.add( 'jetpack-likes-widget-loading' );

	wrapper.querySelector( 'iframe' ).addEventListener( 'load', e => {
		JetpackLikesPostMessage(
			{ event: 'loadLikeWidget', name: e.target.name, width: e.target.width },
			window.frames[ 'likes-master' ]
		);

		wrapper.classList.remove( 'jetpack-likes-widget-loading' );
		wrapper.classList.add( 'jetpack-likes-widget-loaded' );
	} );
}

function jetpackGetUnloadedWidgetsInView() {
	const unloadedWidgets = document.querySelectorAll( 'div.jetpack-likes-widget-unloaded' );

	return [ ...unloadedWidgets ].filter( item => jetpackIsScrolledIntoView( item ) );
}

function jetpackIsScrolledIntoView( element ) {
	const top = element.getBoundingClientRect().top;
	const bottom = element.getBoundingClientRect().bottom;

	// Allow some slack above and bellow the fold with jetpackLikesLookAhead,
	// with the aim of hiding the transition from unloaded to loaded widget from users.
	return top + jetpackLikesLookAhead >= 0 && bottom <= window.innerHeight + jetpackLikesLookAhead;
}

function jetpackUnloadScrolledOutWidgets() {
	for ( let i = jetpackCommentLikesLoadedWidgets.length - 1; i >= 0; i-- ) {
		const currentWidgetIframe = jetpackCommentLikesLoadedWidgets[ i ];

		if ( ! jetpackIsScrolledIntoView( currentWidgetIframe ) ) {
			const widgetWrapper =
				currentWidgetIframe &&
				currentWidgetIframe.parentElement &&
				currentWidgetIframe.parentElement.parentElement;

			// Restore parent class to 'unloaded' so this widget can be picked up by queue manager again if needed.
			widgetWrapper.classList.remove( 'jetpack-likes-widget-loaded' );
			widgetWrapper.classList.remove( 'jetpack-likes-widget-loading' );
			widgetWrapper.classList.add( 'jetpack-likes-widget-unloaded' );

			// Bring back the loading placeholder into view.
			widgetWrapper
				.querySelectorAll( '.comment-likes-widget-placeholder' )
				.forEach( item => ( item.style.display = 'block' ) );

			// Remove it from the list of loaded widgets.
			jetpackCommentLikesLoadedWidgets.splice( i, 1 );

			// Remove comment like widget iFrame.
			currentWidgetIframe.remove();
		}
	}
}

var jetpackWidgetsDelayedExec = function ( after, fn ) {
	var timer;
	return function () {
		clearTimeout( timer );
		timer = setTimeout( fn, after );
	};
};

var jetpackOnScrollStopped = jetpackWidgetsDelayedExec( 250, JetpackLikesWidgetQueueHandler );

// Load initial batch of widgets, prior to any scrolling events.
JetpackLikesWidgetQueueHandler();

// Add event listener to execute queue handler after scroll.
window.addEventListener( 'scroll', jetpackOnScrollStopped, true );
;
/*! This file is auto-generated */
window.addComment=function(v){var I,C,h,E=v.document,b={commentReplyClass:"comment-reply-link",commentReplyTitleId:"reply-title",cancelReplyId:"cancel-comment-reply-link",commentFormId:"commentform",temporaryFormId:"wp-temp-form-div",parentIdFieldId:"comment_parent",postIdFieldId:"comment_post_ID"},e=v.MutationObserver||v.WebKitMutationObserver||v.MozMutationObserver,r="querySelector"in E&&"addEventListener"in v,n=!!E.documentElement.dataset;function t(){d(),e&&new e(o).observe(E.body,{childList:!0,subtree:!0})}function d(e){if(r&&(I=g(b.cancelReplyId),C=g(b.commentFormId),I)){I.addEventListener("touchstart",l),I.addEventListener("click",l);function t(e){if((e.metaKey||e.ctrlKey)&&13===e.keyCode)return C.removeEventListener("keydown",t),e.preventDefault(),C.submit.click(),!1}C&&C.addEventListener("keydown",t);for(var n,d=function(e){var t=b.commentReplyClass;e&&e.childNodes||(e=E);e=E.getElementsByClassName?e.getElementsByClassName(t):e.querySelectorAll("."+t);return e}(e),o=0,i=d.length;o<i;o++)(n=d[o]).addEventListener("touchstart",a),n.addEventListener("click",a)}}function l(e){var t,n,d=g(b.temporaryFormId);d&&h&&(g(b.parentIdFieldId).value="0",t=d.textContent,d.parentNode.replaceChild(h,d),this.style.display="none",n=(d=(d=g(b.commentReplyTitleId))&&d.firstChild)&&d.nextSibling,d&&d.nodeType===Node.TEXT_NODE&&t&&(n&&"A"===n.nodeName&&n.id!==b.cancelReplyId&&(n.style.display=""),d.textContent=t),e.preventDefault())}function a(e){var t=g(b.commentReplyTitleId),t=t&&t.firstChild.textContent,n=this,d=m(n,"belowelement"),o=m(n,"commentid"),i=m(n,"respondelement"),r=m(n,"postid"),n=m(n,"replyto")||t;d&&o&&i&&r&&!1===v.addComment.moveForm(d,o,i,r,n)&&e.preventDefault()}function o(e){for(var t=e.length;t--;)if(e[t].addedNodes.length)return void d()}function m(e,t){return n?e.dataset[t]:e.getAttribute("data-"+t)}function g(e){return E.getElementById(e)}return r&&"loading"!==E.readyState?t():r&&v.addEventListener("DOMContentLoaded",t,!1),{init:d,moveForm:function(e,t,n,d,o){var i,r,l,a,m,c,s,e=g(e),n=(h=g(n),g(b.parentIdFieldId)),y=g(b.postIdFieldId),p=g(b.commentReplyTitleId),u=(p=p&&p.firstChild)&&p.nextSibling;if(e&&h&&n){void 0===o&&(o=p&&p.textContent),a=h,m=b.temporaryFormId,c=g(m),s=(s=g(b.commentReplyTitleId))?s.firstChild.textContent:"",c||((c=E.createElement("div")).id=m,c.style.display="none",c.textContent=s,a.parentNode.insertBefore(c,a)),d&&y&&(y.value=d),n.value=t,I.style.display="",e.parentNode.insertBefore(h,e.nextSibling),p&&p.nodeType===Node.TEXT_NODE&&(u&&"A"===u.nodeName&&u.id!==b.cancelReplyId&&(u.style.display="none"),p.textContent=o),I.onclick=function(){return!1};try{for(var f=0;f<C.elements.length;f++)if(i=C.elements[f],r=!1,"getComputedStyle"in v?l=v.getComputedStyle(i):E.documentElement.currentStyle&&(l=i.currentStyle),(i.offsetWidth<=0&&i.offsetHeight<=0||"hidden"===l.visibility)&&(r=!0),"hidden"!==i.type&&!i.disabled&&!r){i.focus();break}}catch(e){}return!1}}}}(window);;
/* globals JSON */
( function () {
	var eventName = 'wpcom_masterbar_click';

	var linksTracksEvents = {
		// top level items
		'wp-admin-bar-blog'                        : 'my_sites',
		'wp-admin-bar-newdash'                     : 'reader',
		'wp-admin-bar-ab-new-post'                 : 'write_button',
		'wp-admin-bar-my-account'                  : 'my_account',
		'wp-admin-bar-notes'                       : 'notifications',
		// my sites - top items
		'wp-admin-bar-switch-site'                 : 'my_sites_switch_site',
		'wp-admin-bar-blog-info'                   : 'my_sites_site_info',
		'wp-admin-bar-site-view'                   : 'my_sites_view_site',
		'wp-admin-bar-blog-stats'                  : 'my_sites_site_stats',
		'wp-admin-bar-plan'                        : 'my_sites_plan',
		'wp-admin-bar-plan-badge'                  : 'my_sites_plan_badge',
		// my sites - manage
		'wp-admin-bar-edit-page'                   : 'my_sites_manage_site_pages',
		'wp-admin-bar-new-page-badge'              : 'my_sites_manage_add_page',
		'wp-admin-bar-edit-post'                   : 'my_sites_manage_blog_posts',
		'wp-admin-bar-new-post-badge'              : 'my_sites_manage_add_post',
		'wp-admin-bar-edit-attachment'             : 'my_sites_manage_media',
		'wp-admin-bar-new-attachment-badge'        : 'my_sites_manage_add_media',
		'wp-admin-bar-comments'                    : 'my_sites_manage_comments',
		'wp-admin-bar-edit-jetpack-testimonial'    : 'my_sites_manage_testimonials',
		'wp-admin-bar-new-jetpack-testimonial'     : 'my_sites_manage_add_testimonial',
		'wp-admin-bar-edit-jetpack-portfolio'      : 'my_sites_manage_portfolio',
		'wp-admin-bar-new-jetpack-portfolio'       : 'my_sites_manage_add_portfolio',
		// my sites - personalize
		'wp-admin-bar-themes'                      : 'my_sites_personalize_themes',
		'wp-admin-bar-cmz'                         : 'my_sites_personalize_themes_customize',
		// my sites - configure
		'wp-admin-bar-sharing'                     : 'my_sites_configure_sharing',
		'wp-admin-bar-people'                      : 'my_sites_configure_people',
		'wp-admin-bar-people-add'                  : 'my_sites_configure_people_add_button',
		'wp-admin-bar-plugins'                     : 'my_sites_configure_plugins',
		'wp-admin-bar-domains'                     : 'my_sites_configure_domains',
		'wp-admin-bar-domains-add'                 : 'my_sites_configure_add_domain',
		'wp-admin-bar-blog-settings'               : 'my_sites_configure_settings',
		'wp-admin-bar-legacy-dashboard'            : 'my_sites_configure_wp_admin',
		// reader
		'wp-admin-bar-followed-sites'              : 'reader_followed_sites',
		'wp-admin-bar-reader-followed-sites-manage': 'reader_manage_followed_sites',
		'wp-admin-bar-discover-discover'           : 'reader_discover',
		'wp-admin-bar-discover-search'             : 'reader_search',
		'wp-admin-bar-my-activity-my-likes'        : 'reader_my_likes',
		// account
		'wp-admin-bar-user-info'                   : 'my_account_user_name',
		// account - profile
		'wp-admin-bar-my-profile'                  : 'my_account_profile_my_profile',
		'wp-admin-bar-account-settings'            : 'my_account_profile_account_settings',
		'wp-admin-bar-billing'                     : 'my_account_profile_manage_purchases',
		'wp-admin-bar-security'                    : 'my_account_profile_security',
		'wp-admin-bar-notifications'               : 'my_account_profile_notifications',
		// account - special
		'wp-admin-bar-get-apps'                    : 'my_account_special_get_apps',
		'wp-admin-bar-next-steps'                  : 'my_account_special_next_steps',
		'wp-admin-bar-help'                        : 'my_account_special_help',
	};

	var notesTracksEvents = {
		openSite: function ( data ) {
			return {
				clicked: 'masterbar_notifications_panel_site',
				site_id: data.siteId
			};
		},
		openPost: function ( data ) {
			return {
				clicked: 'masterbar_notifications_panel_post',
				site_id: data.siteId,
				post_id: data.postId
			};
		},
		openComment: function ( data ) {
			return {
				clicked: 'masterbar_notifications_panel_comment',
				site_id: data.siteId,
				post_id: data.postId,
				comment_id: data.commentId
			};
		}
	};

	// Element.prototype.matches as a standalone function, with old browser fallback
	function matches( node, selector ) {
		if ( ! node ) {
			return undefined;
		}

		if ( ! Element.prototype.matches && ! Element.prototype.msMatchesSelector ) {
			throw new Error( 'Unsupported browser' );
		}

		return Element.prototype.matches ? node.matches( selector ) : node.msMatchesSelector( selector );
	}

	// Element.prototype.closest as a standalone function, with old browser fallback
	function closest( node, selector ) {
		if ( ! node ) {
			return undefined;
		}

		if ( Element.prototype.closest ) {
			return node.closest( selector );
		}

		do {
			if ( matches( node, selector ) ) {
				return node;
			}

			node = node.parentElement || node.parentNode;
		} while ( node !== null && node.nodeType === 1 );

		return null;
	}

	function recordTracksEvent( eventProps ) {
		eventProps = eventProps || {};
		window._tkq = window._tkq || [];
		window._tkq.push( [ 'recordEvent', eventName, eventProps ] );
	}

	function parseJson( s, defaultValue ) {
		try {
			return JSON.parse( s );
		} catch ( e ) {
			return defaultValue;
		}
	}

	function createTrackableLinkEventHandler( link ) {
		return function () {
			var parent = closest( link, 'li' );

			if ( ! parent ) {
				return;
			}

			var trackingId = link.getAttribute( 'ID' ) || parent.getAttribute( 'ID' );

			if ( ! linksTracksEvents.hasOwnProperty( trackingId ) ) {
				return;
			}

			var eventProps = { 'clicked': linksTracksEvents[ trackingId ] };
			recordTracksEvent( eventProps );
		}
	}

	function init() {
		var trackableLinkSelector = '.mb-trackable .ab-item:not(div),' +
			'#wp-admin-bar-notes .ab-item,' +
			'#wp-admin-bar-user-info .ab-item,' +
			'.mb-trackable .ab-secondary';

		var trackableLinks = document.querySelectorAll( trackableLinkSelector );

		for ( var i = 0; i < trackableLinks.length; i++ ) {
			var link = trackableLinks[ i ];
			var handler = createTrackableLinkEventHandler( link );

			link.addEventListener( 'click', handler );
			link.addEventListener( 'touchstart', handler );
		}
	}

	if ( document.readyState === 'loading' ) {
		document.addEventListener( 'DOMContentLoaded', init );
	} else {
		init();
	}

	// listen for postMessage events from the notifications iframe
	window.addEventListener( 'message', function ( event ) {
		if ( event.origin !== 'https://widgets.wp.com' ) {
			return;
		}

		var data = ( typeof event.data === 'string' ) ? parseJson( event.data, {} ) : event.data;
		if ( data.type !== 'notesIframeMessage' ) {
			return;
		}

		var eventData = notesTracksEvents[ data.action ];
		if ( ! eventData ) {
			return;
		}

		recordTracksEvent( eventData( data ) );
	}, false );

} )();
;
/**
 * Observe how the user enters content into the comment form in order to determine whether it's a bot or not.
 *
 * Note that no actual input is being saved here, only counts and timings between events.
 */

( function() {
	// Passive event listeners are guaranteed to never call e.preventDefault(),
	// but they're not supported in all browsers.  Use this feature detection
	// to determine whether they're available for use.
	var supportsPassive = false;

	try {
		var opts = Object.defineProperty( {}, 'passive', {
			get : function() {
				supportsPassive = true;
			}
		} );

		window.addEventListener( 'testPassive', null, opts );
		window.removeEventListener( 'testPassive', null, opts );
	} catch ( e ) {}

	function init() {
		var input_begin = '';

		var keydowns = {};
		var lastKeyup = null;
		var lastKeydown = null;
		var keypresses = [];

		var modifierKeys = [];
		var correctionKeys = [];

		var lastMouseup = null;
		var lastMousedown = null;
		var mouseclicks = [];

		var mousemoveTimer = null;
		var lastMousemoveX = null;
		var lastMousemoveY = null;
		var mousemoveStart = null;
		var mousemoves = [];

		var touchmoveCountTimer = null;
		var touchmoveCount = 0;

		var lastTouchEnd = null;
		var lastTouchStart = null;
		var touchEvents = [];

		var scrollCountTimer = null;
		var scrollCount = 0;

		var correctionKeyCodes = [ 'Backspace', 'Delete', 'ArrowUp', 'ArrowDown', 'ArrowLeft', 'ArrowRight', 'Home', 'End', 'PageUp', 'PageDown' ];
		var modifierKeyCodes = [ 'Shift', 'CapsLock' ];

		var forms = document.querySelectorAll( 'form[method=post]' );

		for ( var i = 0; i < forms.length; i++ ) {
			var form = forms[i];

			var formAction = form.getAttribute( 'action' );

			// Ignore forms that POST directly to other domains; these could be things like payment forms.
			if ( formAction ) {
				// Check that the form is posting to an external URL, not a path.
				if ( formAction.indexOf( 'http://' ) == 0 || formAction.indexOf( 'https://' ) == 0 ) {
					if ( formAction.indexOf( 'http://' + window.location.hostname + '/' ) != 0 && formAction.indexOf( 'https://' + window.location.hostname + '/' ) != 0 ) {
						continue;
					}
				}
			}

			form.addEventListener( 'submit', function () {
				var ak_bkp = prepare_timestamp_array_for_request( keypresses );
				var ak_bmc = prepare_timestamp_array_for_request( mouseclicks );
				var ak_bte = prepare_timestamp_array_for_request( touchEvents );
				var ak_bmm = prepare_timestamp_array_for_request( mousemoves );

				var input_fields = {
					// When did the user begin entering any input?
					'ak_bib': input_begin,

					// When was the form submitted?
					'ak_bfs': Date.now(),

					// How many keypresses did they make?
					'ak_bkpc': keypresses.length,

					// How quickly did they press a sample of keys, and how long between them?
					'ak_bkp': ak_bkp,

					// How quickly did they click the mouse, and how long between clicks?
					'ak_bmc': ak_bmc,

					// How many mouseclicks did they make?
					'ak_bmcc': mouseclicks.length,

					// When did they press modifier keys (like Shift or Capslock)?
					'ak_bmk': modifierKeys.join( ';' ),

					// When did they correct themselves? e.g., press Backspace, or use the arrow keys to move the cursor back
					'ak_bck': correctionKeys.join( ';' ),

					// How many times did they move the mouse?
					'ak_bmmc': mousemoves.length,

					// How many times did they move around using a touchscreen?
					'ak_btmc': touchmoveCount,

					// How many times did they scroll?
					'ak_bsc': scrollCount,

					// How quickly did they perform touch events, and how long between them?
					'ak_bte': ak_bte,

					// How many touch events were there?
					'ak_btec' : touchEvents.length,

					// How quickly did they move the mouse, and how long between moves?
					'ak_bmm' : ak_bmm
				};

				for ( var field_name in input_fields ) {
					var field = document.createElement( 'input' );
					field.setAttribute( 'type', 'hidden' );
					field.setAttribute( 'name', field_name );
					field.setAttribute( 'value', input_fields[ field_name ] );
					this.appendChild( field );
				}
			}, supportsPassive ? { passive: true } : false  );

			form.addEventListener( 'keydown', function ( e ) {
				// If you hold a key down, some browsers send multiple keydown events in a row.
				// Ignore any keydown events for a key that hasn't come back up yet.
				if ( e.key in keydowns ) {
					return;
				}

				var keydownTime = ( new Date() ).getTime();
				keydowns[ e.key ] = [ keydownTime ];

				if ( ! input_begin ) {
					input_begin = keydownTime;
				}

				// In some situations, we don't want to record an interval since the last keypress -- for example,
				// on the first keypress, or on a keypress after focus has changed to another element. Normally,
				// we want to record the time between the last keyup and this keydown. But if they press a
				// key while already pressing a key, we want to record the time between the two keydowns.

				var lastKeyEvent = Math.max( lastKeydown, lastKeyup );

				if ( lastKeyEvent ) {
					keydowns[ e.key ].push( keydownTime - lastKeyEvent );
				}

				lastKeydown = keydownTime;
			}, supportsPassive ? { passive: true } : false  );

			form.addEventListener( 'keyup', function ( e ) {
				if ( ! ( e.key in keydowns ) ) {
					// This key was pressed before this script was loaded, or a mouseclick happened during the keypress, or...
					return;
				}

				var keyupTime = ( new Date() ).getTime();

				if ( 'TEXTAREA' === e.target.nodeName || 'INPUT' === e.target.nodeName ) {
					if ( -1 !== modifierKeyCodes.indexOf( e.key ) ) {
						modifierKeys.push( keypresses.length - 1 );
					} else if ( -1 !== correctionKeyCodes.indexOf( e.key ) ) {
						correctionKeys.push( keypresses.length - 1 );
					} else {
						// ^ Don't record timings for keys like Shift or backspace, since they
						// typically get held down for longer than regular typing.

						var keydownTime = keydowns[ e.key ][0];

						var keypress = [];

						// Keypress duration.
						keypress.push( keyupTime - keydownTime );

						// Amount of time between this keypress and the previous keypress.
						if ( keydowns[ e.key ].length > 1 ) {
							keypress.push( keydowns[ e.key ][1] );
						}

						keypresses.push( keypress );
					}
				}

				delete keydowns[ e.key ];

				lastKeyup = keyupTime;
			}, supportsPassive ? { passive: true } : false  );

			form.addEventListener( "focusin", function ( e ) {
				lastKeydown = null;
				lastKeyup = null;
				keydowns = {};
			}, supportsPassive ? { passive: true } : false  );

			form.addEventListener( "focusout", function ( e ) {
				lastKeydown = null;
				lastKeyup = null;
				keydowns = {};
			}, supportsPassive ? { passive: true } : false  );
		}

		document.addEventListener( 'mousedown', function ( e ) {
			lastMousedown = ( new Date() ).getTime();
		}, supportsPassive ? { passive: true } : false  );

		document.addEventListener( 'mouseup', function ( e ) {
			if ( ! lastMousedown ) {
				// If the mousedown happened before this script was loaded, but the mouseup happened after...
				return;
			}

			var now = ( new Date() ).getTime();

			var mouseclick = [];
			mouseclick.push( now - lastMousedown );

			if ( lastMouseup ) {
				mouseclick.push( lastMousedown - lastMouseup );
			}

			mouseclicks.push( mouseclick );

			lastMouseup = now;

			// If the mouse has been clicked, don't record this time as an interval between keypresses.
			lastKeydown = null;
			lastKeyup = null;
			keydowns = {};
		}, supportsPassive ? { passive: true } : false  );

		document.addEventListener( 'mousemove', function ( e ) {
			if ( mousemoveTimer ) {
				clearTimeout( mousemoveTimer );
				mousemoveTimer = null;
			}
			else {
				mousemoveStart = ( new Date() ).getTime();
				lastMousemoveX = e.offsetX;
				lastMousemoveY = e.offsetY;
			}

			mousemoveTimer = setTimeout( function ( theEvent, originalMousemoveStart ) {
				var now = ( new Date() ).getTime() - 500; // To account for the timer delay.

				var mousemove = [];
				mousemove.push( now - originalMousemoveStart );
				mousemove.push(
					Math.round(
						Math.sqrt(
							Math.pow( theEvent.offsetX - lastMousemoveX, 2 ) +
							Math.pow( theEvent.offsetY - lastMousemoveY, 2 )
						)
					)
				);

				if ( mousemove[1] > 0 ) {
					// If there was no measurable distance, then it wasn't really a move.
					mousemoves.push( mousemove );
				}

				mousemoveStart = null;
				mousemoveTimer = null;
			}, 500, e, mousemoveStart );
		}, supportsPassive ? { passive: true } : false  );

		document.addEventListener( 'touchmove', function ( e ) {
			if ( touchmoveCountTimer ) {
				clearTimeout( touchmoveCountTimer );
			}

			touchmoveCountTimer = setTimeout( function () {
				touchmoveCount++;
			}, 500 );
		}, supportsPassive ? { passive: true } : false );

		document.addEventListener( 'touchstart', function ( e ) {
			lastTouchStart = ( new Date() ).getTime();
		}, supportsPassive ? { passive: true } : false );

		document.addEventListener( 'touchend', function ( e ) {
			if ( ! lastTouchStart ) {
				// If the touchstart happened before this script was loaded, but the touchend happened after...
				return;
			}

			var now = ( new Date() ).getTime();

			var touchEvent = [];
			touchEvent.push( now - lastTouchStart );

			if ( lastTouchEnd ) {
				touchEvent.push( lastTouchStart - lastTouchEnd );
			}

			touchEvents.push( touchEvent );

			lastTouchEnd = now;

			// Don't record this time as an interval between keypresses.
			lastKeydown = null;
			lastKeyup = null;
			keydowns = {};
		}, supportsPassive ? { passive: true } : false );

		document.addEventListener( 'scroll', function ( e ) {
			if ( scrollCountTimer ) {
				clearTimeout( scrollCountTimer );
			}

			scrollCountTimer = setTimeout( function () {
				scrollCount++;
			}, 500 );
		}, supportsPassive ? { passive: true } : false );
	}

	/**
	 * For the timestamp data that is collected, don't send more than `limit` data points in the request.
	 * Choose a random slice and send those.
	 */
	function prepare_timestamp_array_for_request( a, limit ) {
		if ( ! limit ) {
			limit = 100;
		}

		var rv = '';

		if ( a.length > 0 ) {
			var random_starting_point = Math.max( 0, Math.floor( Math.random() * a.length - limit ) );

			for ( var i = 0; i < limit && i < a.length; i++ ) {
				rv += a[ random_starting_point + i ][0];

				if ( a[ random_starting_point + i ].length >= 2 ) {
					rv += "," + a[ random_starting_point + i ][1];
				}

				rv += ";";
			}
		}

		return rv;
	}

	if ( document.readyState !== 'loading' ) {
		init();
	} else {
		document.addEventListener( 'DOMContentLoaded', init );
	}
})();;
!function(){var e=document.currentScript;function t(t){var n=document.createElement("script"),o=e||document.getElementsByTagName("script")[0];n.setAttribute("async",!0),n.setAttribute("src",t),o.parentNode.insertBefore(n,o)}function n(e,t){return Element.prototype.matches?e.matches(t):Element.prototype.msMatchesSelector?e.msMatchesSelector(t):void 0}function o(e,t){if(e.closest)return e.closest(t);var o=e;do{if(n(o,t))return o;o=o.parentElement||o.parentNode}while(null!==o&&1===o.nodeType);return null}function i(e,t){for(var n=0;n<e.length;n++)t(e[n],n,e)}var r=".sharing-hidden .inner",s="data-sharing-more-button-id";function a(e){this.button=e,this.pane=o(e,"div").querySelector(r),this.openedBy=null,this.recentlyOpenedByHover=!1,a.instances.push(this),this.pane.setAttribute(s,a.instances.length-1),this.attachHandlers()}if(a.instances=[],a.hoverOpenDelay=200,a.recentOpenDelay=400,a.hoverCloseDelay=300,a.instantiateOrReuse=function(e){var t=o(e,"div").querySelector(r),n=t&&t.getAttribute(s),i=a.instances[n];return i||new a(e)},a.getButtonInstanceFromPane=function(e){var t=e&&e.getAttribute(s);return a.instances[t]},a.closeAll=function(){for(var e=0;e<a.instances.length;e++)a.instances[e].close()},a.prototype.open=function(){var e,t,n=[0,0];function o(e){var t=e.getBoundingClientRect();return[t.left+(window.scrollX||window.pageXOffset||0),t.top+(window.scrollY||window.pageYOffset||0)]}function i(e,t){return parseInt(getComputedStyle(e).getPropertyValue(t)||0)}for(e=o(this.button),t=this.button.offsetParent||document.documentElement;t&&(t===document.body||t===document.documentElement)&&"static"===getComputedStyle(t).getPropertyValue("position");)t=t.parentNode;t&&t!==this.button&&1===t.nodeType&&(n=[(n=o(t))[0]+i(t,"border-left-width"),n[1]+i(t,"border-top-width")]);var r,s=e[0]-n[0]-i(this.button,"margin-left"),a=e[1]-n[1]-i(this.button,"margin-top");this.pane.style.left=s+"px",this.pane.style.top=a+this.button.offsetHeight+3+"px",(r=this.pane)&&r.style.removeProperty("display")},a.prototype.close=function(){var e;(e=this.pane)&&(e.style.display="none"),this.openedBy=null},a.prototype.toggle=function(){var e;(e=this.pane)&&"none"!==e.style.display?this.close():this.open()},a.prototype.resetCloseTimer=function(){clearTimeout(this.closeTimer),this.closeTimer=setTimeout(this.close.bind(this),a.hoverCloseDelay)},a.prototype.attachHandlers=function(){this.buttonClick=function(e){e.preventDefault(),e.stopPropagation(),this.openedBy="click",clearTimeout(this.openTimer),clearTimeout(this.closeTimer),this.recentlyOpenedByHover?(this.recentlyOpenedByHover=!1,clearTimeout(this.hoverOpenTimer),this.open()):this.toggle()}.bind(this),this.buttonEnter=function(){this.openedBy||(this.openTimer=setTimeout(function(){this.open(),this.openedBy="hover",this.recentlyOpenedByHover=!0,this.hoverOpenTimer=setTimeout(function(){this.recentlyOpenedByHover=!1}.bind(this),a.recentOpenDelay)}.bind(this),a.hoverOpenDelay)),clearTimeout(this.closeTimer)}.bind(this),this.buttonLeave=function(){"hover"===this.openedBy&&this.resetCloseTimer(),clearTimeout(this.openTimer)}.bind(this),this.paneEnter=function(){clearTimeout(this.closeTimer)}.bind(this),this.paneLeave=function(){"hover"===this.openedBy&&this.resetCloseTimer()}.bind(this),this.documentClick=function(){this.close()}.bind(this),this.button.addEventListener("click",this.buttonClick),document.addEventListener("click",this.documentClick),void 0===document.ontouchstart&&(this.button.addEventListener("mouseenter",this.buttonEnter),this.button.addEventListener("mouseleave",this.buttonLeave),this.pane.addEventListener("mouseenter",this.paneEnter),this.pane.addEventListener("mouseleave",this.paneLeave))},window.sharing_js_options&&window.sharing_js_options.counts){var c={done_urls:[],get_counts:function(){var e,n,o,i,r;if("undefined"!=typeof WPCOM_sharing_counts)for(e in WPCOM_sharing_counts)if(o=WPCOM_sharing_counts[e],void 0===c.done_urls[o]){for(i in n={pinterest:[window.location.protocol+"//api.pinterest.com/v1/urls/count.json?callback=WPCOMSharing.update_pinterest_count&url="+encodeURIComponent(e)]})if(document.querySelector("a[data-shared=sharing-"+i+"-"+o+"]")){for(;r=n[i].pop();)t(r);window.sharing_js_options.is_stats_active&&c.bump_sharing_count_stat(i)}c.done_urls[o]=!0}},update_pinterest_count:function(e){void 0!==e.count&&1*e.count>0&&c.inject_share_count("sharing-pinterest-"+WPCOM_sharing_counts[e.url],e.count)},inject_share_count:function(e,t){i(document.querySelectorAll("a[data-shared="+e+"] > span"),(function(e){var n,o=e.querySelector(".share-count");(n=o)&&n.parentNode&&n.parentNode.removeChild(n);var i=document.createElement("span");i.className="share-count",i.textContent=c.format_count(t),e.appendChild(i)}))},format_count:function(e){return e<1e3?e:e>=1e3&&e<1e4?String(e).substring(0,1)+"K+":"10K+"},bump_sharing_count_stat:function(e){(new Image).src=document.location.protocol+"//pixel.wp.com/g.gif?v=wpcom-no-pv&x_sharing-count-request="+e+"&r="+Math.random()}};window.WPCOMSharing=c}function u(e,t){e.setAttribute("jetpack-share-click-count",t)}function l(e){var t=e.getAttribute("jetpack-share-click-count");return null===t?0:parseInt(t,10)}function d(e,t){var n,o=new XMLHttpRequest;o.open("POST",e,!0),o.setRequestHeader("Content-Type","application/x-www-form-urlencoded; charset=UTF-8"),o.setRequestHeader("x-requested-with","XMLHttpRequest"),o.send((n=t,(encodeURIComponent("email-share-nonce")+"="+encodeURIComponent(n)).replace(/%20/g,"+")))}function h(){p()}function p(){window.WPCOMSharing&&window.WPCOMSharing.get_counts(),i(document.querySelectorAll(".sharedaddy a"),(function(e){var t=e.getAttribute("href");t&&-1!==t.indexOf("share=")&&-1===t.indexOf("&nb=1")&&e.setAttribute("href",t+"&nb=1")})),i(document.querySelectorAll(".sharedaddy a.sharing-anchor"),(function(e){a.instantiateOrReuse(e)})),void 0!==document.ontouchstart&&document.body.classList.add("jp-sharing-input-touch"),i(document.querySelectorAll(".sharedaddy ul"),(function(e){"true"!==e.getAttribute("data-sharing-events-added")&&(e.setAttribute("data-sharing-events-added","true"),i(e.querySelectorAll("a.share-print"),(function(e){e.addEventListener("click",(function(t){t.preventDefault(),t.stopPropagation();var n=e.getAttribute("href")||"",i=function(){if(-1===n.indexOf("#print")){var e=(new Date).getTime();t=e,o=n,(i=document.createElement("iframe")).setAttribute("style","position:fixed; top:100; left:100; height:1px; width:1px; border:none;"),i.setAttribute("id","printFrame-"+t),i.setAttribute("name",i.getAttribute("id")),i.setAttribute("src",o),i.setAttribute("onload",'frames["printFrame-'+t+'"].focus();frames["printFrame-'+t+'"].print();'),document.body.appendChild(i)}else window.print();var t,o,i},s=o(e,r);if(s){var c=a.getButtonInstanceFromPane(s);c&&(c.close(),i())}else i()}))})),i(e.querySelectorAll("a.share-press-this"),(function(e){e.addEventListener("click",(function(t){t.preventDefault(),t.stopPropagation();var n="";if(window.getSelection?n=window.getSelection():document.getSelection?n=document.getSelection():document.selection&&(n=document.selection.createRange().text),n){var o=e.getAttribute("href");e.setAttribute("href",o+"&sel="+encodeURI(n))}window.open(e.getAttribute("href"),"t","toolbar=0,resizable=1,scrollbars=1,status=1,width=720,height=570")||(document.location.href=e.getAttribute("href"))}))})),i(e.querySelectorAll("a.share-email"),(function(t){u(t,0);var n,o,r=t.getAttribute("data-email-share-nonce"),s=t.getAttribute("data-email-share-track-url");r&&s&&(n=s,o=window.location.protocol+"//"+window.location.hostname+"/",0===String(n).indexOf(o))&&t.addEventListener("click",(function(){var n;u(n=t,l(n)+1),l(t)>2&&function(e,t){var n=t.parentElement;if(n.classList.contains("sd-content")){i(n.querySelectorAll(".share-email-error"),(function(e){e.parentElement.removeChild(e)}));var o=document.createElement("div");o.className="share-email-error";var r=document.createElement("h6");r.className="share-email-error-title",r.innerText=e.getAttribute("data-email-share-error-title"),o.appendChild(r);var s=document.createElement("p");s.className="share-email-error-text",s.innerText=e.getAttribute("data-email-share-error-text"),o.appendChild(s),n.appendChild(o)}}(t,e),d(s,r)}))})))})),i(document.querySelectorAll("li.share-email, li.share-custom a.sharing-anchor"),(function(e){e.classList.add("share-service-visible")}))}"loading"!==document.readyState?h():document.addEventListener("DOMContentLoaded",h),document.body.addEventListener("is.post-load",p)}();;

